Introducing Automated Regression Testing in Open Source Projects

To learn how to introduce automated regression testing to existing medium scale Open Source projects, a long-term field experiment was performed with the Open Source project FreeCol. Results indicate that (1) introducing testing is both beneficial for the project and feasible for an outside innovator, (2) testing can enhance communication between developers, (3) signaling is important for engaging the project participants to fill a newly vacant position left by a withdrawal of the innovator. Five prescriptive strategies are extracted for the innovator and two conjectures offered about the ability of an Open Source project to learn about innovations.

==> 02-testing.tex <==

\section{Automated testing}\label{sec:freecol:testing}

Automated testing is the practice of writing executable specification against
which an application can automatically be tested. ``Automated testing'' is used
as a term to distinguish from manual testing in which software response is
verified by a human against manually entered input.\footnote{From now on, we will
use the unqualified term of \emph{testing} as referring to \emph{automated}
testing exclusively and will qualify all occurrences of testing as pertaining to
manual testing respectively.} We typically distinguish unit testing of individual
classes and modules, integration testing of the interaction of several modules,
and system testing of the application in the context of later
use~\cite[p.77]{WhittakerJA00}. Since the boundaries between these different
testing scopes are often hard to draw precisely, the term unit testing, which was
originally reserved for testing the smallest possible unit in isolation and
allowing also manual execution, has become near synonymous with automated testing
independent of the granularity of the tests contained in a test suite.


While automated testing is primarily a quality assurance technique to achieve
compliance with specification, it also has become popular to view it (a) as a
specification in its own right, for instance when translating an ambiguous bug
report into a specific test case, and (b) as a means to track development
progress by the individual developer (``you will be done developing when the test
runs''~\cite{BecGam00}).


It is not necessarily defined at which time the test cases are created with
relation to the code they are testing. In a waterfall or V model software
development process it is likely that unit and integration tests will be created
bottom-up in a ``sequential fashion'' after implementation and integration
respectively~\cite{JorEri94} and in a dedicated testing department. Yet, with the
advent of more agile development processes, developers have become increasingly
involved in writing tests during or even before implementation. Such
\emph{test-driven development} (TDD, also ``test-first'') has received a lot of
attention in academia and industry~\cite{JefMel07} and is characterized by
repeated cycles of writing tests, implementing functionality to pass the tests
and subsequent refactoring to improve the quality of the code.


The last step in the TDD cycle is aided by the \emph{regression} detecting 
capabilities of a test suite. Since tests ensure compliance to the behavior 
coded in them, deviations from this behavior will cause affected tests to fail. 
This capability of tests is cited to increase developers' confidence to 
refactoring code~\cite[p.129]{MenTou04}.

Lastly, for the relationship between testing and finding bugs in software, the
black-box properties of the test execution must be regarded. This is famously
summarized by Dijktra's remark that ``Program testing can be used to show the
presence of bugs, but never to show their absence''~\cite{DijkstraEW70}, which
reminds us that tests compare expected and actual output of the program for a
defined set of scenarios and do not prove correctness of the code. In practical
terms this means that even though the tester derives confidence about the quality
of the code by successfully testing a program, it still might be that the tests
(1) do not \emph{cover} all the scenarios in which the code might be used, (2)
contain bugs themselves, and (3) do not detect interrelating defects that result
in seemingly correct behavior.


% Automated testing has become one of the most widely spread software
% engineering inventions~\cite{xxx}, easily the number one of quality
% assurance methods used.
% 
 
At this point we do not further qualify what kinds of means and ends
are targeted by the habit of automated testing (for instance whether
developers translate bug reports to test cases or use it for test-driven
development), but rather leave the exact kind of usage up to the Open
Source project and its specific requirements.


==> command-definitions.tex <==

\makeatletter

% Gmanda References point to the cited email.
% Param #1 = name of mailing-list
% Param #2 = id of message
\newcommand{\internalgref}[3]{[%
	\newif\ifgref%
  	\greftrue%
 	\ifthenelse{\equal{#1}{kvm}}{%
		\href{http://article.gmane.org/gmane.comp.emulators.kvm.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{xfce}}{%
		\href{http://article.gmane.org/gmane.comp.desktop.xfce.devel.version4/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{rox}}{%
		\href{http://article.gmane.org/gmane.comp.desktop.rox.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{freedos}}{%
		\href{http://article.gmane.org/gmane.comp.emulators.freedos.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{bochs}}{%
		\href{http://article.gmane.org/gmane.comp.emulators.bochs.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{rt}}{%
		\href{http://article.gmane.org/gmane.comp.bug-tracking.request-tracker.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{flyspray}}{%
		\href{http://article.gmane.org/gmane.comp.bug-tracking.flyspray.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{uboot}}{%
		\href{http://article.gmane.org/gmane.comp.boot-loaders.u-boot/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{grub}}{%
		\href{http://article.gmane.org/gmane.comp.boot-loaders.grub.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{koha}}{%
		\href{http://article.gmane.org/gmane.education.libraries.koha.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{bugzilla}}{%
		\href{http://article.gmane.org/gmane.comp.bug-tracking.bugzilla.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{geda}}{%
		\href{http://article.gmane.org/gmane.comp.cad.geda.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{argouml}}{%
		\href{http://article.gmane.org/gmane.comp.db.axion.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{monetdb}}{%
		\href{http://article.gmane.org/gmane.comp.db.monetdb.devel/#2}{#3}%
		\greffalse%
  	}{}%
	\ifthenelse{\equal{#1}{kernel}}{%
		\href{http://article.gmane.org/gmane.linux.kernel/#2}{#3}%
		\greffalse%
  	}{}%
  	 \ifthenelse{\equal{#1}{freecol}}{%
  	      \@ifundefined{freecol-developers.mbox_#2}{%
             \PackageWarning{GmanDA}{Undefined Email #2 in List #1}%
          }{%
             \href{http://sourceforge.net/mailarchive/message.php?msg_name=\@nameuse{freecol-developers.mbox_#2}}{#3}%
             \greffalse%
          }%
    }{}%
	\ifgref%
		\PackageWarning{GmanDA}{Unknown mailing-list #1}%
		#3 (??)%
    \fi]%
}

\makeatother

%
% GmandaReference(list: String, id: int)
%
\newcommand{\gref}[2]{\internalgref{#1}{#2}{#1:#2}}

% dref - Definition References. Points to the Glossary and puts the given
% explaination/term in emphasis.
\newcommand{\dref}[2]{\emph{\hyperref[def:#1]{#2}}}

\newcommand{\ddref}[1]{\texttt{\hyperref[def:#1]{#1}}}

\makeatletter

\@namedef{freecol-developers.mbox_1}{3C5EB8BC.5070809\%40easynet.be}
\@namedef{freecol-developers.mbox_2}{3C5F97A1.6090408\%40easynet.be}
\@namedef{freecol-developers.mbox_3}{OF57B18E38.46454FD9-ON03256B57.00503A95\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_4}{3C60029B.3000100\%40easynet.be}
\@namedef{freecol-developers.mbox_5}{3C601806.3090202\%40TeleLev.net}
\@namedef{freecol-developers.mbox_6}{3C601D1D.4060706\%40TeleLev.net}
\@namedef{freecol-developers.mbox_7}{3C60E48C.1030405\%40easynet.be}
\@namedef{freecol-developers.mbox_8}{OFB5EBC9A6.30A6CD94-ON03256B58.006E163A\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_9}{3C64F452.7090704\%40easynet.be}
\@namedef{freecol-developers.mbox_10}{3C6531F1.C3D89990\%40swissonline.ch}
\@namedef{freecol-developers.mbox_11}{3C65334D.3090705\%40easynet.be}
\@namedef{freecol-developers.mbox_12}{3C666CB1.1030802\%40easynet.be}
\@namedef{freecol-developers.mbox_14}{3C693996.5030907\%40easynet.be}
\@namedef{freecol-developers.mbox_13}{3C681430.CB08A043\%40swissonline.ch}
\@namedef{freecol-developers.mbox_15}{000001c1b40f$62b9d6e0$0200a8c0\%40casia}
\@namedef{freecol-developers.mbox_16}{3C6A338A.20803\%40easynet.be}
\@namedef{freecol-developers.mbox_17}{Pine.SOL.4.30.0202131410050.2331-100000\%40grey03.nada.kth.se}
\@namedef{freecol-developers.mbox_20}{3C6A9376.5070703\%40easynet.be}
\@namedef{freecol-developers.mbox_26}{003001c1b5cf$1700ca30$a4294c42\%40roosserver}
\@namedef{freecol-developers.mbox_18}{OFAF351DFF.7C5CB493-ON03256B5F.004C6FAF\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_19}{OF78ED1F3E.F80461B8-ON03256B5F.004DA9A8\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_21}{3C6AE310.C20E473E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_22}{001d01c1b4e1$2bea4820$01a97c35\%40DURON800}
\@namedef{freecol-developers.mbox_23}{3C6B6F89.1020400\%40easynet.be}
\@namedef{freecol-developers.mbox_27}{003f01c1b5cf$5e44a7e0$a4294c42\%40roosserver}
\@namedef{freecol-developers.mbox_24}{3C6C27F1.326F1C50\%40swissonline.ch}
\@namedef{freecol-developers.mbox_25}{3C6C2E51.88CB6CC9\%40swissonline.ch}
\@namedef{freecol-developers.mbox_28}{Pine.SOL.4.30.0202161045190.15584-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_30}{3C6E3B6B.4060204\%40easynet.be}
\@namedef{freecol-developers.mbox_29}{002201c1b6d3$e49f89e0$01a97c35\%40DURON800}
\@namedef{freecol-developers.mbox_31}{3C6E3FD1.5000004\%40easynet.be}
\@namedef{freecol-developers.mbox_37}{002e01c1b72a$ab120980$a4294c42\%40roosserver}
\@namedef{freecol-developers.mbox_39}{3C6F80D9.70106\%40easynet.be}
\@namedef{freecol-developers.mbox_32}{3C6E67E2.5040508\%40TeleLev.net}
\@namedef{freecol-developers.mbox_33}{Pine.SOL.4.30.0202161412510.17374-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_34}{3C6E6B80.6030509\%40TeleLev.net}
\@namedef{freecol-developers.mbox_35}{Pine.SOL.4.30.0202161423550.17374-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_36}{Pine.SOL.4.30.0202161414320.17374-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_38}{3C6EDB66.A0A7AC70\%40swissonline.ch}
\@namedef{freecol-developers.mbox_40}{00a001c1b79e$affe9f20$01a97c35\%40DURON800}
\@namedef{freecol-developers.mbox_41}{3C6F8BC4.2090409\%40easynet.be}
\@namedef{freecol-developers.mbox_42}{Pine.SOL.4.30.0202181134220.13909-100000\%40altair.nada.kth.se}
\@namedef{freecol-developers.mbox_43}{3C70FD24.5040305\%40easynet.be}
\@namedef{freecol-developers.mbox_44}{Pine.SOL.4.30.0202181415230.29434-100000\%40red09.nada.kth.se}
\@namedef{freecol-developers.mbox_45}{3C710B19.6030004\%40easynet.be}
\@namedef{freecol-developers.mbox_46}{000801c1b8a9$b254a4c0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_47}{OFFBB2CF48.2FE77C36-ON03256B64.0065A255\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_48}{3C717E8F.283EACD9\%40swissonline.ch}
\@namedef{freecol-developers.mbox_49}{20020219072735.29885.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_50}{3C720F69.6090902\%40easynet.be}
\@namedef{freecol-developers.mbox_51}{Pine.SOL.4.30.0202190945160.24987-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_52}{3C7218FC.20104\%40easynet.be}
\@namedef{freecol-developers.mbox_53}{Pine.SOL.4.30.0202191035340.2587-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_55}{20020219135057.30130.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_54}{OFE42BB78D.56659129-ON03256B65.004A747D\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_56}{3C725A85.30703\%40easynet.be}
\@namedef{freecol-developers.mbox_57}{3C726009.6050909\%40easynet.be}
\@namedef{freecol-developers.mbox_58}{OF0932782F.C3622756-ON03256B65.00509867\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_59}{3C726CAD.3070808\%40easynet.be}
\@namedef{freecol-developers.mbox_60}{OFD3789EF3.2418053E-ON03256B65.005807E3\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_61}{3C72A3ED.E55EA995\%40swissonline.ch}
\@namedef{freecol-developers.mbox_62}{000001c1b98a$dde51d90$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_63}{3C73BF0E.D95E534B\%40fak.ch}
\@namedef{freecol-developers.mbox_64}{3C7682A4.2030500\%40TeleLev.net}
\@namedef{freecol-developers.mbox_65}{OFD92C762A.2D473DBB-ON03256B68.005D9272\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_66}{3C768D74.6040103\%40easynet.be}
\@namedef{freecol-developers.mbox_67}{3C768F76.80848377\%40swissonline.ch}
\@namedef{freecol-developers.mbox_68}{Pine.SOL.4.30.0202222004400.1188-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_70}{3C76B605.8FB1B868\%40swissonline.ch}
\@namedef{freecol-developers.mbox_69}{000801c1bbda$d9ec4810$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_71}{Pine.SOL.4.30.0202222306420.1188-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_72}{000001c1bc95$95c80ff0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_73}{3C77645E.3010209\%40easynet.be}
\@namedef{freecol-developers.mbox_74}{000101c1bc9d$4a3acf20$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_75}{3C77E94C.1080209\%40easynet.be}
\@namedef{freecol-developers.mbox_76}{3C78064D.A3F1AE6E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_77}{3C78B9FB.2050300\%40easynet.be}
\@namedef{freecol-developers.mbox_78}{Pine.SOL.4.30.0202241128070.2376-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_79}{3C78C521.8060007\%40easynet.be}
\@namedef{freecol-developers.mbox_80}{000001c1bd25$1f7670e0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_81}{3C78D52E.415B0CC3\%40swissonline.ch}
\@namedef{freecol-developers.mbox_82}{000101c1bd2a$c02a0560$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_83}{3C78DA26.B27C0E2F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_84}{Pine.SOL.4.30.0202241321030.2376-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_86}{3C78E361.8A1C9729\%40swissonline.ch}
\@namedef{freecol-developers.mbox_85}{3C78E170.7EFC3ABE\%40swissonline.ch}
\@namedef{freecol-developers.mbox_87}{3C78EFD8.482AA9E6\%40swissonline.ch}
\@namedef{freecol-developers.mbox_88}{3C78F1D9.E4B9C8DD\%40swissonline.ch}
\@namedef{freecol-developers.mbox_89}{OFC82A0D58.4A9C63E8-ON03256B6B.0051D0E1\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_91}{3C7A592E.3040506\%40easynet.be}
\@namedef{freecol-developers.mbox_90}{OFDB318C2A.E97C7B05-ON03256B6B.00547EBA\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_92}{3C7A5B16.2030601\%40easynet.be}
\@namedef{freecol-developers.mbox_93}{3C7A7E73.6AC23B8E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_94}{3C7AB5E4.87142659\%40swissonline.ch}
\@namedef{freecol-developers.mbox_95}{000001c1be4a$3579da00$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_96}{OFCD22280F.570C6F32-ON03256B6C.00466CAF\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_97}{3C7B9608.80902\%40easynet.be}
\@namedef{freecol-developers.mbox_98}{3C7BBA02.276A8503\%40swissonline.ch}
\@namedef{freecol-developers.mbox_99}{3C7BC810.2B68F6C6\%40swissonline.ch}
\@namedef{freecol-developers.mbox_100}{3C7BD7C2.80901\%40easynet.be}
\@namedef{freecol-developers.mbox_101}{3C7BE69C.5A03FA34\%40swissonline.ch}
\@namedef{freecol-developers.mbox_102}{000001c1bf05$1c700690$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_103}{3C7C04E8.6A141670\%40swissonline.ch}
\@namedef{freecol-developers.mbox_104}{000001c1bfdc$03b24690$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_105}{3C7E8491.1B375B6E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_106}{3C7E8C84.D2A60B3F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_110}{3C7F34D6.9000600\%40easynet.be}
\@namedef{freecol-developers.mbox_107}{3C7E8D98.E7B615B6\%40swissonline.ch}
\@namedef{freecol-developers.mbox_108}{Pine.SOL.4.30.0202282216510.26281-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_109}{3C7EAA8E.D5A6213E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_111}{3C7FDE29.962BDC13\%40swissonline.ch}
\@namedef{freecol-developers.mbox_114}{3C809556.6070501\%40easynet.be}
\@namedef{freecol-developers.mbox_112}{3C7FE01E.37FB6734\%40swissonline.ch}
\@namedef{freecol-developers.mbox_113}{000301c1c15c$9ba2bc10$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_115}{3C81490B.28E85907\%40swissonline.ch}
\@namedef{freecol-developers.mbox_116}{3C814A8E.5376EB8F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_117}{3C828C8F.5AD6DE40\%40swissonline.ch}
\@namedef{freecol-developers.mbox_118}{3C85281E.82D91755\%40swissonline.ch}
\@namedef{freecol-developers.mbox_119}{3C87576E.2020507\%40easynet.be}
\@namedef{freecol-developers.mbox_120}{20020307161717.13318.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_121}{3C8796A1.2040406\%40easynet.be}
\@namedef{freecol-developers.mbox_122}{3C892ADE.3269BDC3\%40swissonline.ch}
\@namedef{freecol-developers.mbox_123}{3C8A0750.7AAB8A1C\%40swissonline.ch}
\@namedef{freecol-developers.mbox_124}{3C8A0973.63D0EB47\%40swissonline.ch}
\@namedef{freecol-developers.mbox_125}{3C8A10DD.F0D99881\%40swissonline.ch}
\@namedef{freecol-developers.mbox_126}{000101c1c77c$081153f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_129}{3C8A53A6.2090307\%40easynet.be}
\@namedef{freecol-developers.mbox_127}{3C8A37D8.7A93F50A\%40swissonline.ch}
\@namedef{freecol-developers.mbox_128}{3C8A4229.C31CB115\%40swissonline.ch}
\@namedef{freecol-developers.mbox_130}{3C8A5ACF.71D0CC75\%40swissonline.ch}
\@namedef{freecol-developers.mbox_131}{3C8A7652.BC230329\%40swissonline.ch}
\@namedef{freecol-developers.mbox_132}{3C8A8122.1B428BB3\%40swissonline.ch}
\@namedef{freecol-developers.mbox_133}{3C8A8124.B8B806F2\%40swissonline.ch}
\@namedef{freecol-developers.mbox_134}{3C8B3829.8090101\%40easynet.be}
\@namedef{freecol-developers.mbox_135}{000001c1c866$81e718f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_136}{3C8BB6D7.6030205\%40easynet.be}
\@namedef{freecol-developers.mbox_137}{3C8BCBEA.6FFADCFF\%40swissonline.ch}
\@namedef{freecol-developers.mbox_138}{3C8E3A82.53F94895\%40swissonline.ch}
\@namedef{freecol-developers.mbox_139}{3C8E3BF6.8080408\%40easynet.be}
\@namedef{freecol-developers.mbox_140}{3C8E5015.B2FBB578\%40swissonline.ch}
\@namedef{freecol-developers.mbox_141}{3C8E6767.81EE4C0C\%40swissonline.ch}
\@namedef{freecol-developers.mbox_142}{3C8F043B.1030704\%40easynet.be}
\@namedef{freecol-developers.mbox_143}{3C8F9B45.2E813DAA\%40swissonline.ch}
\@namedef{freecol-developers.mbox_144}{3C8F9B6A.76ABF0C0\%40swissonline.ch}
\@namedef{freecol-developers.mbox_145}{000101c1cacd$32141d50$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_147}{3C909AD6.1050302\%40easynet.be}
\@namedef{freecol-developers.mbox_146}{Pine.SOL.4.30.0203140902550.904-100000\%40red19.nada.kth.se}
\@namedef{freecol-developers.mbox_149}{3C90DF05.EA470749\%40swissonline.ch}
\@namedef{freecol-developers.mbox_148}{3C90D42F.F9AD8F64\%40swissonline.ch}
\@namedef{freecol-developers.mbox_150}{3C9105B9.2B5E89BA\%40swissonline.ch}
\@namedef{freecol-developers.mbox_151}{000001c1ccc3$b614ccb0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_152}{Pine.SOL.4.30.0203142251410.3903-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_153}{3C934059.E6CA94E0\%40swissonline.ch}
\@namedef{freecol-developers.mbox_154}{3C934404.6D5EE725\%40swissonline.ch}
\@namedef{freecol-developers.mbox_155}{000001c1cd19$f9661d60$0200a8c0\%40casia}
\@namedef{freecol-developers.mbox_156}{3C939707.9030109\%40easynet.be}
\@namedef{freecol-developers.mbox_157}{000001c1cd99$c138f3b0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_158}{3C9479F5.70601\%40easynet.be}
\@namedef{freecol-developers.mbox_159}{Pine.SOL.4.30.0203180817390.8012-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_160}{20020318074850.22543.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_161}{Pine.SOL.4.30.0203180845080.8012-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_162}{20020318091309.22656.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_163}{3C962363.2080302\%40easynet.be}
\@namedef{freecol-developers.mbox_164}{000001c1cea6$b1261300$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_165}{Pine.SOL.4.30.0203251703200.3473-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_166}{3C9F5E49.2090504\%40easynet.be}
\@namedef{freecol-developers.mbox_167}{000201c1d42a$71979900$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_168}{3C9F735B.8000108\%40easynet.be}
\@namedef{freecol-developers.mbox_169}{Pine.SOL.4.30.0203252029020.12170-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_170}{Pine.SOL.4.30.0203252055560.12170-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_177}{3CA02A7B.1040706\%40easynet.be}
\@namedef{freecol-developers.mbox_171}{000001c1d438$17b63a00$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_172}{000101c1d438$ced30ec0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_173}{000001c1d439$98ac7d30$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_174}{Pine.SOL.4.30.0203252127150.12170-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_175}{000001c1d48b$b787d680$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_176}{3CA028B6.5000800\%40easynet.be}
\@namedef{freecol-developers.mbox_178}{20020326101439.4444.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_179}{3CA04C80.7000007\%40easynet.be}
\@namedef{freecol-developers.mbox_180}{20020326222749.218b1f2c.Linuxer\%40TeleLev.net}
\@namedef{freecol-developers.mbox_181}{000001c1d505$c0ed8970$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_182}{000001c1d5c7$711738c0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_183}{3CA359F0.20906\%40easynet.be}
\@namedef{freecol-developers.mbox_184}{20020329110528.4004035a.Linuxer\%40TeleLev.net}
\@namedef{freecol-developers.mbox_185}{3CA47869.60304\%40easynet.be}
\@namedef{freecol-developers.mbox_186}{20020330130722.322baa55.Linuxer\%40TeleLev.net}
\@namedef{freecol-developers.mbox_188}{3CA5CEF8.6040308\%40easynet.be}
\@namedef{freecol-developers.mbox_187}{NFBBKFIOILGINLHMNCDFIEHPCDAA.colorrr\%40usa.net}
\@namedef{freecol-developers.mbox_189}{3CA5F1F8.C1ABE9C9\%40swissonline.ch}
\@namedef{freecol-developers.mbox_190}{000001c1d81e$8947d810$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_191}{3CA62672.3C37451\%40swissonline.ch}
\@namedef{freecol-developers.mbox_192}{000101c1d887$871242b0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_193}{3CA6FB18.2010101\%40easynet.be}
\@namedef{freecol-developers.mbox_194}{000201c1d99f$dbefae30$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_195}{3CA89F5A.8020604\%40easynet.be}
\@namedef{freecol-developers.mbox_196}{3CA9D6C7.38AB98B3\%40swissonline.ch}
\@namedef{freecol-developers.mbox_197}{000201c1da65$501a7db0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_198}{3CA9EDBA.3080602\%40easynet.be}
\@namedef{freecol-developers.mbox_199}{004301c1da9c$e525d620$01a97c35\%40DURON800}
\@namedef{freecol-developers.mbox_200}{Pine.SOL.4.30.0204032045001.8459-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_204}{20020404064655.11672.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_205}{3CABFAAA.10004\%40easynet.be}
\@namedef{freecol-developers.mbox_208}{20020404091056.11854.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_210}{3CAC00FB.3060905\%40easynet.be}
\@namedef{freecol-developers.mbox_215}{3CB346E0.4020806\%40easynet.be}
\@namedef{freecol-developers.mbox_201}{Pine.SOL.4.30.0204031109330.21401-100000\%40my.nada.kth.se}
\@namedef{freecol-developers.mbox_202}{3CAAD3BD.10005\%40easynet.be}
\@namedef{freecol-developers.mbox_203}{20020404064339.11656.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_206}{000201c1db35$48e1c5f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_207}{3CAC0E93.6060001\%40easynet.be}
\@namedef{freecol-developers.mbox_209}{OFEA2E0FC4.2368A75C-ON03256B91.0046A671\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_211}{3CAC90B4.5030008\%40easynet.be}
\@namedef{freecol-developers.mbox_212}{OFF2661EF3.5E501F96-ON03256B92.0047180D\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_213}{20020405135301.12935.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_214}{OF7D4E91F4.CA87DB8B-ON03256B92.004C7A12\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_216}{000001c1e006$a0d035f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_217}{3CB40186.2050001\%40easynet.be}
\@namedef{freecol-developers.mbox_218}{20020410082758.1798.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_219}{3CB42672.6080207\%40easynet.be}
\@namedef{freecol-developers.mbox_220}{Pine.SOL.4.30.0204101155100.6309-100000\%40eridanus.nada.kth.se}
\@namedef{freecol-developers.mbox_221}{3CB5DFA8.4010805\%40easynet.be}
\@namedef{freecol-developers.mbox_222}{3CB6C18D.50400\%40easynet.be}
\@namedef{freecol-developers.mbox_223}{3CB6E3B9.8000406\%40easynet.be}
\@namedef{freecol-developers.mbox_224}{OF6AA307C6.DF5A62BF-ON03256B99.00487E40\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_225}{3CB6FCAE.5010900\%40easynet.be}
\@namedef{freecol-developers.mbox_226}{3CB72441.4080504\%40easynet.be}
\@namedef{freecol-developers.mbox_227}{OF46B86432.52A9F420-ON03256B99.005F51AB\%40uy.ibm.com}
\@namedef{freecol-developers.mbox_228}{3CB7FFC6.1010809\%40easynet.be}
\@namedef{freecol-developers.mbox_229}{3CB9992A.2010401\%40easynet.be}
\@namedef{freecol-developers.mbox_230}{000301c1e3eb$87c18170$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_231}{20020415053417.5206.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_232}{3CC45AA9.6030704\%40easynet.be}
\@namedef{freecol-developers.mbox_233}{3CC58417.39C33E62\%40swissonline.ch}
\@namedef{freecol-developers.mbox_234}{3CD83475.1030909\%40easynet.be}
\@namedef{freecol-developers.mbox_235}{3CEC0327.1040604\%40easynet.be}
\@namedef{freecol-developers.mbox_236}{3CF0FA6A.9030305\%40easynet.be}
\@namedef{freecol-developers.mbox_237}{3CF7E776.421329DE\%40swissonline.ch}
\@namedef{freecol-developers.mbox_238}{3D08E729.65C38C1F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_242}{3D0B2E29.3000609\%40easynet.be}
\@namedef{freecol-developers.mbox_239}{000001c2130c$555a45f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_240}{3D09122F.FCF795E3\%40swissonline.ch}
\@namedef{freecol-developers.mbox_243}{3D0B326C.3050002\%40easynet.be}
\@namedef{freecol-developers.mbox_241}{20020613223424.28855.qmail\%40uwdvg002.cms.usa.net}
\@namedef{freecol-developers.mbox_244}{3D0CA005.6FEAA3B8\%40swissonline.ch}
\@namedef{freecol-developers.mbox_245}{3D0DB4FE.7010805\%40easynet.be}
\@namedef{freecol-developers.mbox_246}{3D137525.2A428FEA\%40swissonline.ch}
\@namedef{freecol-developers.mbox_247}{3D13A2BB.A5E8757F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_248}{Pine.SOL.4.30.0206222207110.6018-100000\%40tjatte.nada.kth.se}
\@namedef{freecol-developers.mbox_250}{3D15BCB8.3020304\%40easynet.be}
\@namedef{freecol-developers.mbox_249}{000201c21a6d$7b0e08f0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_251}{3D1E02FA.F4DC1B25\%40swissonline.ch}
\@namedef{freecol-developers.mbox_252}{3D1F414A.1A6FC00E\%40swissonline.ch}
\@namedef{freecol-developers.mbox_253}{3D1F7337.7E53F16C\%40swissonline.ch}
\@namedef{freecol-developers.mbox_254}{3D285052.3E6D4149\%40swissonline.ch}
\@namedef{freecol-developers.mbox_255}{3D2ED585.8010003\%40easynet.be}
\@namedef{freecol-developers.mbox_256}{3D307C93.3AD66F3F\%40swissonline.ch}
\@namedef{freecol-developers.mbox_257}{3D36DA78.8010700\%40easynet.be}
\@namedef{freecol-developers.mbox_258}{3D64E63C.70905\%40easynet.be}
\@namedef{freecol-developers.mbox_259}{001101c24a49$e4bf8560$e52f4c42\%40roosserver}
\@namedef{freecol-developers.mbox_260}{3D91F601.2030400\%40easynet.be}
\@namedef{freecol-developers.mbox_261}{3D958D31.9080705\%40easynet.be}
\@namedef{freecol-developers.mbox_262}{3DC16971.9000401\%40easynet.be}
\@namedef{freecol-developers.mbox_263}{3DC94AE3.3060106\%40easynet.be}
\@namedef{freecol-developers.mbox_264}{3DEE0EBD.7050607\%40easynet.be}
\@namedef{freecol-developers.mbox_265}{Pine.SOL.4.30.0212051620370.20756-100000\%40knatte.nada.kth.se}
\@namedef{freecol-developers.mbox_266}{3DEFA137.9020200\%40easynet.be}
\@namedef{freecol-developers.mbox_267}{Pine.SOL.4.30.0212131712520.16718-100000\%40fnatte.nada.kth.se}
\@namedef{freecol-developers.mbox_268}{3DFA2763.2030902\%40easynet.be}
\@namedef{freecol-developers.mbox_269}{3E0A1CF2.1010104\%40easynet.be}
\@namedef{freecol-developers.mbox_270}{3E1445C5.8030905\%40easynet.be}
\@namedef{freecol-developers.mbox_271}{3E1B23F7.3080604\%40easynet.be}
\@namedef{freecol-developers.mbox_272}{E18WwPi-0005Ii-00\%40mars.green}
\@namedef{freecol-developers.mbox_273}{3E1ECBA5.8010500\%40easynet.be}
\@namedef{freecol-developers.mbox_274}{Pine.LNX.4.44.0301100954170.1464-200000\%40home.net}
\@namedef{freecol-developers.mbox_277}{3E1F0F5A.60901\%40easynet.be}
\@namedef{freecol-developers.mbox_275}{Pine.LNX.4.44.0301100957580.1469-100000\%40home.net}
\@namedef{freecol-developers.mbox_278}{3E1F1469.9070904\%40easynet.be}
\@namedef{freecol-developers.mbox_276}{Pine.LNX.4.44.0301101003400.1473-200000\%40home.net}
\@namedef{freecol-developers.mbox_279}{3E20149F.90508\%40easynet.be}
\@namedef{freecol-developers.mbox_280}{3E201AB4.6050409\%40easynet.be}
\@namedef{freecol-developers.mbox_281}{000401c2b9ab$f00e4b50$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_282}{3E207969.4050403\%40easynet.be}
\@namedef{freecol-developers.mbox_283}{001001c2ba16$3462c410$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_284}{3E2138F0.9070901\%40easynet.be}
\@namedef{freecol-developers.mbox_285}{001301c2ba20$1f3fa620$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_286}{3E22C463.9030505\%40easynet.be}
\@namedef{freecol-developers.mbox_287}{20030113152516.19794.qmail\%40bastion.codemint.com}
\@namedef{freecol-developers.mbox_288}{3E2406BC.8080708\%40easynet.be}
\@namedef{freecol-developers.mbox_289}{Pine.LNX.4.44.0301140904200.457-100000\%40home.net}
\@namedef{freecol-developers.mbox_290}{Pine.LNX.4.44.0301150847360.606-100000\%40home.net}
\@namedef{freecol-developers.mbox_291}{3E25882E.9050008\%40easynet.be}
\@namedef{freecol-developers.mbox_292}{3E25AF12.50508\%40easynet.be}
\@namedef{freecol-developers.mbox_293}{3E2690FA.9060505\%40easynet.be}
\@namedef{freecol-developers.mbox_294}{3E26CFA7.2070001\%40easynet.be}
\@namedef{freecol-developers.mbox_295}{3E295CD1.8060400\%40easynet.be}
\@namedef{freecol-developers.mbox_296}{1043001391.14424.3.camel\%40localhost.cox-internet.com}
\@namedef{freecol-developers.mbox_297}{3E2B042A.6020605\%40easynet.be}
\@namedef{freecol-developers.mbox_298}{Pine.LNX.4.44.0301191601290.834-100000\%40home.net}
\@namedef{freecol-developers.mbox_299}{Pine.LNX.4.44.0301201556530.383-100000\%40home.net}
\@namedef{freecol-developers.mbox_300}{3E2C9044.4070209\%40easynet.be}
\@namedef{freecol-developers.mbox_301}{Pine.LNX.4.44.0301231058370.551-100000\%40home.net}
\@namedef{freecol-developers.mbox_302}{3E302BFA.2030000\%40easynet.be}
\@namedef{freecol-developers.mbox_303}{3E3030A1.9060101\%40easynet.be}
\@namedef{freecol-developers.mbox_304}{3E33DAD5.2030803\%40easynet.be}
\@namedef{freecol-developers.mbox_305}{3E342D5E.4050807\%40easynet.be}
\@namedef{freecol-developers.mbox_306}{3E36EDF0.20802\%40seanbaby.com}
\@namedef{freecol-developers.mbox_307}{3E37853B.2000001\%40easynet.be}
\@namedef{freecol-developers.mbox_308}{3E37BBC3.4040300\%40easynet.be}
\@namedef{freecol-developers.mbox_309}{3E37FCA1.5010306\%40easynet.be}
\@namedef{freecol-developers.mbox_310}{E18e0bN-0001Xt-00\%40mars.green}
\@namedef{freecol-developers.mbox_311}{3E3A052A.1060200\%40seanbaby.com}
\@namedef{freecol-developers.mbox_312}{3E3A3F35.4070806\%40easynet.be}
\@namedef{freecol-developers.mbox_313}{3E3CA1FF.8010508\%40seanbaby.com}
\@namedef{freecol-developers.mbox_314}{3E3CE7D5.3050407\%40easynet.be}
\@namedef{freecol-developers.mbox_315}{3E3E4C55.8090806\%40easynet.be}
\@namedef{freecol-developers.mbox_316}{3E40F0D7.8080302\%40easynet.be}
\@namedef{freecol-developers.mbox_317}{Pine.LNX.4.44.0302050740190.597-100000\%40home.net}
\@namedef{freecol-developers.mbox_318}{3E412927.4030905\%40easynet.be}
\@namedef{freecol-developers.mbox_319}{3E4401E5.4010701\%40easynet.be}
\@namedef{freecol-developers.mbox_320}{3E44D37C.6070004\%40easynet.be}
\@namedef{freecol-developers.mbox_321}{3E48D52E.4060503\%40easynet.be}
\@namedef{freecol-developers.mbox_322}{3E4A0EB3.4080603\%40easynet.be}
\@namedef{freecol-developers.mbox_323}{200302171128.53504.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_324}{200302181910.38526.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_325}{200302190057.AA55968390\%40seanbaby.com}
\@namedef{freecol-developers.mbox_326}{Pine.LNX.4.44.0302190809350.853-100000\%40home.net}
\@namedef{freecol-developers.mbox_327}{200302201122.38302.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_328}{3E5682F2.8040301\%40easynet.be}
\@namedef{freecol-developers.mbox_329}{3E589E88.1090503\%40easynet.be}
\@namedef{freecol-developers.mbox_330}{3E5A2D54.6000105\%40easynet.be}
\@namedef{freecol-developers.mbox_331}{3E5CE22C.20505\%40easynet.be}
\@namedef{freecol-developers.mbox_332}{20030227092825.78561821F\%40neptune.green}
\@namedef{freecol-developers.mbox_333}{3E5DEAF5.1000908\%40easynet.be}
\@namedef{freecol-developers.mbox_334}{Pine.LNX.4.44.0302280809250.681-100000\%40home.net}
\@namedef{freecol-developers.mbox_337}{3E5FA70C.7050508\%40easynet.be}
\@namedef{freecol-developers.mbox_335}{000401c2df41$ead04060$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_336}{3E5FA56B.5090109\%40easynet.be}
\@namedef{freecol-developers.mbox_338}{002801c2dfe0$bca39260$3624d943\%40comp}
\@namedef{freecol-developers.mbox_339}{LOENLNCGFBLNMGOKOMEFIEOFCEAA.stephen\%40fidorama.com}
\@namedef{freecol-developers.mbox_340}{3E61DA46.7090802\%40easynet.be}
\@namedef{freecol-developers.mbox_341}{3E623021.5000307\%40seanbaby.com}
\@namedef{freecol-developers.mbox_342}{LOENLNCGFBLNMGOKOMEFEEOJCEAA.stephen\%40fidorama.com}
\@namedef{freecol-developers.mbox_343}{3E6318E6.8040505\%40easynet.be}
\@namedef{freecol-developers.mbox_344}{LOENLNCGFBLNMGOKOMEFGEOLCEAA.stephen\%40fidorama.com}
\@namedef{freecol-developers.mbox_345}{3E636BA0.20901\%40easynet.be}
\@namedef{freecol-developers.mbox_346}{LOENLNCGFBLNMGOKOMEFIEOMCEAA.stephen\%40fidorama.com}
\@namedef{freecol-developers.mbox_347}{3E6379E6.7040403\%40easynet.be}
\@namedef{freecol-developers.mbox_348}{3E63A7A1.3010403\%40seanbaby.com}
\@namedef{freecol-developers.mbox_349}{3E6470B7.8040904\%40easynet.be}
\@namedef{freecol-developers.mbox_350}{3E64DA96.6080605\%40easynet.be}
\@namedef{freecol-developers.mbox_351}{000001c2e342$4052f380$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_352}{3E66460A.1050700\%40easynet.be}
\@namedef{freecol-developers.mbox_353}{LOENLNCGFBLNMGOKOMEFEEPKCEAA.stephen\%40fidorama.com}
\@namedef{freecol-developers.mbox_355}{3E6719ED.1040202\%40easynet.be}
\@namedef{freecol-developers.mbox_354}{000401c2e35e$91bf4ea0$0600a8c0\%40EBE2K}
\@namedef{freecol-developers.mbox_356}{699HcFNcS8240S03.1046955764\%40uwdvg003.cms.usa.net}
\@namedef{freecol-developers.mbox_357}{3E6E701B.6020208\%40seanbaby.com}
\@namedef{freecol-developers.mbox_358}{3E745B11.2010509\%40easynet.be}
\@namedef{freecol-developers.mbox_359}{3E76EF5A.9030502\%40easynet.be}
\@namedef{freecol-developers.mbox_360}{3E785421.4010208\%40easynet.be}
\@namedef{freecol-developers.mbox_361}{3E817742.2020006\%40easynet.be}
\@namedef{freecol-developers.mbox_362}{3E8372E1.8050202\%40randito.com}
\@namedef{freecol-developers.mbox_363}{3E840A52.6050303\%40easynet.be}
\@namedef{freecol-developers.mbox_364}{3E89ACEE.8080305\%40easynet.be}
\@namedef{freecol-developers.mbox_365}{3E91DF66.1060205\%40seanbaby.com}
\@namedef{freecol-developers.mbox_366}{3E927BBD.1040209\%40easynet.be}
\@namedef{freecol-developers.mbox_367}{3E937755.7050303\%40seanbaby.com}
\@namedef{freecol-developers.mbox_368}{3E947C52.8000409\%40seanbaby.com}
\@namedef{freecol-developers.mbox_369}{3E9533F9.1060509\%40easynet.be}
\@namedef{freecol-developers.mbox_370}{3EAA5DE4.20001\%40easynet.be}
\@namedef{freecol-developers.mbox_371}{20030504204206.Q93650-100000\%40byron.fachschaften.uni-muenchen.de}
\@namedef{freecol-developers.mbox_373}{3EB64814.9030704\%40easynet.be}
\@namedef{freecol-developers.mbox_374}{20030505205622.J5621-100000\%40byron.fachschaften.uni-muenchen.de}
\@namedef{freecol-developers.mbox_376}{3EBA9E56.8000508\%40seanbaby.com}
\@namedef{freecol-developers.mbox_377}{3EBB5881.6040108\%40easynet.be}
\@namedef{freecol-developers.mbox_372}{20030505011431.P95398-100000\%40byron.fachschaften.uni-muenchen.de}
\@namedef{freecol-developers.mbox_375}{20030507000120.U19045-100000\%40byron.fachschaften.uni-muenchen.de}
\@namedef{freecol-developers.mbox_378}{3EC91CAC.1050506\%40easynet.be}
\@namedef{freecol-developers.mbox_379}{Pine.LNX.4.21.0306112055040.25133-100000\%40miranda.org}
\@namedef{freecol-developers.mbox_380}{Pine.LNX.4.21.0306231501430.4030-100000\%40miranda.org}
\@namedef{freecol-developers.mbox_381}{200307021746.h62HkHQ05987\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_382}{3F0336C0.2070009\%40easynet.be}
\@namedef{freecol-developers.mbox_383}{3F03C94A.9080908\%40seanbaby.com}
\@namedef{freecol-developers.mbox_410}{200309261617.50015.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_411}{3F76B55F.9030404\%40easynet.be}
\@namedef{freecol-developers.mbox_384}{200307171719.h6HHJwQ20317\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_385}{3F166400.6070301\%40easynet.be}
\@namedef{freecol-developers.mbox_386}{3F175FC6.1010002\%40murtos.com}
\@namedef{freecol-developers.mbox_388}{3F183299.8010000\%40easynet.be}
\@namedef{freecol-developers.mbox_387}{E19dLkJ-0008DH-00\%40symonds.net}
\@namedef{freecol-developers.mbox_389}{200307221725.h6MHPmQ01410\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_390}{3F1F0F21.9080203\%40murtos.com}
\@namedef{freecol-developers.mbox_391}{3F1F3332.7000800\%40seanbaby.com}
\@namedef{freecol-developers.mbox_392}{3F1F4571.1090700\%40seanbaby.com}
\@namedef{freecol-developers.mbox_393}{E19fZlC-00058o-00\%40symonds.net}
\@namedef{freecol-developers.mbox_395}{3F1FEAF0.1030602\%40murtos.com}
\@namedef{freecol-developers.mbox_396}{3F1F9854.5020801\%40easynet.be}
\@namedef{freecol-developers.mbox_394}{200307241011.h6OABsQ09015\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_397}{3F204B98.1030607\%40murtos.com}
\@namedef{freecol-developers.mbox_398}{3F216B7F.3020308\%40easynet.be}
\@namedef{freecol-developers.mbox_399}{200307280852.h6S8q9Q08207\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_400}{200307282324.3385.tolf.ifi.uio.no\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_401}{3F25C079.6000306\%40seanbaby.com}
\@namedef{freecol-developers.mbox_402}{E19hOHk-0001Mn-00\%40mars.green}
\@namedef{freecol-developers.mbox_404}{3F26A202.8090007\%40murtos.com}
\@namedef{freecol-developers.mbox_405}{3F26E052.2030601\%40murtos.com}
\@namedef{freecol-developers.mbox_403}{200307291317.h6TDHMQ12873\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_406}{200307301635.h6UGZVQ11310\%40mailgate5.cinetic.de}
\@namedef{freecol-developers.mbox_407}{200308051515.4620.ellifu.ifi.uio.no\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_408}{20030821082658.23956.qmail\%40webmail31.rediffmail.com}
\@namedef{freecol-developers.mbox_409}{20030821082658.23956.qmail\%40webmail31.rediffmail.com}
\@namedef{freecol-developers.mbox_412}{Pine.LNX.4.33.0310091308390.18562-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_413}{200310100857.09045.neil\%40dist.ro}
\@namedef{freecol-developers.mbox_415}{3F86DB9E.8090804\%40easynet.be}
\@namedef{freecol-developers.mbox_414}{Pine.LNX.4.33.0310100208490.1384-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_416}{Pine.LNX.4.33.0310100931490.2150-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_417}{Pine.LNX.4.33.0310121542460.13282-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_418}{3F8AD9B1.6080402\%40easynet.be}
\@namedef{freecol-developers.mbox_419}{Pine.LNX.4.33.0310131056480.18321-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_420}{Pine.LNX.4.33.0310200919070.13263-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_421}{200312102023.9957.tva.ifi.uio.no\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_422}{Pine.LNX.4.33.0312211601000.17294-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_423}{3FEEE4E3.6070904\%40easynet.be}
\@namedef{freecol-developers.mbox_424}{Pine.LNX.4.33.0312281209420.9774-100000\%40osdlab.pdx.osdl.net}
\@namedef{freecol-developers.mbox_425}{3FF01681.7050309\%40easynet.be}
\@namedef{freecol-developers.mbox_426}{Law15-F121RA0gbWC3S00037bde\%40hotmail.com}
\@namedef{freecol-developers.mbox_427}{200402061046.14404.niu.ifi.uio.no\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_428}{E1AqZlT-0000um-00\%40ulrik.uio.no}
\@namedef{freecol-developers.mbox_429}{404F66B5.8010705\%40easynet.be}
\@namedef{freecol-developers.mbox_430}{E1AqeL1-0000uU-00\%40ulrik.uio.no}
\@namedef{freecol-developers.mbox_431}{200402140850.13989.tolf.ifi.uio.no\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_432}{400D4153.5030902\%40easynet.be}
\@namedef{freecol-developers.mbox_433}{200402211452.00858.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_434}{40187178.9060008\%40easynet.be}
\@namedef{freecol-developers.mbox_435}{E1B2sKe-0004AM-7C\%40sc8-sf-mx2.sourceforge.net}
\@namedef{freecol-developers.mbox_436}{200403152255.16484.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_437}{40566DF6.3080703\%40murtos.com}
\@namedef{freecol-developers.mbox_438}{200403161029.06018.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_439}{4057DB98.1070902\%40murtos.com}
\@namedef{freecol-developers.mbox_440}{200403171448.31663.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_441}{200404042336.33663.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_442}{200404141344.05839.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_443}{407B485C.1070403\%40easynet.be}
\@namedef{freecol-developers.mbox_444}{200404181014.48604.neil\%40dist.ro}
\@namedef{freecol-developers.mbox_445}{408263E4.5080406\%40easynet.be}
\@namedef{freecol-developers.mbox_446}{200404201207.32901.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_447}{408888BF.5000502\%40shaw.ca}
\@namedef{freecol-developers.mbox_449}{200404231220.34832.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_448}{200404231146.51479.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_450}{40899090.2080108\%40shaw.ca}
\@namedef{freecol-developers.mbox_451}{200404240148.19459.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_452}{408A1CDA.8050300\%40easynet.be}
\@namedef{freecol-developers.mbox_453}{408B0D5A.50704\%40shaw.ca}
\@namedef{freecol-developers.mbox_454}{20040426001016.14853.qmail\%40web60604.mail.yahoo.com}
\@namedef{freecol-developers.mbox_455}{408D45D3.8010107\%40easynet.be}
\@namedef{freecol-developers.mbox_456}{200404271711.25577.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_457}{406B01E8.2060705\%40easynet.be}
\@namedef{freecol-developers.mbox_458}{4093CC8A.2030908\%40shaw.ca}
\@namedef{freecol-developers.mbox_459}{408FF668.20102\%40easynet.be}
\@namedef{freecol-developers.mbox_460}{40943FDA.1010408\%40shaw.ca}
\@namedef{freecol-developers.mbox_461}{409504DD.60303\%40shaw.ca}
\@namedef{freecol-developers.mbox_462}{40A17D48.20206\%40shaw.ca}
\@namedef{freecol-developers.mbox_463}{200405141403.21797.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_464}{000901c439e0$1ded8760$0100a8c0\%40hallnetcolgc}
\@namedef{freecol-developers.mbox_465}{40A52D31.1070504\%40shaw.ca}
\@namedef{freecol-developers.mbox_466}{200407081316.15790.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_468}{40EEE0B8.9080806\%40easynet.be}
\@namedef{freecol-developers.mbox_470}{40F0A7D5.1090907\%40shaw.ca}
\@namedef{freecol-developers.mbox_483}{4103A49A.20806\%40easynet.be}
\@namedef{freecol-developers.mbox_467}{200407090025.45143.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_469}{40F0A689.9060101\%40shaw.ca}
\@namedef{freecol-developers.mbox_471}{200407122020.29470.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_472}{40F2FC69.5000808\%40easynet.be}
\@namedef{freecol-developers.mbox_474}{200407141534.51142.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_475}{40F578EA.6070001\%40easynet.be}
\@namedef{freecol-developers.mbox_473}{200407141357.32209.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_476}{40F5A02F.3010705\%40murtos.com}
\@namedef{freecol-developers.mbox_479}{40F6E678.4020500\%40easynet.be}
\@namedef{freecol-developers.mbox_477}{40F5D97D.4020901\%40murtos.com}
\@namedef{freecol-developers.mbox_478}{200407151058.11909.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_480}{200407162346.25925.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_481}{41026D33.7030100\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_482}{4103A00F.40808\%40easynet.be}
\@namedef{freecol-developers.mbox_484}{4103AA5E.4070705\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_485}{200407251644.34180.unclouded\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_487}{4103D7AF.1000307\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_486}{4103D723.6060301\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_488}{410A4B88.80007\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_489}{410A8AAA.1050302\%40easynet.be}
\@namedef{freecol-developers.mbox_490}{410B687A.6080108\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_491}{410B8688.6000308\%40easynet.be}
\@namedef{freecol-developers.mbox_492}{410B6E38.4010705\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_493}{410CFD87.3000107\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_494}{410D1BAB.3090901\%40easynet.be}
\@namedef{freecol-developers.mbox_495}{410D5344.3080500\%40easynet.be}
\@namedef{freecol-developers.mbox_496}{410E4EE4.4050801\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_497}{410F5B80.7020708\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_498}{410FD094.2020400\%40easynet.be}
\@namedef{freecol-developers.mbox_499}{200408041059.55251.unclouded\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_500}{4110F08A.6010605\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_501}{200408041740.18424.unclouded\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_502}{41112F00.5080102\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_503}{41124047.9050509\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_504}{4112768A.5030700\%40easynet.be}
\@namedef{freecol-developers.mbox_506}{411352EC.5020402\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_508}{4113FD31.3030509\%40easynet.be}
\@namedef{freecol-developers.mbox_509}{200408070034.36771.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_512}{4114BC90.9000302\%40easynet.be}
\@namedef{freecol-developers.mbox_514}{4114AA3D.2000608\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_513}{4114A7DA.6060907\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_515}{200408091618.10227.unclouded\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_505}{20040806031401.36573.qmail\%40web60501.mail.yahoo.com}
\@namedef{freecol-developers.mbox_507}{4113F498.8070608\%40easynet.be}
\@namedef{freecol-developers.mbox_510}{200408070055.50560.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_511}{4114B997.7050204\%40easynet.be}
\@namedef{freecol-developers.mbox_516}{4117CA85.4030307\%40easynet.be}
\@namedef{freecol-developers.mbox_517}{4118994F.5020209\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_518}{41190B85.6050902\%40easynet.be}
\@namedef{freecol-developers.mbox_519}{41260B87.5070703\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_520}{200408202023.50144.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_521}{200408271021.05431.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_522}{200408271200.55314.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_523}{200408271247.28052.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_524}{200408271308.43732.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_525}{200409011558.00376.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_526}{200409021809.56600.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_527}{200409022236.05138.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_529}{200409031802.31581.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_528}{41389270.3010202\%40gmx.de}
\@namedef{freecol-developers.mbox_530}{413A3645.8030901\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_531}{413C9D60.9040409\%40gmx.de}
\@namedef{freecol-developers.mbox_532}{413EA84E.8080302\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_533}{413FF8C4.9070506\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_535}{200409091351.18521.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_534}{200409091312.37800.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_536}{41404F62.9050502\%40gmx.de}
\@namedef{freecol-developers.mbox_546}{414562E9.7020206\%40gmx.de}
\@namedef{freecol-developers.mbox_547}{200409131131.59807.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_537}{41431F2E.1040102\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_538}{200409121035.42611.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_539}{414418C8.5080302\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_541}{200409121159.01161.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_542}{414425C5.6090004\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_540}{200409121148.47351.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_551}{200409182018.54772.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_555}{414DA628.7000204\%40murtos.com}
\@namedef{freecol-developers.mbox_557}{200409191914.39903.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_543}{200409121507.14342.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_544}{200409121540.43268.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_545}{41445388.9040005\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_548}{a06100500bd6d021b7e0e\%40[10.0.1.202]}
\@namedef{freecol-developers.mbox_549}{E1C8cEJ-0008V8-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_550}{E1C8d8R-0006Gv-00\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_552}{200409191550.35950.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_553}{414D91B9.20207\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_554}{200409191642.03070.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_556}{414DA802.4060909\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_558}{200409201425.53483.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_559}{200409201756.08991.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_560}{414EFFDC.9000002\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_561}{E1CALQI-0007wh-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_562}{41536EC3.7080700\%40murtos.com}
\@namedef{freecol-developers.mbox_566}{200409241115.47149.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_567}{415514B4.3000808\%40murtos.com}
\@namedef{freecol-developers.mbox_568}{4155B4AE.8040500\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_563}{41538F7F.9050001\%40murtos.com}
\@namedef{freecol-developers.mbox_564}{200409240907.19943.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_565}{E1CAeAx-0006jL-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_569}{4156303A.9070501\%40murtos.com}
\@namedef{freecol-developers.mbox_571}{200409261127.38408.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_570}{E1CBQYQ-0005Be-00\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_572}{200409261156.10754.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_573}{415732E4.7050401\%40murtos.com}
\@namedef{freecol-developers.mbox_575}{200409271835.25592.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_574}{4157343C.7010809\%40murtos.com}
\@namedef{freecol-developers.mbox_576}{20040930050648.75042.qmail\%40web60604.mail.yahoo.com}
\@namedef{freecol-developers.mbox_620}{41681820.1010009\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_577}{20040930051158.79925.qmail\%40web60607.mail.yahoo.com}
\@namedef{freecol-developers.mbox_578}{20040930052557.81743.qmail\%40web60607.mail.yahoo.com}
\@namedef{freecol-developers.mbox_579}{200409301259.24344.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_580}{20041001100903.GA1095\%40inutil.org}
\@namedef{freecol-developers.mbox_581}{200410011956.35198.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_587}{20041003150633.GA8145\%40informatik.uni-bremen.de}
\@namedef{freecol-developers.mbox_588}{200410031907.25791.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_582}{200410020003.42457.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_583}{200410020005.23848.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_595}{200410041225.09705.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_584}{E1CDWct-0005LC-00\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_585}{200410022024.23586.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_586}{E1CE4va-000479-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_589}{200410032150.55015.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_596}{200410041255.02964.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_590}{E1CE4l8-00067y-00\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_591}{4160AF1E.2070109\%40murtos.com}
\@namedef{freecol-developers.mbox_598}{200410041438.18012.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_601}{41620CF7.8040001\%40murtos.com}
\@namedef{freecol-developers.mbox_602}{200410050829.30644.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_592}{4160BFF1.4040709\%40murtos.com}
\@namedef{freecol-developers.mbox_593}{4160C189.7020903\%40murtos.com}
\@namedef{freecol-developers.mbox_597}{200410041304.05536.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_594}{E1CEPSg-000811-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_599}{416165F7.3040404\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_600}{200410042053.31057.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_603}{4162B05C.80303\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_604}{200410051747.56640.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_605}{E1CEwP3-0004YL-00\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_606}{E1CF1wb-0000vP-00\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_607}{E1CF6je-0006pY-00\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_608}{E1CF6mH-00055Z-00\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_609}{200410081807.23880.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_613}{200410090052.06011.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_618}{4167E9CC.5010903\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_610}{E1CFx4P-00077U-00\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_611}{4166E43A.4090609\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_612}{200410082253.53933.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_614}{41672137.30904\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_615}{200410091115.00447.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_616}{200410091128.51947.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_617}{4167CC6D.5020502\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_619}{4167EB66.50202\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_621}{41694E0B.4060307\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_622}{200410101714.12989.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_624}{416953D9.5070109\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_625}{200410101739.55937.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_626}{200410101746.52340.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_623}{200410101714.31522.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_627}{4169622F.5050406\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_628}{200410101840.04528.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_629}{41696D44.6090200\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_636}{200410110008.48714.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_643}{200410111820.37765.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_647}{416B7D34.20002\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_659}{416CD45E.8020703\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_660}{200410131011.37937.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_668}{41712807.1020601\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_672}{200410181242.14212.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_630}{41696ED1.7010406\%40murtos.com}
\@namedef{freecol-developers.mbox_631}{1097436029.1048.61.camel\%40verheyens}
\@namedef{freecol-developers.mbox_632}{4169A433.5090605\%40murtos.com}
\@namedef{freecol-developers.mbox_635}{200410102358.10669.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_633}{4169A7CA.8060709\%40murtos.com}
\@namedef{freecol-developers.mbox_634}{200410102349.41209.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_641}{200410111801.53958.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_637}{416A0B4A.4000002\%40murtos.com}
\@namedef{freecol-developers.mbox_640}{200410111158.31498.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_644}{200410111921.41601.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_648}{416B7DB8.6000007\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_650}{200410121107.45589.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_654}{200410122103.38699.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_655}{200410122207.30676.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_658}{416C7D74.1000600\%40murtos.com}
\@namedef{freecol-developers.mbox_662}{200410131844.51205.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_661}{200410131820.57055.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_651}{200410120055.07120.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_638}{E1CGsUx-0002zz-7O\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_639}{E1CGtzT-0007hR-R6\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_642}{E1CH2oX-0004AO-NT\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_645}{200410112358.27233.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_646}{416B395A.6040705\%40murtos.com}
\@namedef{freecol-developers.mbox_649}{416B8184.6050108\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_652}{200410121457.47736.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_663}{200410131932.00209.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_653}{200410122032.27566.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_656}{1097612913.2586.5.camel\%40verheyens}
\@namedef{freecol-developers.mbox_657}{200410122239.16535.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_664}{E1CI6TP-00029d-64\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_665}{E1CI6Wv-000555-BG\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_666}{002701c4b2eb$db291d60$220110ac\%40DOUGNOTE4}
\@namedef{freecol-developers.mbox_667}{BAY12-F1Hiu3fQtYdVz00004381\%40hotmail.com}
\@namedef{freecol-developers.mbox_669}{E1CIpay-0002hL-Vi\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_670}{41713EEC.9060009\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_671}{41735F77.3040503\%40student.ulg.ac.be}
\@namedef{freecol-developers.mbox_673}{200410181801.42425.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_679}{417B7832.9000800\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_674}{200410202012.29178.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_675}{001301c4b82a$92474ce0$0400a8c0\%40DOUGNOTE4}
\@namedef{freecol-developers.mbox_677}{200410221824.43461.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_676}{E1CKzfq-0006zP-Ps\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_678}{E1CL5E9-0008Hp-9O\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_680}{E1CLs2y-0000lm-NP\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_681}{E1CMEny-00082C-W3\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_682}{417DAAC9.4020101\%40murtos.com}
\@namedef{freecol-developers.mbox_683}{200410272112.54453.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_684}{200410291523.24560.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_685}{41838B35.1080308\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_686}{4183A8FE.6050908\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_687}{41843739.3090500\%40horizonwimba.com}
\@namedef{freecol-developers.mbox_688}{4184444A.5020407\%40horizonwimba.com}
\@namedef{freecol-developers.mbox_690}{41860394.1080005\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_689}{017701c4bf19$287413c0$14e5fea9\%40comp}
\@namedef{freecol-developers.mbox_691}{200411011134.53470.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_692}{41863948.7090406\%40murtos.com}
\@namedef{freecol-developers.mbox_696}{4186E3E9.7070809\%40murtos.com}
\@namedef{freecol-developers.mbox_693}{4187A329.1090703\%40gimpel.org}
\@namedef{freecol-developers.mbox_694}{200411021841.52641.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_710}{419F8E21.8010700\%40gimpel.org}
\@namedef{freecol-developers.mbox_711}{200411211217.05582.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_713}{41A1A6F1.3080509\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_695}{BAY12-F1VpJ9AUjui4I0000eb92\%40hotmail.com}
\@namedef{freecol-developers.mbox_697}{E1CQOSQ-0007u9-FL\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_698}{E1CREJd-0001SA-Pl\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_699}{4191E2B6.2050608\%40edward.dyndns.org}
\@namedef{freecol-developers.mbox_700}{20041115210149.SHUI3360.gx6.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_701}{41996DC1.7040401\%40murtos.com}
\@namedef{freecol-developers.mbox_703}{200411161205.37762.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_706}{419AA2DC.2060100\%40murtos.com}
\@namedef{freecol-developers.mbox_702}{4199ADF9.7020709\%40run.montefiore.ulg.ac.be}
\@namedef{freecol-developers.mbox_705}{200411161755.32989.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_707}{200411170224.42901.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_704}{20041116151859.VYJD3360.gx6.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_708}{20041117014240.ZKPO3360.gx6.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_709}{419F1C5F.1000803\%40gimpel.org}
\@namedef{freecol-developers.mbox_712}{200411211223.08101.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_714}{20041124064603.27879.qmail\%40web60505.mail.yahoo.com}
\@namedef{freecol-developers.mbox_715}{E1CY0Qx-0000r8-NX\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_716}{200411271948.30327.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_718}{200411291352.46249.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_720}{200411301942.07499.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_717}{41AA0481.3030501\%40laposte.net}
\@namedef{freecol-developers.mbox_719}{200411291758.33590.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_721}{009101c4d789$5555e340$3031fea9\%40comp}
\@namedef{freecol-developers.mbox_722}{200501131217.01172.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_723}{200501131806.54134.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_724}{200501132100.22346.stiangre\%40ifi.uio.no}
\@namedef{freecol-developers.mbox_725}{E1Cq0sZ-0004eD-Sp\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_726}{200501281840.00836.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_727}{20050129180354.GSDY13012.gx4.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_728}{3171.80.213.138.84.1107033755.squirrel\%4080.213.138.84}
\@namedef{freecol-developers.mbox_729}{E1CvqTk-00005M-02\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_730}{E1Cvr1v-0005rY-8x\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_731}{E1CxmRU-0000Vf-DG\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_732}{E1CyvkI-00018h-E5\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_733}{000e01c50ed0$90dbfd90$0801a8c0\%40Kepler}
\@namedef{freecol-developers.mbox_734}{1327.80.213.138.84.1107985397.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_735}{003701c510b2$9d07e2d0$0801a8c0\%40Kepler}
\@namedef{freecol-developers.mbox_736}{200502121115.28371.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_737}{E1D01o7-0004ca-Et\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_738}{E1D0OyK-0000UL-Nm\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_739}{1578.80.213.198.53.1108672738.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_740}{200503021753.14860.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_741}{1325.80.213.141.87.1109785094.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_742}{E1D8ZwC-0004hS-Sr\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_743}{200503131046.08331.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_744}{dda0131305032311324c29baea\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_745}{200503241904.47709.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_746}{dda01313050325084621a7c6ed\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_747}{200503251938.33171.lwillems\%40easynet.be}
\@namedef{freecol-developers.mbox_748}{E1DIdM3-0008DA-SI\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_749}{E1DNWlf-0003dZ-UN\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_750}{E1DSdlL-00035B-KN\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_751}{E1DSeIc-0004lr-9Y\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_752}{1508.80.213.142.79.1115464354.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_753}{200505071935.41583.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_754}{4290DBDD.8010600\%40hanquier.com}
\@namedef{freecol-developers.mbox_755}{1116797256.11347.5.camel\%40localhost.localdomain}
\@namedef{freecol-developers.mbox_756}{1660.80.213.197.221.1116799433.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_757}{1116803677.11347.21.camel\%40localhost.localdomain}
\@namedef{freecol-developers.mbox_764}{1238.80.213.197.221.1117022543.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_758}{4290CF7C.4050102\%40hanquier.com}
\@namedef{freecol-developers.mbox_759}{20050524161825.YWKJ10638.gx4.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_760}{200505241847.35039.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_761}{200505241919.01755.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_762}{1229.80.213.197.221.1116959087.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_763}{20050525040100.BJRO21147.gx6.fuse.net\%4064BitBadass}
\@namedef{freecol-developers.mbox_765}{E1DbRCs-0002Ea-U5\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_766}{E1Dbij6-0000pt-N7\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_767}{E1Dcfcq-00024N-B9\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_768}{E1Dcs3i-0002hF-7V\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_769}{E1DeRB6-0003Cp-25\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_770}{42A8852D.7050503\%40hanquier.com}
\@namedef{freecol-developers.mbox_771}{E1DgZ3i-0002Fa-LS\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_772}{E1DjKlP-0007cm-3H\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_773}{E1DjKy5-0000wK-4T\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_774}{E1DjLUT-0003jT-I1\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_775}{E1DjMSk-0003pT-DF\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_776}{1578.80.213.137.202.1119389454.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_777}{E1Dl7Sl-0005MM-D4\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_778}{E1DltRR-0007yN-C3\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_779}{E1DlvCX-0003YO-5L\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_780}{E1DlvJ8-00016z-HY\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_781}{E1DmIPP-0007bN-2Y\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_782}{E1Dn40k-00059Q-OX\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_783}{E1Dn3zH-00056o-I5\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_784}{E1Dn442-0005DQ-Gp\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_785}{42C19957.40606\%40hanquier.com}
\@namedef{freecol-developers.mbox_786}{E1DnvHq-0001e5-UU\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_787}{E1DqASK-0005aR-Mx\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_788}{000601c5862f$70dc5540$a8bc2950\%40DJX82G1J}
\@namedef{freecol-developers.mbox_793}{1965.80.213.139.47.1123868599.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_789}{E1E0Nlm-0007n7-Aa\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_790}{42F2357C.3080708\%40gmx.de}
\@namedef{freecol-developers.mbox_794}{3589.80.213.141.130.1123936642.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_795}{42FDF519.7030002\%40gmx.de}
\@namedef{freecol-developers.mbox_796}{1092.80.213.141.130.1123940689.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_791}{E1E1gq8-0002qQ-1k\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_792}{E1E39lS-0005vP-VK\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_797}{42FE040A.6090904\%40triph.de}
\@namedef{freecol-developers.mbox_798}{E1E4stQ-0006Cq-ES\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_799}{E1E4teP-0005qB-Bb\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_800}{E1E4tjY-0005t8-SP\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_801}{E1E4tnW-0005vU-Ik\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_802}{E1E4zLd-0004bR-E7\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_803}{E1E4zem-0004NJ-Cf\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_804}{E1E4zhu-0004Pq-PC\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_805}{E1E4zng-0004Vi-2F\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_806}{E1E4ztB-0004ap-Kz\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_807}{E1E51pV-0005tN-4W\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_808}{E1E51xT-00069c-UP\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_809}{E1E526m-0007D2-JK\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_810}{E1E52Bp-0007PA-G6\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_811}{E1E52F1-0007aO-Go\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_812}{E1E52Ii-0007eD-Qs\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_813}{E1E5Fic-0000SO-DZ\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_814}{E1E5FkO-0000Ul-4R\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_815}{E1E5Fm9-0000XV-OV\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_816}{E1E5HtM-0000Xu-Ue\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_817}{E1E5RaP-0000iB-3O\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_818}{E1E5yec-0000eP-J1\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_819}{50673.80.202.174.94.1124442924.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_820}{200508191850.58481.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_821}{2611.80.213.141.130.1124483641.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_822}{430E0CB4.3030502\%40bfh.ch}
\@namedef{freecol-developers.mbox_834}{40116.129.240.70.199.1127388569.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_823}{E1EANmn-0000uG-Gn\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_824}{431B392C.90506\%40bfh.ch}
\@namedef{freecol-developers.mbox_825}{1899.80.213.199.143.1125947059.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_826}{E1ED4cL-0002NA-Iw\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_827}{E1EDeod-0006VD-P5\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_828}{E1EDets-000779-FD\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_829}{E1EDfOT-0004fh-1i\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_830}{E1EDfbk-0008R5-4B\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_831}{E1EDfmc-0000QQ-BG\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_832}{E1EEWMH-0003YQ-RN\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_833}{E1EFzX1-0000HM-P2\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_835}{E1EJ4jg-0005V6-0x\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_836}{E1EJA6R-0006Yu-Ul\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_837}{E1EKF2e-0000bA-Ix\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_838}{E1EKHAW-0003aq-Rd\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_839}{1245.80.213.143.10.1127916647.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_840}{20051002170435.MEFQ15475.outaamta01.mail.tds.net\%40smtp.tds.net}
\@namedef{freecol-developers.mbox_858}{200510021953.27010.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_841}{20051003094216.SEDH2142.outaamta02.mail.tds.net\%40smtp.tds.net}
\@namedef{freecol-developers.mbox_842}{1598.80.213.140.222.1128335060.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_843}{E1EN7jO-0007kd-KW\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_844}{E1EN7wc-00080K-R1\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_845}{E1EN81o-00087e-AD\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_846}{E1EN8D4-0008Nm-BP\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_847}{E1EN8JC-0008Ux-H7\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_848}{E1EN8L8-00005R-Jm\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_849}{E1EN8VI-0000uc-JW\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_850}{E1EN8fj-0001AO-Ah\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_851}{E1EN8mk-0001K2-Ed\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_852}{E1EN8vQ-0001V3-KU\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_853}{E1EN8zH-0001bN-Sw\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_854}{E1ENYV1-0006qt-AA\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_855}{E1ENfIq-0007Z4-QC\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_856}{E1ENtEB-00056u-8Q\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_857}{707606270510080910t184a6598vb84aaeed61d3c3ae\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_859}{E1EStDz-00053N-Ik\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_860}{E1EUk66-0002rh-Gb\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_861}{E1EYC8h-0001hY-Hg\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_862}{E1EbTAt-0000UL-Uk\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_863}{000001c5e93e$e138fe20$4201a8c0\%40mikepc}
\@namedef{freecol-developers.mbox_864}{200511141935.56050.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_865}{12408.1132053858\%40www45.gmx.net}
\@namedef{freecol-developers.mbox_866}{E1Egqzn-0000sG-V8\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_867}{43908923.204\%40gmx.de}
\@namedef{freecol-developers.mbox_868}{1133550002.25222.31.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_869}{1635.80.213.142.107.1133555754.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_870}{E1Ej9kl-00004u-Ep\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_871}{E1Ej9na-00006J-90\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_872}{PFELJGOLOAENFCLLELIOCEKIEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_876}{42722.129.240.70.211.1133883054.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_873}{PFELJGOLOAENFCLLELIOGEKIEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_881}{48074.129.240.70.211.1133966119.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_874}{PFELJGOLOAENFCLLELIOKEKIEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_877}{42904.129.240.70.211.1133883894.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_875}{PFELJGOLOAENFCLLELIOCELDEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_878}{44016.129.240.70.211.1133888977.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_879}{PFELJGOLOAENFCLLELIOCELMEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_882}{49007.129.240.70.211.1134041146.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_880}{E1EjvUb-0000bg-AV\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_883}{E1EkKRr-0005i7-HT\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_884}{E1EkMJN-0007aH-9G\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_885}{PFELJGOLOAENFCLLELIOOEMOEJAA.Burschik\%40lotto-berlin.de}
\@namedef{freecol-developers.mbox_886}{1134499477.2417.3.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_887}{E1EmHwP-0001Pf-FA\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_888}{E1EmNlL-0001Ll-Ha\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_889}{E1EmSCu-0005Sd-3V\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_890}{43A2D4B4.7020901\%40gmx.de}
\@namedef{freecol-developers.mbox_891}{200512161824.jBGIO1ML032720\%40outmx018.isp.belgacom.be}
\@namedef{freecol-developers.mbox_892}{200512161829.jBGITfgp003333\%40outmx018.isp.belgacom.be}
\@namedef{freecol-developers.mbox_896}{1212.80.213.193.225.1135024523.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_893}{E1EnzJ0-0003Xl-Sp\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_898}{43ABD5F1.8050707\%40gmx.de}
\@namedef{freecol-developers.mbox_900}{200512241252.11492.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_894}{E1EnzL8-0003hO-DC\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_895}{E1EoPko-0006k5-DK\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_897}{E1Eoi5d-0005L7-Kc\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_899}{43ABEB01.9000201\%40gmx.de}
\@namedef{freecol-developers.mbox_926}{36646.129.240.70.206.1137769413.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_901}{43AEA90A.5060507\%40gmx.de}
\@namedef{freecol-developers.mbox_902}{43B69E8B.5070608\%40gmx.de}
\@namedef{freecol-developers.mbox_903}{200601011900.45582.freecol\%40willemsens.org}
\@namedef{freecol-developers.mbox_904}{E1EtQ7j-00054o-Ky\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_905}{E1EujHj-0007gA-6L\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_906}{E1ExyOy-0004by-Cl\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_907}{E1ExydG-0008PU-7S\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_908}{E1Ey02h-0005YM-Ia\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_909}{E1Ey05P-0005ZR-0Q\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_910}{E1Ey07i-0005au-3U\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_911}{E1Ey097-0005bm-TE\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_912}{E1Ey0A6-0005cD-Fk\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_913}{1137308758.12783.14.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_914}{E1EyFV4-0004PV-HP\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_915}{E1EyKAq-0007ry-Tp\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_916}{E1EyPs4-0002VP-1D\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_917}{E1EySev-0008NH-5j\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_918}{E1Eyhcr-000628-TZ\%40sc8-sf-web4.sourceforge.net}
\@namedef{freecol-developers.mbox_919}{E1EynKn-0002rP-T3\%40sc8-sf-web3.sourceforge.net}
\@namedef{freecol-developers.mbox_920}{E1EynYk-0006jo-Ld\%40sc8-sf-web1.sourceforge.net}
\@namedef{freecol-developers.mbox_921}{852230060435076648}
\@namedef{freecol-developers.mbox_922}{E1EzIfj-0002wX-GO\%40sc8-sf-web2.sourceforge.net}
\@namedef{freecol-developers.mbox_923}{1326.80.213.143.41.1137695188.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_924}{1137746186.12114.24.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_925}{35677.129.240.70.206.1137765740.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_928}{43DFB245.1050702\%40gmx.de}
\@namedef{freecol-developers.mbox_929}{1091.80.213.133.247.1138803782.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_934}{1139776910.20674.3.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_935}{1139804557.22946.11.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_927}{3671.80.213.143.41.1138456618.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_930}{54917.129.240.70.71.1139234964.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_931}{200602061836.02764.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_932}{1139260303.28752.11.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_933}{1687.80.213.133.247.1139260961.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_936}{43F86D16.7060709\%40gmx.de}
\@namedef{freecol-developers.mbox_937}{1140391033.30265.3.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_938}{4401E025.5090000\%40gmx.de}
\@namedef{freecol-developers.mbox_939}{4401DF4F.8090400\%40gmx.de}
\@namedef{freecol-developers.mbox_942}{35076.129.240.70.225.1143467563.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_940}{1141980978.5455.6.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_941}{1142104594.16577.11.camel\%40callisto.green}
\@namedef{freecol-developers.mbox_943}{397d46d00604200605ie3d1ee4sec4b2be7da80b85e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_944}{1960.80.213.132.168.1147439564.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_945}{449E47E3.1090306\%40gmx.de}
\@namedef{freecol-developers.mbox_946}{44A00337.2030103\%40gmx.de}
\@namedef{freecol-developers.mbox_947}{200606261819.10398.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_949}{2072.80.213.139.103.1153134676.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_950}{200607171909.57209.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_948}{2020.80.213.139.103.1153133071.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_951}{200607212131.00572.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_952}{2801.80.213.199.62.1153604594.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_953}{200607231231.52360.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_954}{4755.80.213.199.62.1153999321.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_955}{200607271955.30182.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_956}{200608020116.51067.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_957}{200608021826.00096.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_958}{44D0EB69.4040701\%40hanquier.com}
\@namedef{freecol-developers.mbox_959}{200608080057.28050.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_960}{200608091828.15361.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_961}{200608101635.51026.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_962}{200608150027.52479.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_964}{200608152041.01577.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_963}{200608151316.04627.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_965}{200608152046.36954.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_966}{200608170259.05600.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_967}{44E3EE10.6080501\%40gmx.de}
\@namedef{freecol-developers.mbox_968}{200608171123.26369.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_969}{200608171610.57202.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_970}{200608171630.10892.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_971}{200608171653.42541.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_973}{200608171713.11964.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_980}{d311c6a80608171615u7b8f11cfw84260f532f23929c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_981}{200608181351.06343.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_972}{200608171712.09146.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_974}{200608171906.07599.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_975}{1089.80.213.134.22.1155844932.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_976}{000201c6c23d$20f3ccc0$3402a8c0\%4064BitBadass}
\@namedef{freecol-developers.mbox_977}{44E4E4E2.6050102\%40murtos.com}
\@namedef{freecol-developers.mbox_978}{2059.80.213.134.22.1155852344.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_979}{d311c6a80608171612t200fdbe9i8916f15f0a32bb58\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_984}{44E5D79E.1080409\%40murtos.com}
\@namedef{freecol-developers.mbox_985}{2195.80.213.134.22.1155917872.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_982}{200608181411.23647.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_983}{44E5D687.4040402\%40murtos.com}
\@namedef{freecol-developers.mbox_986}{200608182220.16585.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_987}{2787.80.213.134.22.1155935845.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_988}{200608190323.45010.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_989}{1156.80.213.134.22.1155977302.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_990}{44E714B4.4040502\%40gmx.de}
\@namedef{freecol-developers.mbox_999}{44F03438.4040007\%40gmx.de}
\@namedef{freecol-developers.mbox_1000}{200608272042.19275.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1003}{200608280426.44045.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1005}{44F27D26.6090307\%40gmx.de}
\@namedef{freecol-developers.mbox_1006}{200608281705.39553.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_991}{44E94329.3040405\%40gmx.de}
\@namedef{freecol-developers.mbox_992}{200608221345.18615.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_993}{200608221400.57862.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1015}{44F83B28.8020804\%40unizar.es}
\@namedef{freecol-developers.mbox_1016}{43793.129.240.70.67.1157120274.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1017}{44F84538.3030509\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1018}{20060901154516.150260\%40gmx.net}
\@namedef{freecol-developers.mbox_1019}{200609012050.19852.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1026}{200609070004.17511.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1027}{44FFAAD0.3050601\%40gmx.de}
\@namedef{freecol-developers.mbox_1030}{1725.80.213.134.22.1157623321.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1032}{450130AF.2060700\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1031}{200609071957.01652.mark.wagner17\%40gte.net}
\@namedef{freecol-developers.mbox_1033}{4503BE5D.5030301\%40gmx.de}
\@namedef{freecol-developers.mbox_1035}{1533.80.213.143.60.1157964383.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1041}{45057CCC.8020905\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_994}{200608221653.33087.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_995}{003d01c6c608$b9657570$2c306050$\%40de}
\@namedef{freecol-developers.mbox_996}{200608222005.21969.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_997}{200608222108.24333.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_998}{20060823053851.277350\%40gmx.net}
\@namedef{freecol-developers.mbox_1001}{200608280123.48416.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1002}{200608280209.38334.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1004}{200608280501.45573.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1007}{44F32559.7090405\%40hanquier.com}
\@namedef{freecol-developers.mbox_1009}{200608282220.55850.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1008}{200608282149.00526.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1010}{200608290355.09038.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1011}{44F3235D.3070702\%40hanquier.com}
\@namedef{freecol-developers.mbox_1012}{2736.212.97.186.77.1156848329.squirrel\%40correo.ensanjose.net}
\@namedef{freecol-developers.mbox_1013}{44F7D041.5000608\%40gmx.de}
\@namedef{freecol-developers.mbox_1014}{44F7E442.5000408\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1020}{200609031129.28239.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_1021}{44FAA55A.9070102\%40gmx.de}
\@namedef{freecol-developers.mbox_1022}{44FAE2A7.5090901\%40hanquier.com}
\@namedef{freecol-developers.mbox_1023}{200609032138.10652.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1024}{54825.129.240.71.211.1157476452.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1025}{200609052101.51898.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_1028}{19793.80.118.33.228.1157615139.squirrel\%4080.118.33.228}
\@namedef{freecol-developers.mbox_1029}{1472.80.213.134.22.1157618107.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1034}{200609102056.57579.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1038}{450572E0.3010807\%40gmx.de}
\@namedef{freecol-developers.mbox_1036}{2210.80.213.143.60.1157977014.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1037}{4505633C.5020505\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1040}{2709.80.213.143.60.1157986720.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1039}{4505749C.3040307\%40gmx.de}
\@namedef{freecol-developers.mbox_1042}{2773.80.213.143.60.1157987956.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1043}{450581F8.9080000\%40gmx.de}
\@namedef{freecol-developers.mbox_1044}{450582FC.2070708\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1045}{45058AA7.6020402\%40gmx.de}
\@namedef{freecol-developers.mbox_1046}{45058E07.9000300\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1047}{1414.80.213.143.60.1158048703.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1048}{397d46d00609120502k2954d6fevb660248652d35dc9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1049}{4506C3B8.6020803\%40gmx.de}
\@namedef{freecol-developers.mbox_1050}{49527.129.240.71.211.1158074670.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1052}{4506E884.8010404\%40gmx.de}
\@namedef{freecol-developers.mbox_1053}{200609122043.38979.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1051}{50533.129.240.71.211.1158075366.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1054}{41754.129.240.71.217.1158580579.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1055}{451B8C72.8090206\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1056}{200610060012.25332.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1057}{452664D0.7050001\%40gmx.de}
\@namedef{freecol-developers.mbox_1058}{3c8f359e0610151112p63ebf718v719c1121bb3beb74\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1059}{200610162119.30305.lars\%40willemsens.org}
\@namedef{freecol-developers.mbox_1060}{200610280212.36775.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1061}{54869.80.213.142.68.1162025978.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1062}{37957.80.213.140.123.1162512363.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1064}{3c8f359e0611030715kf46e663u2dde561d1a278676\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1065}{200611032019.00876.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1066}{454C3BD9.2060909\%40gmx.de}
\@namedef{freecol-developers.mbox_1067}{37077.80.213.140.123.1162646336.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1068}{d311c6a80611040638h565c9827ke04755b864d3b4cd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1069}{454CB3FE.5050709\%40gmx.de}
\@namedef{freecol-developers.mbox_1071}{200611041754.30571.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1073}{3c8f359e0611051313s38557e83ya6eee9e9d683ef65\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1063}{49842.129.240.153.64.1162561738.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1070}{454CC33F.80203\%40gmx.de}
\@namedef{freecol-developers.mbox_1072}{33796.80.213.140.123.1162671121.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1074}{454EE3AE.6090809\%40gmx.de}
\@namedef{freecol-developers.mbox_1075}{45501E67.9020008\%40gmx.de}
\@namedef{freecol-developers.mbox_1079}{45654.80.213.139.73.1163626631.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1076}{200611112102.28200.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1078}{57651.80.213.139.73.1163623551.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1077}{200611142131.29034.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1080}{48184.80.213.139.73.1164457401.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1081}{4568430A.5070904\%40gmx.de}
\@namedef{freecol-developers.mbox_1082}{200611251950.05747.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1083}{60141.80.213.139.73.1164548783.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1084}{456C7659.2000601\%40gmx.de}
\@namedef{freecol-developers.mbox_1085}{200611282140.38973.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1086}{456DA734.4000904\%40gmx.de}
\@namedef{freecol-developers.mbox_1087}{456DA793.6000300\%40gmx.de}
\@namedef{freecol-developers.mbox_1088}{37757.80.213.139.73.1164843440.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1089}{200611300107.56087.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1090}{54124.80.213.139.73.1164845691.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1091}{456F085A.6090001\%40gmx.de}
\@namedef{freecol-developers.mbox_1092}{58049.80.213.139.73.1164907316.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1093}{456F1DD3.7070804\%40gmx.de}
\@namedef{freecol-developers.mbox_1095}{35137.80.213.139.73.1165016265.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1096}{45713DC4.7050502\%40gmx.de}
\@namedef{freecol-developers.mbox_1097}{200612021214.42365.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1094}{60776.80.213.139.73.1165009536.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1098}{32822fe60612030013o5195e59ej9943b9f968264faa\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1100}{45728BBD.8070606\%40gmx.de}
\@namedef{freecol-developers.mbox_1114}{32822fe60612062031w593810d2pb811f17da4ecc2fd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1115}{4577B341.5000508\%40gmx.de}
\@namedef{freecol-developers.mbox_1117}{32822fe60612070854k2adf042eu6a68fa46a06741f1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1121}{45790C22.6040602\%40gmx.de}
\@namedef{freecol-developers.mbox_1124}{54581.129.240.76.172.1165581447.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1139}{32822fe60612120738g1641a661va949bbea33cc643c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1140}{44600.80.213.195.201.1165939195.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1254}{32822fe60701261808q423992i4b8e8a607afba194\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1103}{56098.80.213.139.73.1165175686.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1099}{32822fe60612030021m262695a9m5f49379afc1dce9c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1101}{45728C35.9030408\%40gmx.de}
\@namedef{freecol-developers.mbox_1102}{33630.80.213.139.73.1165164141.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1106}{4575365B.8030500\%40gmail.com}
\@namedef{freecol-developers.mbox_1108}{3c8f359e0612050848t72eeb7b1v21e716542e702c60\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1109}{60708.80.213.139.73.1165360767.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1110}{d311c6a80612051611y4c70daau1195db6acdd71143\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1113}{32822fe60612060550i2a9a943eld16ee65f491e9a0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1123}{53165.129.240.76.172.1165581237.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1104}{49482.80.213.139.73.1165273680.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1105}{4575210C.70807\%40gmx.de}
\@namedef{freecol-developers.mbox_1107}{54750.80.213.139.73.1165313296.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1111}{45766CF9.7050401\%40gmx.de}
\@namedef{freecol-developers.mbox_1119}{55726.80.213.135.132.1165535585.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1120}{45790946.6070607\%40gmx.de}
\@namedef{freecol-developers.mbox_1137}{58058.80.213.195.201.1165876424.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1112}{49547.80.213.139.73.1165403748.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1126}{457AFAAC.7060206\%40gmx.de}
\@namedef{freecol-developers.mbox_1127}{200612092314.40886.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1116}{38817.80.213.135.132.1165494276.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1118}{32822fe60612070901x52732f62x3bea363e0518fbf8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1122}{45790CE9.1040001\%40gmx.de}
\@namedef{freecol-developers.mbox_1125}{54659.129.240.76.172.1165586005.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1128}{457C2EC7.6030800\%40gmx.de}
\@namedef{freecol-developers.mbox_1129}{457C4169.6040901\%40gmx.de}
\@namedef{freecol-developers.mbox_1135}{59856.193.157.182.100.1165853053.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1130}{3c8f359e0612101318i3d4859dasb2590c30328d7863\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1131}{3c8f359e0612101335s48d951d1gd0d4bb0fcde9231c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1136}{58874.193.157.182.100.1165853761.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1132}{200612110000.01729.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1133}{20061211092025.83590\%40gmx.net}
\@namedef{freecol-developers.mbox_1134}{59034.193.157.182.100.1165852065.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1138}{60648.80.213.195.201.1165921888.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1253}{32822fe60701261805v390c1710h8535ee6d150d9cc4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1141}{52965.80.213.195.201.1166095140.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1142}{45817FD9.5070600\%40gmx.de}
\@namedef{freecol-developers.mbox_1143}{2006121505586.07222\%40MICROSOF-812002.net}
\@namedef{freecol-developers.mbox_1144}{7b94298e0612180843g28d26258xd7e852f95594002d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1145}{7b94298e0612180855j74d667fepa77f3370a5dc10c9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1146}{200612182053.50963.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1147}{7b94298e0612181804w6331fc64l1cb8556c8f3d4e60\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1148}{7b94298e0612211536l43ba82bfs67dd71ba6481b9f6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1149}{3c8f359e0612221522y6525b529s99c48fa999bc041a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1150}{458CCC2F.60804\%40gmx.de}
\@namedef{freecol-developers.mbox_1151}{7b94298e0612231104n37e7dab9p181eae02b6346b82\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1152}{34656.80.213.195.201.1166963933.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1153}{3c8f359e0612240839x48989b3fj1ff5b9de85756d0d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1154}{200612252246.19249.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1155}{459142BA.8030802\%40gmx.de}
\@namedef{freecol-developers.mbox_1156}{7b94298e0612260844u6d8597cdw34355c4af2845072\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1157}{7b94298e0612260852r4da285b9i38d5fc19b2d34f1c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1160}{45922320.5090202\%40gmx.de}
\@namedef{freecol-developers.mbox_1183}{50925.80.213.192.230.1168598098.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1187}{45A89D94.9010202\%40gmx.de}
\@namedef{freecol-developers.mbox_1189}{3c8f359e0701130947k9780303qb31aa44d4f5c147f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1158}{200612262042.28727.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1159}{3c8f359e0612261656j4ed2af18i9c1d8b831f587f1e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1161}{7e2763d07d1ba21f84ab75888eb47d25\%40localhost}
\@namedef{freecol-developers.mbox_1162}{45928D4B.8030904\%40gmx.de}
\@namedef{freecol-developers.mbox_1163}{200612271921.51938.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1164}{4598D6D8.6010004\%40nours.org}
\@namedef{freecol-developers.mbox_1165}{3c8f359e0701022025q6f791507gd89a6e7fe07058d3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1166}{200701031854.55190.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1167}{45A0E30B.4090204\%40gmx.de}
\@namedef{freecol-developers.mbox_1168}{7b94298e0701070744y2a37200fs9d22f1b7858a823\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1169}{45A1F2AD.6070002\%40gmx.de}
\@namedef{freecol-developers.mbox_1173}{7b94298e0701091237t444240bas235c8b89801c2efa\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1180}{7b94298e0701101237l580041ffif4e9eae7a68120fa\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1170}{e12601c73376$5dcc5c20$8edd10e4\%40Forward_Earnings_}
\@namedef{freecol-developers.mbox_1171}{200701092044.28918.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1172}{7b94298e0701091210p53373c07s3257c23d58240bc3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1181}{34797.80.213.192.230.1168596688.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1174}{200701092139.53661.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1175}{2A5C006D-B010-4773-BBF5-37B23DC59970\%40transmog.com.au}
\@namedef{freecol-developers.mbox_1177}{35262.80.232.91.135.1168388513.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1178}{52ae8df10701100110q4fafd677i40db336d416f39b6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1176}{7b94298e0701091557l112b3532r532e94620bbfe9d2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1179}{7b94298e0701101227s5fecfd13g58786bb515373aef\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1182}{36712.80.213.192.230.1168597633.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1184}{35098.80.213.192.230.1168603149.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1185}{7b94298e0701121136p13051461t5a95af1593bda0c5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1186}{45A89C81.10300\%40gmx.de}
\@namedef{freecol-developers.mbox_1188}{200701131033.55679.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1214}{44268.80.213.136.14.1169465189.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1218}{45B4DB4F.5010205\%40gmx.de}
\@namedef{freecol-developers.mbox_1190}{p06002074c1d12cf1836c\%40[192.168.31.11]}
\@namedef{freecol-developers.mbox_1191}{3c8f359e0701150822y227f845co5c544185f1c9c596\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1192}{45ACFF59.9030405\%40gmx.de}
\@namedef{freecol-developers.mbox_1193}{45AE5382.5050306\%40gmx.de}
\@namedef{freecol-developers.mbox_1215}{60140.80.213.136.14.1169470709.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1221}{45B4E214.9050308\%40gmx.de}
\@namedef{freecol-developers.mbox_1231}{40757.80.213.136.14.1169549441.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1194}{45AE54B3.30009\%40gmx.de}
\@namedef{freecol-developers.mbox_1197}{200701182350.27884.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1212}{3c8f359e0701212330v7996b9fby4ccf43b3f1e4dbab\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1195}{45AFA88E.6050504\%40gmx.de}
\@namedef{freecol-developers.mbox_1196}{45AFA985.4070107\%40gmx.de}
\@namedef{freecol-developers.mbox_1198}{45AFF66A.4080902\%40nours.org}
\@namedef{freecol-developers.mbox_1199}{45B24A2A.1020806\%40gmx.de}
\@namedef{freecol-developers.mbox_1200}{200701202106.37621.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1201}{32822fe60701202324r242be2aaof5eaf4efe445fccd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1202}{45B327A2.9010601\%40gmx.de}
\@namedef{freecol-developers.mbox_1204}{32822fe60701210639t7aae1837ja05942f794bde4b3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1203}{200701211518.40885.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1205}{32822fe60701210640n26c3a117of2caee3eecfb911b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1206}{45B380A0.5050500\%40gmx.de}
\@namedef{freecol-developers.mbox_1207}{32822fe60701210945r72d0b7e3ve949a96fee93d005\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1208}{200701211917.29439.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1209}{32822fe60701211118w377edac7qb7c3d0934e1ee4db\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1210}{32822fe60701211319u4e1b13e8rb2db5388ca3ad0d6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1219}{45B4DC68.9060301\%40gmx.de}
\@namedef{freecol-developers.mbox_1228}{200701222202.19741.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1233}{32822fe60701230633p68eb88f8j60202e1138be2397\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1234}{200701231854.03820.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1235}{32822fe60701231635n153c094ci75c750f65904174a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1211}{32822fe60701211613m4f22237s45e7076358ba3fe\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1222}{45B4F03A.3040909\%40gmx.de}
\@namedef{freecol-developers.mbox_1255}{32822fe60701262025v349e2318k2f037ae6af62b603\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1260}{45BB12A8.3080801\%40gmx.de}
\@namedef{freecol-developers.mbox_1213}{006c01c73dfb$a9d3e3b0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1236}{54902.80.213.136.14.1169632876.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1241}{000001c740aa$a46c7de0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1216}{60176.80.213.136.14.1169470868.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1224}{200701221928.02906.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1217}{44bb52ee0701220740i1a41eb35pf75bd3edb8dbce5f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1220}{45B4DFAC.6060108\%40gmx.de}
\@namedef{freecol-developers.mbox_1232}{59583.80.213.136.14.1169549625.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1223}{45B4F0F0.2060904\%40gmx.de}
\@namedef{freecol-developers.mbox_1225}{200701222003.10567.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1229}{20070123070615.44750\%40gmx.net}
\@namedef{freecol-developers.mbox_1226}{32822fe60701221122r67bbd6a7h993e15a5b83c334c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1227}{32822fe60701221234r23e7df9ej387def1fb9c87488\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1230}{20070123073548.44790\%40gmx.net}
\@namedef{freecol-developers.mbox_1237}{32822fe60701241247r4fa15e10odc9f2918f8b3a202\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1238}{20070125083953.51950\%40gmx.net}
\@namedef{freecol-developers.mbox_1239}{5de90cc95fa616584859a7a2a7f59ed9\%40localhost}
\@namedef{freecol-developers.mbox_1256}{32822fe60701262202k1f96fe32v4855a689d609685b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1259}{45BB1252.50702\%40gmx.de}
\@namedef{freecol-developers.mbox_1265}{32822fe60701271417n71056cc3w1b13e92b4a838ff7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1262}{000001c7420f$4c1f70a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1266}{32822fe60701271420o18ff8049w6d0ae1441b88fd63\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1287}{56418.80.213.136.14.1170080141.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1240}{45B8E5A4.6070004\%40gmx.de}
\@namedef{freecol-developers.mbox_1244}{50595.80.213.136.14.1169765150.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1245}{32822fe60701252219r10a75d14sda6a43804910c59d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1246}{20070126103218.256550\%40gmx.net}
\@namedef{freecol-developers.mbox_1248}{52236.194.71.243.129.1169808055.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1250}{56402.80.213.136.14.1169809141.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1251}{32822fe60701261756m1e64b4eeudf56d6bf97ca2ff\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1249}{60663.80.213.136.14.1169808797.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1261}{45BB15CF.2000800\%40gmx.de}
\@namedef{freecol-developers.mbox_1247}{51929.80.213.136.14.1169807913.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1252}{32822fe60701261804i36fd75ifac10c9b43d13a36\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1242}{01c740bb$3f7a7340$8dae9b52\%40oelm23h9ij74tu}
\@namedef{freecol-developers.mbox_1243}{000f01c740bc$d75fd640$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1257}{32822fe60701262254r8d62932p8770c4df35666c8a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1258}{45BB0E6F.9080404\%40gmx.de}
\@namedef{freecol-developers.mbox_1316}{50931.80.213.137.143.1171201249.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1317}{45CF2516.5020409\%40gmx.de}
\@namedef{freecol-developers.mbox_1263}{2007012880428.12108\%40MICROSOF-812002.net}
\@namedef{freecol-developers.mbox_1264}{32822fe60701271341u6c93a486wfbf2defd69ff83ed\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1267}{45BC76B9.3030106\%40gmx.de}
\@namedef{freecol-developers.mbox_1276}{32822fe60701280729g58d4dfabm396b60a934bbce70\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1280}{45BCCB32.8080505\%40gmx.de}
\@namedef{freecol-developers.mbox_1268}{200701281312.26833.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1274}{45BCB480.5040508\%40gmx.de}
\@namedef{freecol-developers.mbox_1277}{32822fe60701280736m66ec6675s2c4580307ac1fad\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1278}{45BCC531.2040604\%40gmx.de}
\@namedef{freecol-developers.mbox_1269}{002f01c742d6$fc4fc7f0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1270}{45BC996A.1020201\%40gmx.de}
\@namedef{freecol-developers.mbox_1271}{45BCA591.5010303\%40gmx.de}
\@namedef{freecol-developers.mbox_1282}{200701290013.08714.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1283}{45BD8CF5.9080000\%40gmx.de}
\@namedef{freecol-developers.mbox_1272}{49034.80.213.136.14.1169994120.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1273}{45BCB420.1050908\%40gmx.de}
\@namedef{freecol-developers.mbox_1281}{200701282309.12685.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1285}{39438.80.213.136.14.1170071255.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1290}{200701310110.33159.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1284}{39435.80.213.136.14.1170071242.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1279}{32822fe60701280750w1913cebmd6fd709571123191\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1286}{32928.80.213.136.14.1170071839.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1291}{32822fe60701301908y3537626bm295fcfd763537611\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1275}{45BCB893.7030509\%40gmx.de}
\@namedef{freecol-developers.mbox_1288}{01c743ba$e9889950$f7e02551\%40bulek123ab2ba3}
\@namedef{freecol-developers.mbox_1289}{45BF3EFA.9040601\%40gmail.com}
\@namedef{freecol-developers.mbox_1318}{52ae8df10702110706n74d16bc7pcc17eb6b768f2b80\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1319}{52ae8df10702110714q135f7ccbr3c8ac4834f8bf23c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1292}{01c747c6$2daa7130$e662c353\%40JAKO}
\@namedef{freecol-developers.mbox_1293}{200702041504.22801.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1294}{000701c7487c$86dd1990$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1307}{32822fe60702071137h3bbd2a95i8d8772dc393c7b7a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1295}{001701c74908$6f4b99a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1296}{001801c7490a$5eef9a50$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1297}{58955.129.240.76.172.1170682667.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1299}{45C75A55.3010501\%40gmx.de}
\@namedef{freecol-developers.mbox_1300}{60639.129.240.76.172.1170695291.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1301}{45C77C44.1020609\%40gmx.de}
\@namedef{freecol-developers.mbox_1302}{200702060047.20347.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1303}{d311c6a80702051550y42874bb1g7ff1d3dde59262e6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1304}{2458.80.213.137.143.1170762529.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1306}{d311c6a80702061324ra7c7d60pd97bdef60e568cb1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1298}{000601c74938$18058680$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1308}{32822fe60702071147k3b9bc46ald907986c761aefb5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1305}{01c749ed$1ce699e0$1cc5b7d4\%40fernandozamora}
\@namedef{freecol-developers.mbox_1309}{45CEFA8A.6020508\%40gmx.de}
\@namedef{freecol-developers.mbox_1311}{59820.80.213.137.143.1171194391.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1312}{45CF0762.6030007\%40gmx.de}
\@namedef{freecol-developers.mbox_1310}{45CEFAED.9010607\%40gmx.de}
\@namedef{freecol-developers.mbox_1313}{46365.80.213.137.143.1171198738.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1314}{200702111423.30111.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1315}{001701c74de0$48556ec0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1320}{000601c74e05$2f4e6ba0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1321}{200702122042.02946.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1322}{46280.194.71.243.129.1171352813.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1323}{58876.80.213.147.140.1171362730.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1326}{45D773A8.30609\%40laposte.net}
\@namedef{freecol-developers.mbox_1324}{01c7509a$0ad14120$6b86115a\%40poulet}
\@namedef{freecol-developers.mbox_1325}{CC0A541B.2EBA8F3\%40gmail.com}
\@namedef{freecol-developers.mbox_1327}{45D81D74.5060608\%40gmx.de}
\@namedef{freecol-developers.mbox_1331}{002a01c7538d$42d4b980$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1328}{C3BEF5F5-964F-4CBA-BFD4-4A58E8D2D9C3\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1329}{45D86E68.5050809\%40gmx.de}
\@namedef{freecol-developers.mbox_1330}{70D8E384-0D4F-4B7C-BD7B-D9F9FDF145A8\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1332}{7B557FBD-4F3C-4A32-97DA-9D778A4C2EB5\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1333}{0746BB64-D134-4642-B0DB-FD20F12B3B15\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1336}{45DE9397.1080000\%40gmx.de}
\@namedef{freecol-developers.mbox_1334}{200702210018.13633.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1335}{200702210027.56732.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1337}{01c75748$d2b57e40$0201a8c0\%40comp}
\@namedef{freecol-developers.mbox_1338}{32822fe60702231956v6bc047e0n89b738e56282b7d5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1339}{45E00193.9040501\%40gmx.de}
\@namedef{freecol-developers.mbox_1340}{54DB139D-1842-485A-A824-878E1188EF51\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1341}{45E2069A.80101\%40gmx.de}
\@namedef{freecol-developers.mbox_1342}{775B01B4-7431-4D4C-BCF2-4638C6E47DC6\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1343}{45E316C0.8000303\%40gmx.de}
\@namedef{freecol-developers.mbox_1346}{200702282244.46190.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1350}{45E70290.9010405\%40gmx.de}
\@namedef{freecol-developers.mbox_1353}{200703012204.03684.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1344}{43b7bc360702280951j4bbb36d5h82c6aaa06daf626f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1347}{d311c6a80702281410p1b13ffe7gf67b54dc567ccd42\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1352}{45E707E3.4070709\%40gmx.de}
\@namedef{freecol-developers.mbox_1345}{200702282047.33448.carstengrohmann\%40gmx.de}
\@namedef{freecol-developers.mbox_1351}{45E70573.2060206\%40gmx.de}
\@namedef{freecol-developers.mbox_1348}{00a901c75b8d$86dfd1c0$0402a8c0\%4064BitBadass}
\@namedef{freecol-developers.mbox_1349}{d311c6a80702281556k56c928ccm2f24684801059604\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1354}{8f92144e0703041332n735498f8l74af3772b9360fa7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1355}{20070308015109.91a979dd.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1356}{45EFB690.4030709\%40gmx.de}
\@namedef{freecol-developers.mbox_1357}{20070308120712.ced0e2b0.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1358}{45EFF6FE.9040504\%40gmx.de}
\@namedef{freecol-developers.mbox_1359}{08CD0C4A-0659-438D-AC1F-8D72E160E9A1\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1360}{16384.194.71.243.129.1173357745.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1362}{45F142A6.4000000\%40gmx.de}
\@namedef{freecol-developers.mbox_1365}{7FBFF6AC-CD9F-4697-AFDB-B0BE0DBF1748\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1364}{3C36665F-8648-4553-A3BC-5704D407EFA8\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1361}{45F12CE9.7050009\%40gmx.de}
\@namedef{freecol-developers.mbox_1363}{45F15204.30306\%40gmx.de}
\@namedef{freecol-developers.mbox_1381}{59212.193.157.188.134.1174660177.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1382}{001501c76d68$93e0d440$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1383}{4604DBC3.5080400\%40gmx.de}
\@namedef{freecol-developers.mbox_1486}{4621CF77.6040909\%40gmx.de}
\@namedef{freecol-developers.mbox_1487}{000601c77f2e$a4639000$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1488}{4621F574.90400\%40gmx.de}
\@namedef{freecol-developers.mbox_1366}{fd6345820703160707u56df6a40o8f5c11c5b377458\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1367}{45FBCDE7.3040807\%40gmx.de}
\@namedef{freecol-developers.mbox_1368}{fd6345820703170525v60990ce6t6c279246a2002d97\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1369}{fd6345820703170530g4118b51cy9c1ff641e0a7f1ce\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1370}{005001c76892$b7dbd5a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1371}{960955110703170558q231e7882vff33afc77595f4f0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1372}{005d01c76894$d7a14f30$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1373}{960955110703170606i52284fb8jcc3c2d18ba0ec761\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1374}{000101c7694e$89dac550$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1375}{45FD2A9E.4030608\%40gmx.de}
\@namedef{freecol-developers.mbox_1377}{200703181353.35618.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1378}{001101c76980$8c9b3220$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1376}{200703181351.45881.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1379}{001201c76985$5a806800$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1380}{36402.194.71.243.129.1174548795.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1413}{200704011234.01320.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1439}{000101c7783b$4cf18a10$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1440}{46162E37.8060200\%40gmx.de}
\@namedef{freecol-developers.mbox_1441}{000301c77844$3e11c650$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1384}{000001c76ec6$8434a0d0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1385}{20070325165808.b2b6f513.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1386}{001101c76f77$837e91d0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1387}{4607E050.10509\%40gmx.de}
\@namedef{freecol-developers.mbox_1388}{4607E299.1090404\%40gmx.de}
\@namedef{freecol-developers.mbox_1389}{20070326211208.3089f971.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1394}{460BD29D.1020503\%40gmx.de}
\@namedef{freecol-developers.mbox_1397}{37362.80.213.141.42.1175265220.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1398}{460D3704.9090701\%40gmx.de}
\@namedef{freecol-developers.mbox_1400}{20070331014158.eeff6e0a.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1390}{000c01c770e0$41d4f890$0402a8c0\%4064BitBadass}
\@namedef{freecol-developers.mbox_1391}{460A2F74.5060906\%40gmail.com}
\@namedef{freecol-developers.mbox_1392}{002301c77136$c77c6720$0402a8c0\%4064BitBadass}
\@namedef{freecol-developers.mbox_1393}{460A7548.3090600\%40gmail.com}
\@namedef{freecol-developers.mbox_1395}{005501c772cb$b8703f40$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1396}{60501.80.213.141.42.1175262856.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1399}{460D3CF5.3070700\%40gmx.de}
\@namedef{freecol-developers.mbox_1414}{200704011248.35257.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1415}{fd6345820704010446w489f58baw131657612c526636\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1401}{002d01c77383$8597da20$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1402}{fd6345820703310420x2e3a14f3ned253913cd6c38d0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1403}{fd6345820703310436i15480138i667f7d66d7adac21\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1404}{460E4AA3.2090008\%40gmx.de}
\@namedef{freecol-developers.mbox_1405}{48494.80.213.141.42.1175343637.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1408}{003301c773b5$a04798b0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1411}{460F6054.8030405\%40gmx.de}
\@namedef{freecol-developers.mbox_1406}{460E6246.2080503\%40gmx.de}
\@namedef{freecol-developers.mbox_1409}{003401c773b7$0851daa0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1407}{460E69A2.9010003\%40gmx.de}
\@namedef{freecol-developers.mbox_1410}{003501c773b7$827da430$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1412}{460F66FF.5070909\%40gmx.de}
\@namedef{freecol-developers.mbox_1416}{460FB70F.3040203\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1417}{460FD033.6050709\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1418}{20070401185124.b7632ac2.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1419}{460FD853.4020304\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1420}{20070402052252.M76552\%40pu.ac.in}
\@namedef{freecol-developers.mbox_1421}{461117B8.50105\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1422}{200704022154.13809.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1423}{461165DF.7080900\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1430}{461335FD.3060901\%40gmx.de}
\@namedef{freecol-developers.mbox_1424}{36027.80.213.199.35.1175586427.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1425}{32706.194.71.243.129.1175587513.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1426}{40236.80.213.199.35.1175621184.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1438}{000001c77836$7a965c70$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1427}{200704032147.09923.carstengrohmann\%40gmx.de}
\@namedef{freecol-developers.mbox_1428}{46133434.5080602\%40gmx.de}
\@namedef{freecol-developers.mbox_1429}{d311c6a80704032217v54afceb4nb676203f7c07f8e6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1434}{20070404135346.e539ad58.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1431}{200704040754.05227.carstengrohmann\%40gmx.de}
\@namedef{freecol-developers.mbox_1432}{461340C9.3050009\%40gmx.de}
\@namedef{freecol-developers.mbox_1433}{op.tp84z4x62817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1435}{op.tp9lq7ri2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1436}{4613F5CA.5070107\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1437}{d311c6a80704041801m7a0f99d8qc93a2184dc14222\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1442}{461912F0.1090307\%40peter-lohmann.de}
\@namedef{freecol-developers.mbox_1444}{20070408191044.627068f9.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1451}{32822fe60704101214j69631898o9c637b6123b94603\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1454}{23967.87.234.199.44.1176292103.squirrel\%40ssl.lohmann-services.de}
\@namedef{freecol-developers.mbox_1455}{54532.193.157.182.54.1176295544.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1443}{5213d1d20704080908j6479b6aeg7c1f380647b12397\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1445}{4619E87D.9030206\%40gmx.de}
\@namedef{freecol-developers.mbox_1446}{461A1A83.2090801\%40gmx.de}
\@namedef{freecol-developers.mbox_1447}{54681.80.213.129.243.1176131638.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1449}{461BA7C2.2060702\%40gmx.de}
\@namedef{freecol-developers.mbox_1448}{20070410060201.M90222\%40pu.ac.in}
\@namedef{freecol-developers.mbox_1450}{461BA7FA.3050702\%40gmx.de}
\@namedef{freecol-developers.mbox_1452}{op.tql5wvbn2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1453}{20070411101509.56100\%40gmx.net}
\@namedef{freecol-developers.mbox_1464}{op.tqnblzw52817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1456}{36750.193.157.182.54.1176297369.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1457}{34977.194.71.243.129.1176298753.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1459}{461CF2A5.8090208\%40gmx.de}
\@namedef{freecol-developers.mbox_1465}{40833.193.157.182.54.1176367112.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1458}{461CF0FC.6010907\%40gmx.de}
\@namedef{freecol-developers.mbox_1460}{20070411173756.2f3c1df9.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1462}{461CF8E8.2040408\%40gmx.de}
\@namedef{freecol-developers.mbox_1469}{49010.193.157.182.54.1176374363.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1461}{13A3E7AE-956E-4442-A7DE-A429A0B322D2\%40cl.uni-heidelberg.de}
\@namedef{freecol-developers.mbox_1463}{461D05FA.9030207\%40gmail.com}
\@namedef{freecol-developers.mbox_1466}{5213d1d20704120305t45f534d9xae8f2851d08cebc2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1468}{40096.193.157.182.54.1176373077.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1470}{5213d1d20704120325jbeb6617ied31ffa3df9afeff\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1471}{58114.193.157.182.54.1176374768.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1474}{5213d1d20704120404t7a365708ne50febc19caccf57\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1478}{60431.193.157.188.134.1176379677.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1480}{20070412125735.169720\%40gmx.net}
\@namedef{freecol-developers.mbox_1481}{5213d1d20704120618t35d80229r64b490d05011a38b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1476}{op.tqn5clwb2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1475}{35115.194.71.243.129.1176377879.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1477}{5213d1d20704120448y1da1554i824d245a70e59ecb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1479}{40868.193.157.188.134.1176380461.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1467}{20070412101356.257100\%40gmx.net}
\@namedef{freecol-developers.mbox_1472}{41879.193.157.182.54.1176375109.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1473}{41895.193.157.182.54.1176375117.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1482}{5213d1d20704130943m3bc28e6sf4ca8896ff37560b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1483}{46208533.5030303\%40gmx.de}
\@namedef{freecol-developers.mbox_1484}{5213d1d20704141022y4d2ff036nf1129b86153d5c68\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1485}{000d01c77ebb$48a73410$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1489}{op.tqtlr8er2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1490}{4622193D.1040107\%40gmx.de}
\@namedef{freecol-developers.mbox_1495}{34908.80.213.148.51.1176715573.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1491}{46231215.50200\%40gmx.de}
\@namedef{freecol-developers.mbox_1492}{001301c77fee$9fc30290$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1493}{46231A3E.6030206\%40gmx.de}
\@namedef{freecol-developers.mbox_1496}{34375.80.213.148.51.1176716247.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1497}{20070416110838.33690\%40gmx.net}
\@namedef{freecol-developers.mbox_1498}{54223.80.213.148.51.1176722605.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1494}{42651.80.213.148.51.1176714325.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1499}{20070416143940.A16372\%40email.ro}
\@namedef{freecol-developers.mbox_1500}{53340.80.213.148.51.1176724429.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1501}{59994.193.157.182.54.1176744846.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1502}{41192.129.240.176.68.1176752076.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1503}{20070417033726.130b1fa3.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1504}{46299.193.157.182.54.1176802842.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1505}{46262A1E.4080804\%40gmx.de}
\@namedef{freecol-developers.mbox_1506}{4626646E.8040704\%40gmail.com}
\@namedef{freecol-developers.mbox_1507}{10066312.post\%40talk.nabble.com}
\@namedef{freecol-developers.mbox_1508}{46269226.2020209\%40gmail.com}
\@namedef{freecol-developers.mbox_1510}{34486.193.157.182.54.1176971240.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1511}{462756D6.309\%40gmail.com}
\@namedef{freecol-developers.mbox_1512}{462789D7.3090406\%40gmx.de}
\@namedef{freecol-developers.mbox_1514}{33194.193.157.182.54.1177060433.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1515}{4628A52D.3020706\%40gmail.com}
\@namedef{freecol-developers.mbox_1509}{200704190021.39728.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1513}{4627944E.4090203\%40gmx.de}
\@namedef{freecol-developers.mbox_1516}{20070421151755.2de79c7d.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1517}{20070421160516.5e03a453.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1520}{462A374C.1080008\%40gmx.de}
\@namedef{freecol-developers.mbox_1522}{42767.80.213.148.51.1177174490.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1568}{20070504123723.28e4c05a.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1724}{20070613014112.22b827fe.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1727}{37465.193.157.182.68.1181743926.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1518}{20070421172247.c59a76a4.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1519}{462A36F0.6080704\%40gmx.de}
\@namedef{freecol-developers.mbox_1521}{20070421194142.1eba7982.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1523}{462B0DB3.8090308\%40gmx.de}
\@namedef{freecol-developers.mbox_1524}{20070422113843.417ae4d4.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1530}{57680.80.213.148.51.1177319944.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1538}{463032C3.6020206\%40gmx.de}
\@namedef{freecol-developers.mbox_1586}{42236.193.157.182.83.1178544747.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1525}{200704221232.29126.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1526}{200704221352.41515.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1527}{200704221321.08116.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1528}{000c01c784e1$f72b0c10$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1529}{op.tq64txm62817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1531}{5213d1d20704230619tc8408acra04b6d4aac06268b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1540}{4630351E.7030707\%40gmx.de}
\@namedef{freecol-developers.mbox_1562}{op.trpic50x2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1532}{462CC9AE.3080409\%40qense.nl}
\@namedef{freecol-developers.mbox_1535}{58564.193.157.188.134.1177413119.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1533}{54243.80.213.148.51.1177349058.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1534}{20070424004924.4b812f4c.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1536}{39666.193.157.182.54.1177493334.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1537}{20070425181626.1d4684df.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1539}{4630343A.6050907\%40gmx.de}
\@namedef{freecol-developers.mbox_1541}{4630E7FE.40702\%40gmail.com}
\@namedef{freecol-developers.mbox_1542}{463215EE.6060109\%40qense.nl}
\@namedef{freecol-developers.mbox_1559}{4635A3E4.4010803\%40gmx.de}
\@namedef{freecol-developers.mbox_1543}{05AC0C6C.ACAB446\%40gmail.com}
\@namedef{freecol-developers.mbox_1544}{1831cc480704280859n13c2dd05g1661b9c71721a7cf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1545}{5213d1d20704280926t54322d1m68201ce72e60910\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1546}{46348F93.2020500\%40gmx.de}
\@namedef{freecol-developers.mbox_1547}{4634A89F.1\%40gmx.de}
\@namedef{freecol-developers.mbox_1548}{4634A93D.5030208\%40gmx.de}
\@namedef{freecol-developers.mbox_1549}{AE4FF20C.C1CE454\%40gmail.com}
\@namedef{freecol-developers.mbox_1550}{60140.193.157.182.96.1177933439.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1551}{20070430145817.dd0d1591.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1561}{4635DEFA.6040906\%40gmx.de}
\@namedef{freecol-developers.mbox_1552}{47731.193.157.182.96.1177935943.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1553}{50072.193.157.182.96.1177943613.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1554}{55498.193.157.182.96.1177946922.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1555}{46359898.8040904\%40gmx.de}
\@namedef{freecol-developers.mbox_1585}{45620.193.157.182.83.1178543241.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1556}{20070501003118.6073e96f.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1557}{p0624080dc25c11e5eec6\%40[10.0.1.3]}
\@namedef{freecol-developers.mbox_1558}{p0624080fc25c14e7a337\%40[10.0.1.3]}
\@namedef{freecol-developers.mbox_1560}{p06240817c25cd07999eb\%40[10.0.1.3]}
\@namedef{freecol-developers.mbox_1563}{op.trq5scty2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1564}{4639E9F2.8080607\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1565}{20070503134015.113260\%40gmx.net}
\@namedef{freecol-developers.mbox_1566}{200705032134.50683.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1569}{op.trstpbmi2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1570}{7E33F1C8-5B97-467E-A14F-3B6C98B47B8E\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1571}{463B2057.9030502\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1567}{463A157D.4000706\%40gmx.de}
\@namedef{freecol-developers.mbox_1584}{52349.193.157.182.83.1178542763.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1628}{464AA1D9.8060304\%40gmx.de}
\@namedef{freecol-developers.mbox_1630}{464AB76A.1000104\%40gmx.de}
\@namedef{freecol-developers.mbox_1572}{463C3E99.1010805\%40gmx.de}
\@namedef{freecol-developers.mbox_1573}{200705051257.55689.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1582}{41618.193.157.182.83.1178541640.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1592}{463F36DB.10102\%40gmx.de}
\@namedef{freecol-developers.mbox_1597}{463F5D9B.5010909\%40gmx.de}
\@namedef{freecol-developers.mbox_1574}{7bd504520705051008v56e323b9p5dfb02b69261cca3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1575}{200705052219.44800.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1576}{463D1098.3050209\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1577}{463D8990.9010407\%40gmx.de}
\@namedef{freecol-developers.mbox_1578}{7b94298e0705061403o364e1baeh30183aa97f928742\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1581}{53436.193.157.182.83.1178541188.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1579}{37902.193.157.182.83.1178537058.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1580}{op.tryhqtqt2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1583}{p0624080cc264c98324d8\%40[10.0.1.3]}
\@namedef{freecol-developers.mbox_1591}{463F36BB.70404\%40gmx.de}
\@namedef{freecol-developers.mbox_1587}{JHODZ300.NEI\%40postoffice.sarnoff.com}
\@namedef{freecol-developers.mbox_1595}{463F3ADC.7050703\%40gmx.de}
\@namedef{freecol-developers.mbox_1588}{JHOET800.SH9\%40postoffice.sarnoff.com}
\@namedef{freecol-developers.mbox_1598}{463F5E50.5070401\%40gmx.de}
\@namedef{freecol-developers.mbox_1593}{463F38FD.8000805\%40gmx.de}
\@namedef{freecol-developers.mbox_1618}{4648AF4E.7050001\%40ifrance.com}
\@namedef{freecol-developers.mbox_1621}{op.tscy1n2k2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1589}{op.tryp4ioj2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1594}{463F5349.9000708\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1596}{463F5B6B.8070006\%40gmx.de}
\@namedef{freecol-developers.mbox_1590}{20070507134841.4075.qmail\%40web52902.mail.re2.yahoo.com}
\@namedef{freecol-developers.mbox_1599}{49032.193.157.182.83.1178710746.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1600}{op.tr3s3kvz2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1601}{38806.193.157.189.141.1178790189.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1602}{1178855147.10449.3.camel\%40vbabiy-desktop}
\@namedef{freecol-developers.mbox_1606}{46447994.5000601\%40gmx.de}
\@namedef{freecol-developers.mbox_1603}{57931.193.157.182.83.1178880246.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1604}{20070511110015.278920\%40gmx.net}
\@namedef{freecol-developers.mbox_1605}{11274.194.71.243.129.1178882451.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1607}{fd6345820705110912s1fd2040ai967e0af3afd50e47\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1609}{46456DC4.30706\%40gmx.de}
\@namedef{freecol-developers.mbox_1608}{46456D6C.1020001\%40gmx.de}
\@namedef{freecol-developers.mbox_1610}{fd6345820705120050k2f55de31u96fc954a8a543441\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1611}{464574CC.9030504\%40gmx.de}
\@namedef{freecol-developers.mbox_1612}{7bd504520705121153s4321e43evea981ac55726b2d2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1613}{46461959.4040606\%40ifrance.com}
\@namedef{freecol-developers.mbox_1614}{52395.80.213.132.178.1179062425.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1615}{000601c795a8$57ebbd20$0201a8c0\%40GeneralEric}
\@namedef{freecol-developers.mbox_1616}{4647FF82.70608\%40gmx.de}
\@namedef{freecol-developers.mbox_1617}{46486B3A.8020308\%40gmx.de}
\@namedef{freecol-developers.mbox_1619}{200705142314.38393.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1620}{19462.194.71.243.129.1179210382.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1622}{46497662.5060406\%40gmx.de}
\@namedef{freecol-developers.mbox_1623}{20070515120506.af189868.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1624}{op.tsdbn6vdg1lg6c\%40minime-i.netgear.com}
\@namedef{freecol-developers.mbox_1625}{4649AF98.6020301\%40gmx.de}
\@namedef{freecol-developers.mbox_1626}{op.tsddfkel2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1627}{op.tsdifdso2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1629}{464AA6B0.7010503\%40gmx.de}
\@namedef{freecol-developers.mbox_1631}{430163.59396.qm\%40web52906.mail.re2.yahoo.com}
\@namedef{freecol-developers.mbox_1632}{fd6345820705161517x45a0197fx5a471128b113ada4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1633}{200705170038.41896.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1634}{464C0598.7090808\%40gmx.de}
\@namedef{freecol-developers.mbox_1635}{000e01c79863$17242ee0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1636}{464C218B.1070705\%40gmx.de}
\@namedef{freecol-developers.mbox_1637}{0018a81b19b760ed2619c8fd850b5ba7\%40localhost}
\@namedef{freecol-developers.mbox_1639}{58722.193.157.182.15.1179478529.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1640}{464D6CC9.6080203\%40gmx.de}
\@namedef{freecol-developers.mbox_1641}{001a01c7992c$a5e9eb50$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1643}{464D7618.5000802\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1644}{50110.193.157.189.141.1179488093.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1645}{002601c79943$74a509a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1650}{37421.193.157.189.141.1179495085.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1653}{000a01c7995f$1b036a60$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1658}{464EA1B2.5060009\%40gmx.de}
\@namedef{freecol-developers.mbox_1661}{001201c799f6$3ef55ae0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1666}{465011DC.5020004\%40gmx.de}
\@namedef{freecol-developers.mbox_1638}{464C2727.5060303\%40gmx.de}
\@namedef{freecol-developers.mbox_1642}{1FE45033-F7C0-4681-A83B-B98369D98BAB\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1655}{44673.193.157.182.15.1179503037.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1656}{500DD3CC-DBD8-4A8D-8261-932B80992562\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1659}{464EA63D.3010904\%40gmx.de}
\@namedef{freecol-developers.mbox_1646}{1179492139.10183.1.camel\%40vbabiy-desktop}
\@namedef{freecol-developers.mbox_1647}{464DA533.8060607\%40gmx.de}
\@namedef{freecol-developers.mbox_1648}{0fc76444d43d7ca1a5e2489eea8c05a8\%40localhost}
\@namedef{freecol-developers.mbox_1649}{e0923a4fac6cdc5a0f80a32ef21bcbab\%40localhost}
\@namedef{freecol-developers.mbox_1651}{464DAFBF.10502\%40gmx.de}
\@namedef{freecol-developers.mbox_1652}{000401c7995c$14486c00$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1654}{60126.193.157.182.15.1179501814.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1660}{464EA746.7040305\%40gmx.de}
\@namedef{freecol-developers.mbox_1657}{464E9AFE.7040500\%40gmx.de}
\@namedef{freecol-developers.mbox_1662}{46500470.3050603\%40gmx.de}
\@namedef{freecol-developers.mbox_1663}{E31EF56B-5DFD-4ADF-B3E1-4F5F8CE9568D\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1664}{002401c79abe$50479240$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1667}{20070521013124.7a6af1e3.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1665}{46501091.4050102\%40gmx.de}
\@namedef{freecol-developers.mbox_1668}{1179715319.12415.7.camel\%40vbabiy-desktop}
\@namedef{freecol-developers.mbox_1669}{200705211125.03236.armin\%40h2h.de}
\@namedef{freecol-developers.mbox_1670}{1179836263.7088.1.camel\%40vbabiy-desktop}
\@namedef{freecol-developers.mbox_1671}{4652F36B.4050103\%40gmx.de}
\@namedef{freecol-developers.mbox_1672}{4fb797ba0705220929u33fee4fbn81063d481deef241\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1676}{200705222235.35266.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1673}{685C5A41-AC3E-43B1-965A-24A93022FCBD\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1679}{59219.193.157.189.141.1179923448.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1680}{658FB5E7-D8EA-4F01-8B85-D0B7DAE6DF57\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1674}{000401c79ca4$62ee6a30$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1678}{4653E7F8.60401\%40gmx.de}
\@namedef{freecol-developers.mbox_1675}{54697.193.157.180.217.1179862554.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1677}{001201c79ce2$afeee740$6501a8c0\%40ericb2eb7b1f8c}
\@namedef{freecol-developers.mbox_1681}{006401c79e66$1094f9c0$31beed40$\%40com}
\@namedef{freecol-developers.mbox_1682}{46580796.4050701\%40gmx.de}
\@namedef{freecol-developers.mbox_1683}{46580ADB.7050106\%40gmx.de}
\@namedef{freecol-developers.mbox_1685}{20070526220225.0c3439e1.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1684}{46585A87.5090408\%40gmx.de}
\@namedef{freecol-developers.mbox_1708}{4fb797ba0706030353j363cf42ha1b235c0cc596ec2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1686}{46599D3D.6080106\%40gmx.de}
\@namedef{freecol-developers.mbox_1687}{20070529141312.075e99e6.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1688}{200705292347.46250.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1689}{BEE75F08-B2FD-471E-9AD6-4B7DBDB9829E\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1690}{fd6345820705300254x6a1a5407w8c1a785a004ff073\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1691}{81072A85-2736-4765-B2CB-B2510F530D68\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1692}{fd6345820705300444y3ae756b3sec22ce1f24a661ed\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1693}{op.ts43buhw2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_1694}{fd6345820705300559o7d87c2dr9dd444473580ff52\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1696}{18525.194.71.243.129.1180531246.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1695}{fd6345820705300626u3be62f22h19863ea0d50b9711\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1712}{000401c7a605$d73fd300$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1698}{5FE74B0D-7E18-4F5C-9FD7-0F090725EA21\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1699}{53288.194.71.243.129.1180608149.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1700}{37034.193.157.189.141.1180611346.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1701}{28306.194.71.243.129.1180612110.squirrel\%40bergersjo.com}
\@namedef{freecol-developers.mbox_1702}{fd6345820705310502ha54ed1ambee9db09db6d2beb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1704}{47431.129.240.176.122.1180618553.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1705}{fd6345820705310906q67a3ade4rdb53a119a2ead99c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1719}{49538.193.157.182.68.1181047048.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1703}{41075.129.240.176.122.1180618126.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1697}{200705302053.49593.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1706}{09536705-5AFC-459F-80E6-D7B49D008AE1\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1707}{46617AE0.9060105\%40gmx.de}
\@namedef{freecol-developers.mbox_1709}{4662E238.8050408\%40gmx.de}
\@namedef{freecol-developers.mbox_1710}{fd6345820706031004gc09afaer525d134fa1ddbf77\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1711}{000301c7a603$9cf1e640$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1713}{A6D92221-2FAF-4F4F-ADE1-45A09408C42B\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1714}{200706041846.00213.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1717}{4fb797ba0706041207j72022b19l61df1c66c21e950f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1715}{000601c7a6ca$1862ef10$0201a8c0\%40GeneralEric}
\@namedef{freecol-developers.mbox_1716}{200706041921.06009.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1718}{4fb797ba0706041212y4d81158bn656108a9fab63ba5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1720}{200706072338.26574.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1721}{58011.193.157.182.68.1181311503.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1722}{200706102316.19419.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1726}{44723.193.157.182.68.1181743531.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1723}{466CF75C.1050605\%40district.maple-ridge.bc.ca}
\@namedef{freecol-developers.mbox_1725}{BAY103-F1338F378D6EF5433EACCFBA0180\%40phx.gbl}
\@namedef{freecol-developers.mbox_1728}{37480.193.157.182.68.1181744110.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1729}{43697.193.157.182.68.1181749143.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1730}{49484.193.157.182.68.1181749317.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1731}{87sl8v5q5h.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1733}{34074.193.157.182.68.1181831521.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1732}{44479.193.157.182.68.1181830265.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1734}{000101c7ae91$3c0db250$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1736}{46648.193.157.182.68.1181835427.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1737}{87ps3ywmgv.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1740}{54011.129.240.69.63.1181916771.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1771}{39308.193.157.182.68.1182341735.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1774}{46794A2C.7010205\%40gmx.de}
\@namedef{freecol-developers.mbox_1776}{20070620185234.8070bfe0.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1778}{87odjamwq7.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1781}{46795584.2050406\%40gmx.de}
\@namedef{freecol-developers.mbox_1780}{46795386.8090601\%40gmx.de}
\@namedef{freecol-developers.mbox_1786}{34837.129.240.169.83.1182527218.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1788}{467BF2E3.3000103\%40gmx.de}
\@namedef{freecol-developers.mbox_1809}{20070626094753.5cd3078a.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1808}{20070626094354.e4a0162d.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1735}{87tztaworp.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1738}{87lkemwm56.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1739}{87hcpawh1p.fsf_-_\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1741}{87zm31uueb.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1742}{87vedpug8s.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1743}{87645lp4y3.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1744}{200706181920.47526.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1745}{4676D4FE.3060505\%40namcor.com.na}
\@namedef{freecol-developers.mbox_1746}{BAY139-F345FB69E494CF50D1C0BBFE9130\%40phx.gbl}
\@namedef{freecol-developers.mbox_1747}{200706190108.14221.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1749}{20070619062521.120950\%40gmx.net}
\@namedef{freecol-developers.mbox_1750}{20070619094705.2263c394.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1748}{87y7igom1w.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1755}{4fb797ba0706190218k6caae686u89464f65e2d656fc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1760}{45822.193.157.182.68.1182259689.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1751}{28194.6695.qm\%40web86803.mail.ukl.yahoo.com}
\@namedef{freecol-developers.mbox_1752}{BAY139-F35DD87D7E1E0A5FE67C5FCE9120\%40phx.gbl}
\@namedef{freecol-developers.mbox_1753}{BAY139-F29080BF604DCA176E76BF7E9120\%40phx.gbl}
\@namedef{freecol-developers.mbox_1758}{54655.193.157.182.68.1182258822.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1763}{200706192232.45809.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1754}{BAY139-F38A671AE5FF8009D2F17C6E9120\%40phx.gbl}
\@namedef{freecol-developers.mbox_1756}{422040.12790.qm\%40web86807.mail.ukl.yahoo.com}
\@namedef{freecol-developers.mbox_1757}{87odjcnrb9.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1759}{387259.92434.qm\%40web86802.mail.ukl.yahoo.com}
\@namedef{freecol-developers.mbox_1761}{34347.193.157.182.68.1182260054.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1762}{87fy4onfmh.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1764}{48497.193.157.180.58.1182285863.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1766}{877ipzodl5.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1767}{33311.193.157.180.58.1182287981.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1765}{200706192305.29778.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1768}{200706200000.29317.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1769}{001f01c7b2cf$ad55bc40$bf2eafbe\%40tolw}
\@namedef{freecol-developers.mbox_1770}{200706200244.26206.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1775}{46794ADA.1000702\%40gmx.de}
\@namedef{freecol-developers.mbox_1782}{200706202155.08851.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1772}{87wsxyn1l2.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1777}{46794389.7060006\%40gmx.de}
\@namedef{freecol-developers.mbox_1773}{87sl8mmyyz.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1779}{46795214.6090506\%40gmx.de}
\@namedef{freecol-developers.mbox_1784}{51182.129.240.169.83.1182523323.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1785}{467BEEB7.40709\%40gmx.de}
\@namedef{freecol-developers.mbox_1787}{60812.129.240.169.83.1182527603.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1783}{200706202224.36033.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1789}{467BFC47.5050605\%40gmx.de}
\@namedef{freecol-developers.mbox_1790}{467C2D8F.5040701\%40naturalsolutions.cc}
\@namedef{freecol-developers.mbox_1791}{87wsxuvg1e.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1792}{fd6345820706240339g12e010b5p83934c60966b3847\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1793}{467E770B.9030409\%40gmx.de}
\@namedef{freecol-developers.mbox_1794}{fd6345820706240704u87e51c5oc8dcc81b71140418\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1803}{200706251938.42468.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_1795}{87veddt7op.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1796}{fd6345820706241343i6f4ef665id1111df74d421182\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1797}{87r6o1t6sh.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1798}{87myyots0l.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1799}{44849.80.213.130.36.1182762089.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1800}{E1I2krt-00018f-Eh\%40lucky.acegi.com.au}
\@namedef{freecol-developers.mbox_1801}{87ejk0tl64.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1802}{877ipstioz.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1804}{200706251952.29219.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1806}{87ps3jseg2.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1813}{87abulsqx8.fsf_-_\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1814}{fd6345820706270317g7449a4e7jbb96e3c4ebb8a73c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1805}{200706252243.42482.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1807}{46809A70.7030408\%40gmx.de}
\@namedef{freecol-developers.mbox_1810}{B1EA7726-A869-498C-BC31-D1A4B5C3171B\%40gmail.com}
\@namedef{freecol-developers.mbox_1811}{002801c7b818$79488470$d26e2253\%40wiyuo.cegjl}
\@namedef{freecol-developers.mbox_1812}{4681b331.1420720a.115c.ffffa379\%40mx.google.com}
\@namedef{freecol-developers.mbox_1815}{87k5tnqda7.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1816}{87fy4bqd5k.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1817}{46860795.20703\%40gmx.de}
\@namedef{freecol-developers.mbox_1818}{874pkpqpt9.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1819}{87y7hz0xvn.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1820}{7e1e936bd1089d82834d0bf48494d20f\%40localhost}
\@namedef{freecol-developers.mbox_1821}{468A7649.5090800\%40gmx.de}
\@namedef{freecol-developers.mbox_1822}{200707032023.25815.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1823}{200707040117.56468.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1824}{200707040310.08542.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1825}{468AFBD6.8070601\%40yahoo.co.uk}
\@namedef{freecol-developers.mbox_1826}{002101c7be11$1a770e40$61a5c5e1\%40vgie.sz}
\@namedef{freecol-developers.mbox_1827}{50404.129.240.169.78.1183630421.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1828}{59380.193.157.180.58.1183752628.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1829}{55806.193.157.180.58.1183754171.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1830}{4690CF85.2070704\%40gmx.de}
\@namedef{freecol-developers.mbox_1833}{35757.129.240.176.48.1183978998.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1834}{46924B07.4060506\%40gmx.de}
\@namedef{freecol-developers.mbox_1831}{fd6345820707081415h7a419752p750caee535915ddf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1832}{000501c7c1fb$c3a808f0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1835}{200707102137.07849.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1836}{C22A5F5B-F7BD-4A6C-AAE3-CBB560E496A1\%40internode.on.net}
\@namedef{freecol-developers.mbox_1838}{48756.80.213.130.36.1184238573.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1837}{EDBC7DA2-C47F-470D-ACD8-983AB44A1DAF\%40internode.on.net}
\@namedef{freecol-developers.mbox_1839}{46962DE3.6080601\%40kp.org}
\@namedef{freecol-developers.mbox_1840}{55959.80.213.130.36.1184322000.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1841}{44032.80.213.130.36.1184339278.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1842}{34284.80.213.130.36.1184350984.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1843}{001401c7c5f9$928ed030$be4abdda\%40nb.wa}
\@namedef{freecol-developers.mbox_1844}{4698B654.6050103\%40xerox.com}
\@namedef{freecol-developers.mbox_1845}{4698E5B3.1050801\%40gmx.de}
\@namedef{freecol-developers.mbox_1846}{000301c7c648$a1a860a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1847}{469A4DAB.1070804\%40bseindia.com}
\@namedef{freecol-developers.mbox_1848}{469A5C04.2050108\%40designaxiom.com}
\@namedef{freecol-developers.mbox_1849}{87ps2t6vf6.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1850}{469DBEF7.5070501\%40kuoni.ch}
\@namedef{freecol-developers.mbox_1851}{001401c7c9e7$e28bce70$be4abdda\%40cjy.ndjpa}
\@namedef{freecol-developers.mbox_1852}{46A23BFA.1000607\%40gmx.de}
\@namedef{freecol-developers.mbox_1853}{46A31CD5.2050407\%40indigo.ie}
\@namedef{freecol-developers.mbox_1854}{fd6345820707220414m2495e29xf7571b22bf2feda3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1855}{46A36A48.5070502\%40gmx.de}
\@namedef{freecol-developers.mbox_1856}{87lkd730zi.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1857}{c2dd2ee70707231649m4b09e46cpb2ea71074b01d3fd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1861}{46A57F4C.5030805\%40gmx.de}
\@namedef{freecol-developers.mbox_1862}{c2dd2ee70707232221i6337bec4y2428f07acbcc3a9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1869}{87sl7d22vi.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1870}{fd6345820707240919h2f1f0926iefdfb8119914d078\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1872}{c2dd2ee70707241054o49d04984o693242ee420542d6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1877}{54689.129.240.176.48.1185376564.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1876}{38487.129.240.176.48.1185374245.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1871}{7bd504520707240930m2d40f34fxad8c2d724fe26a68\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1875}{33833.129.240.176.48.1185373420.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1858}{200707240418.23469.DHerding\%40gmx.de}
\@namedef{freecol-developers.mbox_1859}{871wey34ga.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1860}{c2dd2ee70707232002i7d856c82p3ec330245dbddb76\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1866}{fd6345820707240352w15100c1au12c0e2ae5d42db15\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1863}{48285a810707240044m1c929843ue2cf1c5e0bee1eb7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1864}{48285a810707240049v13f91e46lae0b4c0d3e0a697a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1868}{c2dd2ee70707240556m2e03f3f3l33c02093df03b1ce\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1865}{48285a810707240054t114be82fn277b1fa35c74f5a0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1867}{fd6345820707240420j7eeae585h3ee3125b2f18cc26\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1873}{000901c7ce3e$39c9d010$2a91de9d\%40cafg.gz}
\@namedef{freecol-developers.mbox_1874}{000601c7ce95$cf3f9c90$8d6090b9\%40pnoer.ga}
\@namedef{freecol-developers.mbox_1878}{50972.129.240.169.51.1185449058.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1881}{20070727004614.4c2c93ad.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1879}{87y7h3z67o.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1880}{46A8BE47.2050602\%40gmx.de}
\@namedef{freecol-developers.mbox_1882}{c2dd2ee70707262041g3a1fb967w60f3c63213da7f2a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1883}{c2dd2ee70707270806u4a777d56h16bcddeb24412d41\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1884}{87tzrpzbdr.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1885}{c2dd2ee70707271822q1ba4450aw6ac4d018ea7415a8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1886}{46AB01EF.2060608\%40gmx.de}
\@namedef{freecol-developers.mbox_1887}{c2dd2ee70707280210n1d66d2e3rfdc526264ef02b0d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1888}{46AB1162.5030700\%40gmx.de}
\@namedef{freecol-developers.mbox_1895}{58083.129.240.176.48.1185804804.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1897}{c2dd2ee70707310608g125f97f4h9785af077b390f58\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1898}{46AF4F46.20406\%40gmx.de}
\@namedef{freecol-developers.mbox_1900}{42227.80.213.130.36.1186069595.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1904}{20070803071054.268130\%40gmx.net}
\@namedef{freecol-developers.mbox_1952}{c2dd2ee70708120831m7799fefds616508b260ffc0a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1954}{46C00F1D.2040204\%40gmx.de}
\@namedef{freecol-developers.mbox_1960}{c2dd2ee70708130810n7618748dy438d656a7abbb7c2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1962}{46C07FB6.3090305\%40gmx.de}
\@namedef{freecol-developers.mbox_1975}{c2dd2ee70708140827s1e953774t563249b38fabface\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1976}{c2dd2ee70708140840t6667b376j4dbc0a99f7453bda\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2010}{42158.80.35.36.227.1187602888.squirrel\%40correo.ensanjose.net}
\@namedef{freecol-developers.mbox_2011}{c2dd2ee70708200328r13d98349y41337b913134d432\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2012}{af64eac02ebea2770f0bbb251854ef2d\%40localhost}
\@namedef{freecol-developers.mbox_2013}{c2dd2ee70708200516x641bdfebw97c47ca52791c377\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1899}{42222.80.213.130.36.1186069487.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1901}{c2dd2ee70708021106p47fac7bm6adb12218f71a1e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1902}{87bqdp3f54.fsf\%40giorgian.widge.org}
\@namedef{freecol-developers.mbox_1903}{c2dd2ee70708021640u79c69924s96cafb2ee276956a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1889}{46ABD50E.8030605\%40woh.rr.com}
\@namedef{freecol-developers.mbox_1890}{B37CDC4F-5DCE-4FC3-91DA-E5CA3591360A\%40internode.on.net}
\@namedef{freecol-developers.mbox_1891}{46AC4AFD.1070809\%40gmx.de}
\@namedef{freecol-developers.mbox_1892}{d8cfd2b50707290226g5132393bn43254a9ca3b5abbd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1893}{46AC6853.4090203\%40gmx.de}
\@namedef{freecol-developers.mbox_1894}{001901c7d1ee$ccaadd80$5783cd32\%40kfrgz.eucyc}
\@namedef{freecol-developers.mbox_1896}{001601c7d2f5$6055e190$4b392982\%40yo.qglq}
\@namedef{freecol-developers.mbox_1905}{46B45FA7.8060108\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1906}{46B47901.70502\%40free.fr}
\@namedef{freecol-developers.mbox_1916}{46B9B7A0.4030304\%40gmx.de}
\@namedef{freecol-developers.mbox_1917}{1186595577.8910.1.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_1907}{20070805140630.3X6X9.560544.root\%40webfep12}
\@namedef{freecol-developers.mbox_1908}{E1IHnFy-0005Je-8b\%40sc8-sf-web22.sourceforge.net}
\@namedef{freecol-developers.mbox_1909}{200708062104.03967.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1915}{46B9A822.8010405\%40gmx.de}
\@namedef{freecol-developers.mbox_1910}{1186455947.19944.16.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_1912}{002201c7d8c7$a9c06bc0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1911}{46b80b63.1de.71f1.20860\%40internode.on.net}
\@namedef{freecol-developers.mbox_1914}{1186495568.13012.14.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_1913}{46141.80.213.130.36.1186492521.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1918}{f781b8720708091109n253818c1u29d7b75bdd433164\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1921}{46BC13A6.1020502\%40gmx.de}
\@namedef{freecol-developers.mbox_1922}{f781b8720708100628n6fcfb3d7ic89583da275cc37c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1923}{46BC79A1.2080808\%40gmx.de}
\@namedef{freecol-developers.mbox_1932}{f781b8720708102228v767ac6b2j1008905f5f1225f6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1933}{46BD561E.1000807\%40gmx.de}
\@namedef{freecol-developers.mbox_1943}{f781b8720708110958t5fd27aa9jc6caf47e9a27ce30\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1946}{46BEBF0F.40309\%40gmx.de}
\@namedef{freecol-developers.mbox_1951}{f781b8720708120801h366b5c22wf13f9300be5a958\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1955}{46C01071.4010807\%40gmx.de}
\@namedef{freecol-developers.mbox_1961}{c2dd2ee70708130851h319bb34as8019c204bb3e6797\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1968}{f781b8720708131526o350e2e27t7d94de27ba43de39\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2079}{c2dd2ee70708251056n732a73a1meb3919232c00173\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2083}{f781b8720708252138s62c7a745icdcbad50d9e96676\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2041}{200708222112.44722.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2042}{46CC965F.30005\%40gmx.de}
\@namedef{freecol-developers.mbox_1944}{20070811203150.f013c724.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1919}{001101c7dad5$902d3700$199c4033\%40iykdn.qxbd}
\@namedef{freecol-developers.mbox_1920}{f781b8720708100020j39cf545ld978dbca4a395995\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1924}{002601c7db63$e6728aa0$8fa4b0d5\%40hhbql.jeobu}
\@namedef{freecol-developers.mbox_1925}{46BC8870.6020202\%40gmx.de}
\@namedef{freecol-developers.mbox_1926}{46BC90E4.5030202\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1936}{46BD9235.9030002\%40gmx.de}
\@namedef{freecol-developers.mbox_1927}{200708110122.19106.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1935}{46BD6819.2040002\%40gmx.de}
\@namedef{freecol-developers.mbox_1928}{f781b8720708101709n140315aeif1ca2a26d4287311\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1930}{c2dd2ee70708101916m2a6c4504u407d1263ebb173ee\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1931}{f781b8720708102218m41653050mc575a0b51c79ef7a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1938}{200708111513.02200.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1940}{c2dd2ee70708110801j9eb7215ree6437d350a82399\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1942}{f781b8720708110942y744b7daao567bedebec7b6443\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1947}{46BEBF83.3070807\%40gmx.de}
\@namedef{freecol-developers.mbox_1948}{20070812115548.e87ee17b.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1953}{f781b8720708122042u7df265f2y1f9dc24630cdd788\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1934}{46BD58A1.8030401\%40gmx.de}
\@namedef{freecol-developers.mbox_1929}{f781b8720708101825j4a22a05dl7de0624eef9570cd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1937}{200708111505.41167.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1939}{f781b8720708110732h278bec46l5e5040dad95b4f5e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1941}{f781b8720708110918h32643163x26e70c6bd52bd1c1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1945}{001101c7dcb2$7c7c2a70$5f42b0ed\%40xexjs}
\@namedef{freecol-developers.mbox_1949}{20070812151736.d0c6b2af.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1950}{46BEFCA7.2080603\%40gmx.de}
\@namedef{freecol-developers.mbox_1956}{1129.4447.qm\%40web52904.mail.re2.yahoo.com}
\@namedef{freecol-developers.mbox_1957}{46C03FA0.2080802\%40gmx.de}
\@namedef{freecol-developers.mbox_1958}{20070813142447.6619ab3b.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1959}{60573.193.157.182.115.1187008150.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1963}{53225.80.213.130.36.1187023079.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1964}{c2dd2ee70708131313u18472aadh73996ea5f252a4e2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1965}{54749.80.213.130.36.1187038303.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1966}{c2dd2ee70708131421xdb1cc12m1180547af3d6a3a7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1970}{46C15D36.1020400\%40gmx.de}
\@namedef{freecol-developers.mbox_1971}{200708141245.30159.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1967}{002801c7ddee$d6b8f8f0$d1708d77\%40to.wdanz}
\@namedef{freecol-developers.mbox_1969}{001401c7de28$e1610b00$e791bf60\%40qlpsk.eb}
\@namedef{freecol-developers.mbox_1972}{38314.193.157.182.115.1187102313.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1973}{20070814174503.ead1dc76.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1974}{42540.193.157.182.115.1187105269.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1977}{20070814183841.c5652d2f.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_1980}{003001c7de96$e2d355b0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1982}{43565.193.157.182.115.1187113138.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1983}{c2dd2ee70708141048w2299b6b9m152d04f5a51bf66a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1987}{200708151230.20388.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1978}{9E7E8803-F5D0-412D-A536-BC76F6B47CCF\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1981}{003101c7de98$349b59a0$0300a8c0\%40codemint.com}
\@namedef{freecol-developers.mbox_1984}{E9DA2B65-D40C-4919-99E7-91BE8143D887\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_1979}{12148012.post\%40talk.nabble.com}
\@namedef{freecol-developers.mbox_1986}{4fb797ba0708150204m7b1a390dt8839814b4abb7f22\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1985}{60532.129.240.176.50.1187116691.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1988}{55542.193.157.182.115.1187181014.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1989}{42239.193.157.182.115.1187187178.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1990}{46C30D87.2010402\%40gmx.de}
\@namedef{freecol-developers.mbox_1991}{59324.193.157.180.58.1187261551.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_1992}{BAY110-W19D0C81DC8EC1B72DD6594C2DF0\%40phx.gbl}
\@namedef{freecol-developers.mbox_1993}{6e4284620708171014j37714658m7170077ad84fbbf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_1994}{46C69D0E.408\%40gmx.de}
\@namedef{freecol-developers.mbox_1995}{200708182226.58393.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1999}{46C7EC8E.2020605\%40gmx.de}
\@namedef{freecol-developers.mbox_2002}{200708192006.22208.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2008}{46C94075.2050004\%40gmx.de}
\@namedef{freecol-developers.mbox_1996}{200708182317.05993.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_1997}{c2dd2ee70708181751v413fdc56hfe9b7d14937f9df7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2000}{46C7ED7C.8080706\%40gmx.de}
\@namedef{freecol-developers.mbox_1998}{46C7E9EE.5050801\%40gmx.de}
\@namedef{freecol-developers.mbox_2001}{c2dd2ee70708190814u4dce347aoaacfe92cd74054c5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2004}{4fb797ba0708191352l22fff12bs35dec9ca028000ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2003}{200708192016.17909.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2005}{20070820005115.d136a15e.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2006}{200708200002.56106.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2007}{000801c7e2ad$5638a180$6886c0ea\%40tclkt}
\@namedef{freecol-developers.mbox_2009}{46C9455B.7000200\%40gmx.de}
\@namedef{freecol-developers.mbox_2014}{200708202055.13748.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2016}{c2dd2ee70708202022i50de8874ld973f550e383f28d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2017}{46CA91DA.4010908\%40gmx.de}
\@namedef{freecol-developers.mbox_2015}{1INK4J-000X5Y-SE\%4027.126.188.72.cfl.res.rr.com}
\@namedef{freecol-developers.mbox_2018}{d4b2fefd2e430d89427f89db5af25c73\%40localhost}
\@namedef{freecol-developers.mbox_2019}{46CAA27F.1080706\%40gmx.de}
\@namedef{freecol-developers.mbox_2020}{7bf807ee211633db24bf277f039b5582\%40localhost}
\@namedef{freecol-developers.mbox_2021}{46CAAFA3.9040306\%40gmx.de}
\@namedef{freecol-developers.mbox_2022}{c7f70fd8a15250fc43bc9c7d1548fc66\%40localhost}
\@namedef{freecol-developers.mbox_2023}{36452.193.157.182.115.1187705247.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2025}{c2dd2ee70708212005u3549cb46xbafc0795d36ead74\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2028}{46CBDE5D.8080304\%40gmx.de}
\@namedef{freecol-developers.mbox_2031}{48646.80.35.36.227.1187768227.squirrel\%40correo.ensanjose.net}
\@namedef{freecol-developers.mbox_2037}{c2dd2ee70708220542t2ddfb225w29f9576187f322cf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2039}{60e1d1a78ad2de88ae86fe3c1ebfc106\%40localhost}
\@namedef{freecol-developers.mbox_2027}{46CBDB5A.6010105\%40gmx.de}
\@namedef{freecol-developers.mbox_2024}{200708220155.04034.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2026}{c2dd2ee70708212048q7f86d736o56664b7bb669842b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2030}{48641.80.35.36.227.1187768149.squirrel\%40correo.ensanjose.net}
\@namedef{freecol-developers.mbox_2038}{c2dd2ee70708220552y4dc58d31pa5887359b86fa40e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2040}{ac773b92746b2c8a083b8a46fc06aee1\%40localhost}
\@namedef{freecol-developers.mbox_2047}{c2dd2ee70708221724v34a14399t7aabd8bd628bf4e0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2050}{200708230321.41117.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2053}{c2dd2ee70708221951l5aff7698kbe567e399c34ad72\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2055}{46CD43E5.1060908\%40gmx.de}
\@namedef{freecol-developers.mbox_2063}{250aecb5c9dfdfc8d568d231d4e7d583\%40localhost}
\@namedef{freecol-developers.mbox_2066}{46CD954C.3000002\%40gmx.de}
\@namedef{freecol-developers.mbox_2057}{36068.193.157.188.13.1187858760.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2056}{45821.193.157.188.13.1187858533.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2058}{46CD4A43.9050003\%40gmx.de}
\@namedef{freecol-developers.mbox_2060}{59256.193.157.188.13.1187861765.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2062}{46CD5A5C.3040401\%40gmx.de}
\@namedef{freecol-developers.mbox_2065}{33389.193.157.188.13.1187872628.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2067}{46CD965C.8090808\%40gmx.de}
\@namedef{freecol-developers.mbox_2064}{fd8fd68c051d3f2dc0eab3ed21a5ac5b\%40localhost}
\@namedef{freecol-developers.mbox_2059}{56232.193.157.188.13.1187859403.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2029}{48394.80.35.36.227.1187767205.squirrel\%40correo.ensanjose.net}
\@namedef{freecol-developers.mbox_2032}{2dab487e675261dba6946266124cfad9\%40localhost}
\@namedef{freecol-developers.mbox_2033}{46CC0749.70608\%40gmx.de}
\@namedef{freecol-developers.mbox_2034}{4514111ead00513ecb697de18ba639e5\%40localhost}
\@namedef{freecol-developers.mbox_2035}{88c9c1727a993999b5e059a6a50238a5\%40localhost}
\@namedef{freecol-developers.mbox_2036}{46CC2183.2080405\%40gmx.de}
\@namedef{freecol-developers.mbox_2043}{000601c7e4ff$c6bb5e30$0201a8c0\%40GeneralEric}
\@namedef{freecol-developers.mbox_2061}{43111.193.157.188.13.1187862579.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2044}{200708222305.24628.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2046}{c2dd2ee70708221657i55f6b9dcja4d8576dbf21fe94\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2049}{200708230307.39593.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2045}{1IOJ-000N16-I6\%40adsl-220-100-217.mcn.bellsouth.net}
\@namedef{freecol-developers.mbox_2048}{200708230302.27744.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2054}{46CD4065.3030604\%40gmx.de}
\@namedef{freecol-developers.mbox_2051}{200708230322.24111.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2052}{000d01c7e489$4e97eb60$a6ab90d1\%40znv.zh}
\@namedef{freecol-developers.mbox_2068}{46CEAEE2.10106\%40gmx.de}
\@namedef{freecol-developers.mbox_2069}{c2dd2ee70708240552n6a3cae60qcd9b2bc7de246e81\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2070}{200708241757.57394.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2071}{46CFDDB4.1010903\%40gmx.de}
\@namedef{freecol-developers.mbox_2075}{200708251652.16437.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2072}{c2dd2ee70708250708t254531fepde85e9e8d8235feb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2073}{c2dd2ee70708250717i40ffd1eaw80ef074027bf8b47\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2074}{200708251647.13366.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2076}{c2dd2ee70708250854l30f0a792l292bae0e6129fde3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2077}{46D052B5.40506\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2078}{c2dd2ee70708251025r1233bcb7ka2cc516f55c3faf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2080}{200708252015.22340.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2154}{200709050042.58646.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2081}{1IP41\%40-0009G4-DY\%40188.106.broadband4.iol.cz}
\@namedef{freecol-developers.mbox_2082}{20070826031542.1fcfcdab.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2084}{46D12D67.1010400\%40gmx.de}
\@namedef{freecol-developers.mbox_2085}{46D13E95.7080407\%40gmx.de}
\@namedef{freecol-developers.mbox_2086}{c2dd2ee70708260502h5dbdefdbme517c2b8491376b9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2087}{c2dd2ee70708260840s3831644dx256ba8d7c39f8a8a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2088}{200708262212.24974.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2090}{c2dd2ee70708261740h30ddad8mcfeb6dba04684970\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2092}{46D25B6C.8050002\%40gmx.de}
\@namedef{freecol-developers.mbox_2096}{c2dd2ee70708270329o73e3d128hd7f1d4d5d8304e26\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2097}{c2dd2ee70708270350k6ea6e2faie4331476b8a28d0d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2120}{200708301223.18009.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2123}{c2dd2ee70708300554gb72f4c1vaf3890c6ddc73832\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2089}{200708270148.15120.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2091}{c2dd2ee70708261747n51c1d294n7a3069e483433e59\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2094}{46D25E61.1060204\%40gmx.de}
\@namedef{freecol-developers.mbox_2095}{15b6c59b784a03c0713064924188880e\%40localhost}
\@namedef{freecol-developers.mbox_2098}{c2dd2ee70708270418t3db02617rb5021862e1986a00\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2099}{46D2D624.7010705\%40gmx.de}
\@namedef{freecol-developers.mbox_2100}{c2dd2ee70708280555w72b1f251vea7995d967389de\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2101}{46D42340.4000203\%40gmx.de}
\@namedef{freecol-developers.mbox_2107}{c2dd2ee70708281809j438df9b9m7651544ba6a6bf5b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2108}{c2dd2ee70708281954w2ddd2750wef980af680dc24f6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2110}{46D50313.6050408\%40gmx.de}
\@namedef{freecol-developers.mbox_2112}{c2dd2ee70708290612u294c5e5ds752726ea209a8de7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2093}{1IQ\%40u7-000WIB-JX\%40wcct}
\@namedef{freecol-developers.mbox_2102}{46D426FA.1030501\%40gmx.de}
\@namedef{freecol-developers.mbox_2103}{44509.129.240.176.35.1188310498.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2104}{46D430A1.4050502\%40gmx.de}
\@namedef{freecol-developers.mbox_2106}{34030.193.157.182.115.1188319139.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2109}{46D4FE01.2080707\%40gmx.de}
\@namedef{freecol-developers.mbox_2119}{200708301222.27130.sergio\%40entrecables.com}
\@namedef{freecol-developers.mbox_2128}{46D7A557.6030901\%40gmx.de}
\@namedef{freecol-developers.mbox_2139}{46D94D44.2010701\%40gmx.de}
\@namedef{freecol-developers.mbox_2145}{200709020013.02820.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2121}{200708301241.40345.sergio\%40entrecables.com}
\@namedef{freecol-developers.mbox_2159}{46E24B26.9060500\%40gmx.de}
\@namedef{freecol-developers.mbox_2160}{46066.80.213.133.26.1189237579.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2164}{46E2C144.8050402\%40gmx.de}
\@namedef{freecol-developers.mbox_2105}{op.txrxcric2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2111}{46D56DCE.5080204\%40gmx.de}
\@namedef{freecol-developers.mbox_2113}{52413.193.157.182.115.1188393602.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2114}{46D573AD.2010809\%40gmx.de}
\@namedef{freecol-developers.mbox_2115}{60210.193.157.182.115.1188394871.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2116}{46D57834.6040606\%40gmx.de}
\@namedef{freecol-developers.mbox_2117}{6C0C5B5C-D8AC-4AFE-9DCD-5E87D8EF07BC\%40us.army.mil}
\@namedef{freecol-developers.mbox_2118}{86761772-216C-4B18-A910-5D61D4F1F8CD\%40binary.is}
\@namedef{freecol-developers.mbox_2122}{200708301254.46606.sergio\%40entrecables.com}
\@namedef{freecol-developers.mbox_2124}{e092c130708300741i60ef75dcy25adf7ef749b9510\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2127}{46D7A13A.2010600\%40gmx.de}
\@namedef{freecol-developers.mbox_2125}{200708302304.07308.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2126}{46D79E02.7020400\%40gmx.de}
\@namedef{freecol-developers.mbox_2129}{8fc07158df1870a5d27d873d6b00272d\%40localhost}
\@namedef{freecol-developers.mbox_2130}{20070831093321.116950\%40gmx.net}
\@namedef{freecol-developers.mbox_2131}{8f5fe9bfd6fae04039dde3b213d4bcbb\%40localhost}
\@namedef{freecol-developers.mbox_2132}{200708312003.11749.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2133}{200708312246.44322.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2135}{46D90F7F.6040701\%40gmx.de}
\@namedef{freecol-developers.mbox_2134}{000401c7ec25$2d92d0d0$6e1821ec\%40cuhvd}
\@namedef{freecol-developers.mbox_2136}{46D93968.8010109\%40gmx.de}
\@namedef{freecol-developers.mbox_2137}{200709011237.49192.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2138}{46D9461F.1020502\%40gmx.de}
\@namedef{freecol-developers.mbox_2140}{200709011335.55518.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2141}{46D95302.8080109\%40gmx.de}
\@namedef{freecol-developers.mbox_2142}{200709011751.19132.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2143}{46D9914F.6070708\%40gmx.de}
\@namedef{freecol-developers.mbox_2144}{200709011859.46489.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2146}{46DA677B.1050604\%40gmx.de}
\@namedef{freecol-developers.mbox_2153}{200709050019.51295.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2156}{46DEBFC3.4020402\%40gmx.de}
\@namedef{freecol-developers.mbox_2147}{46DAA513.3040104\%40invista.com}
\@namedef{freecol-developers.mbox_2148}{46DC0F6E.4050802\%40innerheight.com}
\@namedef{freecol-developers.mbox_2149}{72113A47-D434-496A-8638-93E262E55637\%40binary.is}
\@namedef{freecol-developers.mbox_2150}{46DC4A08.2070308\%40gmx.de}
\@namedef{freecol-developers.mbox_2151}{7b94298e0709031122p579c64dq2e4c3f7f43c1d39f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2152}{20070904051837.123670\%40gmx.net}
\@namedef{freecol-developers.mbox_2155}{0BB620E12B356B48A6E16F18E3B3966334B135\%40senn5.int.enbnn.ru}
\@namedef{freecol-developers.mbox_2157}{46DF2B35.6060203\%40wldcup.com}
\@namedef{freecol-developers.mbox_2158}{46E1494B.2060001\%40peppermillcas.com}
\@namedef{freecol-developers.mbox_2161}{46E26449.7010308\%40gmx.de}
\@namedef{freecol-developers.mbox_2162}{46E2C0E9.6010507\%40gmx.de}
\@namedef{freecol-developers.mbox_2163}{200709081815.36745.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2165}{46E38556.7020806\%40gmx.de}
\@namedef{freecol-developers.mbox_2166}{46E4F0C4.7080000\%40suttonpl.com}
\@namedef{freecol-developers.mbox_2167}{000301c7f460$ed625230$da6b38da\%40ayge}
\@namedef{freecol-developers.mbox_2168}{20070911121337.136950\%40gmx.net}
\@namedef{freecol-developers.mbox_2172}{43164.80.213.133.26.1189514994.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2176}{200709111947.08978.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2178}{c2dd2ee70709112132j406a3266j450dad60c66e1ccf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2169}{20070911121832.136960\%40gmx.net}
\@namedef{freecol-developers.mbox_2171}{52265.80.213.133.26.1189514339.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2173}{20070911152554.67610\%40gmx.net}
\@namedef{freecol-developers.mbox_2174}{200709111940.13476.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2180}{46E77FD9.1020505\%40gmx.de}
\@namedef{freecol-developers.mbox_2170}{20070911122608.136960\%40gmx.net}
\@namedef{freecol-developers.mbox_2175}{200709111945.28720.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2177}{41637.80.213.133.26.1189539298.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2179}{46E77E6B.4080103\%40gmx.de}
\@namedef{freecol-developers.mbox_2181}{001c01c7f50f$8358add0$7d62d2b6\%40auc}
\@namedef{freecol-developers.mbox_2182}{op.tyjf0tu72817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2185}{20070912151401.176290\%40gmx.net}
\@namedef{freecol-developers.mbox_2186}{58481.80.213.133.26.1189610137.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2189}{op.tyjwssrj2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2191}{46E8C25B.9050806\%40gmx.de}
\@namedef{freecol-developers.mbox_2183}{c6fb1aad6a9bab70708b3193c4d3b059\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2188}{40409.80.213.133.26.1189610970.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2192}{46E8C2B2.1020808\%40gmx.de}
\@namedef{freecol-developers.mbox_2184}{c9a6f7dbd48f55558d90ea300e22777f\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2187}{20070912151840.176280\%40gmx.net}
\@namedef{freecol-developers.mbox_2190}{200709122354.23202.sergio\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2193}{op.tyk0ln2p2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2194}{op.tyk1oifq2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2195}{20070913090910.236680\%40gmx.net}
\@namedef{freecol-developers.mbox_2196}{op.tyk5j1cy2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2197}{20070913120922.12430\%40gmx.net}
\@namedef{freecol-developers.mbox_2198}{35CBE00E-2B2D-4EC4-8E88-D8507AA0AA8D\%40binary.is}
\@namedef{freecol-developers.mbox_2230}{52841.193.157.182.17.1190121521.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2199}{37514.129.240.169.86.1189693444.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2224}{49841.193.157.180.189.1190038419.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2225}{200709180013.08204.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2227}{20070918062331.152860\%40gmx.net}
\@namedef{freecol-developers.mbox_2228}{20070918002011.504b6025.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2200}{20070913144043.131810\%40gmx.net}
\@namedef{freecol-developers.mbox_2205}{f781b8720709131518y315830e6yfe86a23f1eda6ce\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2206}{200709140036.14041.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2207}{f781b8720709132017x5a458a97jde94d0bc8e46ec99\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2213}{1abf3356b356313cbd469ec7b4e58b80\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2216}{f781b8720709140846u5f6a3ab5ob399c99de275cead\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2221}{46EB9095.9000703\%40gmx.de}
\@namedef{freecol-developers.mbox_2226}{f781b8720709171559t7a216f51i842746eee676a6f5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2201}{41156.193.157.182.26.1189697081.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2209}{46EA1F0E.808\%40gmx.de}
\@namedef{freecol-developers.mbox_2211}{58031.129.240.169.86.1189761738.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2218}{C2EFA0AF-BF89-4760-B53F-E62EAAAC20BE\%40internode.on.net}
\@namedef{freecol-developers.mbox_2202}{48768.129.240.176.64.1189710663.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2208}{46EA1B34.6050701\%40gmx.de}
\@namedef{freecol-developers.mbox_2210}{44063.129.240.169.86.1189760539.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2203}{BAY115-F31D58D8FC7D5D9BA7FD74AABC30\%40phx.gbl}
\@namedef{freecol-developers.mbox_2204}{200709140016.11655.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2212}{op.tym0vez52817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2219}{c2dd2ee70709142055q502508cbj8f2e10dc40b73188\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2232}{op.tyypilsb2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2214}{20070914113929.277880\%40gmx.net}
\@namedef{freecol-developers.mbox_2217}{200709142014.01080.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2220}{46EB8B83.5050704\%40gmx.de}
\@namedef{freecol-developers.mbox_2215}{000e01c7f6e1$898bbf20$8202a8c0\%4024J5HTWFKO2345}
\@namedef{freecol-developers.mbox_2222}{46EB96CE.2040609\%40gmx.de}
\@namedef{freecol-developers.mbox_2229}{33043.193.157.182.17.1190120727.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2255}{7b94298e0709281132q5ffcee4cj98ae8add2eb61bb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2223}{000d01c7f821$88546530$95cfea1c\%40algf}
\@namedef{freecol-developers.mbox_2231}{40408.193.157.180.189.1190235127.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2233}{46F34B7E.9010007\%40murtos.com}
\@namedef{freecol-developers.mbox_2234}{46F3EED4.7040906\%40gmx.de}
\@namedef{freecol-developers.mbox_2235}{54971.193.157.182.42.1190621894.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2247}{46F937C4.5000603\%40murtos.com}
\@namedef{freecol-developers.mbox_2236}{56148.129.240.176.123.1190647505.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2237}{46F7E3F6.3060700\%40gmx.de}
\@namedef{freecol-developers.mbox_2238}{7b94298e0709240941s1b265ceekaf891ad62c55a246\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2239}{46F7EA7D.3040904\%40gmx.de}
\@namedef{freecol-developers.mbox_2241}{20070924222004.383b6c60.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2245}{53402.129.240.169.52.1190731572.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2246}{20070925192729.498725ee.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2248}{59443.193.157.182.101.1190802186.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2240}{op.ty57nb2k2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2244}{20070925064951.24520\%40gmx.net}
\@namedef{freecol-developers.mbox_2242}{op.ty6awq0k2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2243}{20070925064911.24490\%40gmx.net}
\@namedef{freecol-developers.mbox_2249}{46FA8EA1.60707\%40gmx.de}
\@namedef{freecol-developers.mbox_2250}{op.ty91rabk2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2259}{46FE08D7.4000509\%40gmx.de}
\@namedef{freecol-developers.mbox_2260}{op.tzesa8f72817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2261}{op.tzes3qmb2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2264}{46FE531D.5060004\%40gmx.de}
\@namedef{freecol-developers.mbox_2262}{46FE1D57.7030203\%40gmx.de}
\@namedef{freecol-developers.mbox_2251}{52030.193.157.182.101.1190903278.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2252}{000601c801e9$30099040$0201a8c0\%40GeneralEric}
\@namedef{freecol-developers.mbox_2256}{200709282335.14606.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2253}{dcfe65cb0709280953wc0cef4bv42f44b2edba35e2b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2254}{1191004044.28541.8.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2257}{200709282335.35308.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2258}{46FE054E.20400\%40gmx.de}
\@namedef{freecol-developers.mbox_2266}{1191184249.5462.5.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2263}{46FE265F.2080108\%40gmx.de}
\@namedef{freecol-developers.mbox_2265}{46FFB41E.2060503\%40gmx.de}
\@namedef{freecol-developers.mbox_2271}{53270.193.157.189.47.1191241418.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2267}{47001B1D.10303\%40debian.org}
\@namedef{freecol-developers.mbox_2268}{47009ABE.2050103\%40gmx.de}
\@namedef{freecol-developers.mbox_2281}{47028FE0.9000104\%40debian.org}
\@namedef{freecol-developers.mbox_2282}{7b94298e0710030943v5d93fb58kf23d9eadec44ef76\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2283}{4703C9AA.1080407\%40gmx.de}
\@namedef{freecol-developers.mbox_2287}{60031.80.213.133.52.1191750190.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2288}{4708DBDF.2090001\%40debian.org}
\@namedef{freecol-developers.mbox_2269}{4700C751.4080407\%40gmx.de}
\@namedef{freecol-developers.mbox_2270}{c2dd2ee70710010439jf84f83pb0e7370f5bf40244\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2272}{1191278284.29928.0.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2273}{BAY102-DAV140717A8C1A22C8443DF2E93AE0\%40phx.gbl}
\@namedef{freecol-developers.mbox_2279}{20071002185624.cb1151cc.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2274}{d597b8ed92d0bdf417b5c244c7b93a52\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2275}{47021214.5000102\%40gmx.de}
\@namedef{freecol-developers.mbox_2280}{20071002185735.aac59ff7.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2284}{f781b8720710041432l760e2b59r1d3f07f27347ca7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2289}{BAY102-DAV6911116B5C97DD93A2CDE93AB0\%40phx.gbl}
\@namedef{freecol-developers.mbox_2276}{002701c804da$7dd87ae0$becf439c\%40dbf}
\@namedef{freecol-developers.mbox_2277}{652043.91541.qm\%40web52904.mail.re2.yahoo.com}
\@namedef{freecol-developers.mbox_2278}{0107ffa4$0107fe78$78b1fc58\%40puk}
\@namedef{freecol-developers.mbox_2285}{470773C2.2020601\%40gmx.de}
\@namedef{freecol-developers.mbox_2286}{60028.80.213.133.52.1191750106.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2290}{47378.193.157.189.47.1191844512.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2291}{20071008133911.266690\%40gmx.net}
\@namedef{freecol-developers.mbox_2294}{470A3445.9070409\%40debian.org}
\@namedef{freecol-developers.mbox_2292}{20071008134050.266650\%40gmx.net}
\@namedef{freecol-developers.mbox_2293}{20071008134223.266690\%40gmx.net}
\@namedef{freecol-developers.mbox_2295}{c2dd2ee70710081015n308259c0ocf1c9e3be24a786d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2296}{470B0C40.20506\%40gmx.de}
\@namedef{freecol-developers.mbox_2297}{470B38FE.8060108\%40debian.org}
\@namedef{freecol-developers.mbox_2301}{470C57E2.80100\%40gmx.de}
\@namedef{freecol-developers.mbox_2298}{20071009153554.MLSV8.162109.root\%40webfep14}
\@namedef{freecol-developers.mbox_2299}{20071009153601.JFGZK.162118.root\%40webfep14}
\@namedef{freecol-developers.mbox_2300}{470C574C.9040902\%40gmx.de}
\@namedef{freecol-developers.mbox_2306}{47143BA3.7020407\%40gmx.de}
\@namedef{freecol-developers.mbox_2309}{200710162306.33310.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2312}{471596EA.9030008\%40gmx.de}
\@namedef{freecol-developers.mbox_2315}{op.t0b112pp2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2323}{47183784.1070005\%40gmx.de}
\@namedef{freecol-developers.mbox_2320}{200710171756.47474.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2302}{471044F7.7060308\%40krinos.com}
\@namedef{freecol-developers.mbox_2303}{001201c80e73$2019f8a0$9f22a92d\%40qzbe}
\@namedef{freecol-developers.mbox_2304}{op.tz8pkvhl2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2305}{200710152252.07650.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2314}{4715995E.70209\%40gmx.de}
\@namedef{freecol-developers.mbox_2307}{517C492D-D968-4BAB-A49A-9D1410B587EF\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_2308}{f7a7c49c0710160644m463dce94ya8fb6deb05c4f675\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2313}{471598CD.6000007\%40gmx.de}
\@namedef{freecol-developers.mbox_2317}{E15959B7-71C6-45D8-A427-9A9E7BC8C616\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_2318}{c2dd2ee70710170546o771799a5g508bd1dfcc75e38f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2322}{065A6448-60D0-4981-A5E8-32CC0C9FA45A\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_2310}{c2dd2ee70710162116y7c9d08ai51bac5c35c3797d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2311}{471595E1.1010400\%40gmx.de}
\@namedef{freecol-developers.mbox_2316}{c2dd2ee70710170318h3f172f73vb76013b378466e62\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2319}{33969.193.157.180.141.1192628899.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2321}{c2dd2ee70710171439h5eb82542h6f5f3397e5fb7578\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2324}{31b861650710201406j7baf66f1u6828d95b5b0c15cc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2325}{471B0040.4000606\%40gmx.de}
\@namedef{freecol-developers.mbox_2326}{01c81668$a8175390$dfb1c2d4\%40cdev}
\@namedef{freecol-developers.mbox_2327}{47208F37.5050407\%40kliaekspres.com}
\@namedef{freecol-developers.mbox_2328}{01c81706$0e05e890$b74e824a\%40vlyxmbk}
\@namedef{freecol-developers.mbox_2329}{4722D5D9.5050403\%40fanitas.com}
\@namedef{freecol-developers.mbox_2330}{02bf01c8186c$624da750$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2331}{1193530878.21925.1.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2332}{472445F2.3080505\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2333}{47245E1A.1010800\%40gmx.de}
\@namedef{freecol-developers.mbox_2334}{1193602077.21827.1.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2335}{1193606969.21827.15.camel\%40openhand.localhost}
\@namedef{freecol-developers.mbox_2336}{20071029084144.321740\%40gmx.net}
\@namedef{freecol-developers.mbox_2337}{002001c81a2c$28c80720$24252349\%40fsvf}
\@namedef{freecol-developers.mbox_2338}{4726CEA5.1050507\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2339}{47283895.5030800\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2340}{200710312103.41195.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2341}{472A8F52.4020909\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2342}{472A8FCD.4090705\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2345}{472C55DE.5040605\%40gmx.de}
\@namedef{freecol-developers.mbox_2343}{01c81dc1$24c0d510$b688965a\%40sjppslatpub}
\@namedef{freecol-developers.mbox_2344}{472C5455.9080806\%40gmx.de}
\@namedef{freecol-developers.mbox_2346}{c2dd2ee70711030458h378e136ekf9e66eb086a95eb0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2347}{op.t07txjm62817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2348}{472C6BCA.7020302\%40gmx.de}
\@namedef{freecol-developers.mbox_2349}{472C7C8D.9050507\%40gmx.de}
\@namedef{freecol-developers.mbox_2350}{472C7F45.5020700\%40gmx.de}
\@namedef{freecol-developers.mbox_2351}{200711031609.29279.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2352}{472CD0B9.1000003\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2353}{200711032116.00813.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2358}{472DBCE6.6010907\%40gmx.de}
\@namedef{freecol-developers.mbox_2359}{472E03B0.6090805\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2362}{472F681F.5040201\%40gmx.de}
\@namedef{freecol-developers.mbox_2363}{000a01c82038$cad84e50$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2366}{47313879.1090106\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2371}{4731F286.7040000\%40gmx.de}
\@namedef{freecol-developers.mbox_2373}{000c01c821c9$44ff1510$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2354}{472CE314.2040801\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2357}{472DA235.3020206\%40gmx.de}
\@namedef{freecol-developers.mbox_2355}{472CEC56.3060102\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2356}{472D665C.9020900\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2360}{472E1763.9000609\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2361}{472E7572.1010304\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2364}{47301362.2010400\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2365}{814ad27f2e6ba13a2d37f3910b8e7ce2\%40ensanjose.net}
\@namedef{freecol-developers.mbox_2367}{000101c820fa$131623b0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2369}{4731E661.3030402\%40gmx.de}
\@namedef{freecol-developers.mbox_2368}{47314A5A.9080301\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2370}{4731EB66.6000109\%40gmx.de}
\@namedef{freecol-developers.mbox_2374}{000d01c821d0$894788e0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2375}{47354D4D.4040702\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2376}{4735985A.7020702\%40gmx.de}
\@namedef{freecol-developers.mbox_2377}{4735FB32.8040004\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2378}{4736C584.8070803\%40gmx.de}
\@namedef{freecol-developers.mbox_2381}{47374B05.4030000\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2372}{47325602.7000602\%40sopd.net}
\@namedef{freecol-developers.mbox_2379}{4737249A.40408\%40gmx.de}
\@namedef{freecol-developers.mbox_2382}{47374D91.9040601\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2380}{473725A3.5060807\%40gmx.de}
\@namedef{freecol-developers.mbox_2383}{473A7B15.4060802\%40www.disney.go.com}
\@namedef{freecol-developers.mbox_2384}{001801c827b8$ca50ae50$3588611b\%40yhw}
\@namedef{freecol-developers.mbox_2385}{473EE7C0.9090107\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2386}{473FE6C4.30008\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2389}{47401DE6.8050505\%40gmx.de}
\@namedef{freecol-developers.mbox_2387}{473FF3C9.7090600\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2388}{47401895.3080207\%40gmx.de}
\@namedef{freecol-developers.mbox_2390}{47409E07.50607\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2392}{4741C149.5060400\%40gmx.de}
\@namedef{freecol-developers.mbox_2391}{01c82a8e$6b375490$5b504fda\%40tein63}
\@namedef{freecol-developers.mbox_2393}{47428448.9070604\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2394}{474300E8.3080606\%40gmx.de}
\@namedef{freecol-developers.mbox_2396}{c2dd2ee70711201413k237eae52s228b6ff54629b450\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2395}{57c05c690711201321g1304f7aew11999027f0b5b622\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2397}{42977.193.157.182.59.1195643487.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2398}{58119.193.157.182.59.1195751441.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2399}{20071122204444.a78f0d98.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2791}{480834D8.2080206\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2813}{50156.80.202.85.174.1209072367.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2400}{37313.193.157.180.109.1195775255.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2402}{20071123160827.836eb452.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2793}{c2dd2ee70804180739k3fb39618i1b7a497ec5afff2c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2401}{47468AEE.1070306\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2403}{4747EBF4.1090201\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2404}{47482E02.4010408\%40gmx.de}
\@namedef{freecol-developers.mbox_2405}{01c82f5f$9672e590$37c2914f\%40mgvjedof}
\@namedef{freecol-developers.mbox_2406}{474A0B24.6060708\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2410}{56542.80.213.198.230.1196112523.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2414}{000601c83192$8b06bd00$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2407}{474B363E.50100\%40gmx.de}
\@namedef{freecol-developers.mbox_2408}{474B37AB.2000903\%40gmx.de}
\@namedef{freecol-developers.mbox_2412}{474C417F.9040603\%40gmx.de}
\@namedef{freecol-developers.mbox_2409}{474B419C.8040602\%40gmx.de}
\@namedef{freecol-developers.mbox_2411}{001c01c83089$f3d2cb30$e5458f51\%40iunrr}
\@namedef{freecol-developers.mbox_2413}{01c83156$021ea390$532f5352\%40tellingson}
\@namedef{freecol-developers.mbox_2415}{474D3271.9090807\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2417}{475171DA.9050509\%40gmx.de}
\@namedef{freecol-developers.mbox_2416}{279103690.19689040906389\%40brandeaux.com}
\@namedef{freecol-developers.mbox_2418}{47531218.108\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2419}{c2dd2ee70712022231x9a57fc0k342aa8bb14c48edb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2422}{475C6B65.5020402\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2420}{01c83760$cd407200$bb86b4bd\%40mmiles}
\@namedef{freecol-developers.mbox_2421}{01c8387d$acba0a00$6db5963e\%40liyveagre}
\@namedef{freecol-developers.mbox_2423}{036301c83c20$bc0d08d0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2424}{01c83c00$c9996900$90cfabbd\%40jerome.gudgeon}
\@namedef{freecol-developers.mbox_2425}{475F6CD1.90905\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2426}{475F7F3A.8080002\%40gmx.de}
\@namedef{freecol-developers.mbox_2427}{476102CC.4040507\%40newaspects.com}
\@namedef{freecol-developers.mbox_2428}{01c83e40$fc31a480$917987de\%40adventure}
\@namedef{freecol-developers.mbox_2429}{cd54e0470712140237o79ea1197j29a061980aa6d69b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2430}{01c83e35$88d66580$76502bbe\%40fosfayhlegaf}
\@namedef{freecol-developers.mbox_2431}{4763D3CE.7060308\%40jupiter.jcom.co.jp}
\@namedef{freecol-developers.mbox_2432}{01c83f11$f8218780$8fb05848\%40tefy}
\@namedef{freecol-developers.mbox_2433}{47650514.7080209\%40gmx.de}
\@namedef{freecol-developers.mbox_2434}{003501c84037$4f7648b0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2443}{476A2B54.2010203\%40gmx.de}
\@namedef{freecol-developers.mbox_2444}{476A3A95.6050309\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2445}{476A42D4.6040404\%40gmx.de}
\@namedef{freecol-developers.mbox_2435}{260524.85574.qm\%40web59006.mail.re1.yahoo.com}
\@namedef{freecol-developers.mbox_2436}{20071217105407.ae03aee0.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2437}{01c840a5$7c584400$52a7a54e\%40mtpq}
\@namedef{freecol-developers.mbox_2438}{47674F14.2010901\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2439}{20071218083039.447fe05b.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2440}{01c841c9$4318f480$c9dff059\%40smmtycv}
\@namedef{freecol-developers.mbox_2441}{15412.10747-4949-490808249-1198107199\%40seznam.cz}
\@namedef{freecol-developers.mbox_2442}{476A28D4.5050702\%40gmx.de}
\@namedef{freecol-developers.mbox_2446}{15068.17772-27719-1382183032-1198155854\%40seznam.cz}
\@namedef{freecol-developers.mbox_2447}{16939.16494-30224-639734363-1198172337\%40seznam.cz}
\@namedef{freecol-developers.mbox_2448}{16857.15943-18738-742699933-1198188919\%40seznam.cz}
\@namedef{freecol-developers.mbox_2452}{476B8E22.7030705\%40gmx.de}
\@namedef{freecol-developers.mbox_2449}{16851.15902-19111-74040410-1198189250\%40seznam.cz}
\@namedef{freecol-developers.mbox_2481}{op.t4l6q5z2rgcyhi\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2482}{478509BD.9040902\%40gmx.de}
\@namedef{freecol-developers.mbox_2450}{476B3B8F.6070100\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2451}{476B8D75.8030100\%40gmx.de}
\@namedef{freecol-developers.mbox_2457}{47700E73.3040504\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2461}{477491B9.4030905\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2462}{4774BC17.2060004\%40gmx.de}
\@namedef{freecol-developers.mbox_2463}{4fb797ba0712280318wd6afe63j58fba4a3024650bf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2464}{4774EAD2.3070408\%40gmx.de}
\@namedef{freecol-developers.mbox_2465}{4776FDD5.3030806\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2466}{47775F8D.7070900\%40gmx.de}
\@namedef{freecol-developers.mbox_2453}{14412.15289-31710-267535741-1198257913\%40seznam.cz}
\@namedef{freecol-developers.mbox_2454}{476E64AF.30303\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2455}{476E6F05.1020006\%40gmx.de}
\@namedef{freecol-developers.mbox_2456}{7b94298e0712230637j76727e26p73296dee49c3f215\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2458}{47715689.203\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2459}{47721523.9050309\%40gmx.de}
\@namedef{freecol-developers.mbox_2460}{01c8490b$1f615700$30156055\%40help}
\@namedef{freecol-developers.mbox_2467}{14624.8771-16109-1948665329-1199056388\%40seznam.cz}
\@namedef{freecol-developers.mbox_2468}{4778C46E.4060207\%40gmx.de}
\@namedef{freecol-developers.mbox_2469}{4778D20D.6060004\%40gmx.de}
\@namedef{freecol-developers.mbox_2470}{c2dd2ee70712310809l1cad3affref15fa13639002ca\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2471}{477915B6.8060407\%40gmx.de}
\@namedef{freecol-developers.mbox_2474}{c2dd2ee70712311938s532219e9l6a6f64a9ceb77867\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2472}{248638172.42288074131903\%40bmssolutions.com}
\@namedef{freecol-developers.mbox_2473}{477955BA.80407\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2475}{4779F159.6080401\%40gmx.de}
\@namedef{freecol-developers.mbox_2476}{0734fd44$14710000$fecd82de\%40akstcallomnsdgs}
\@namedef{freecol-developers.mbox_2477}{477DE307.3000905\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2478}{c2dd2ee70801040912j4515655xbcbbc994de1feb8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2479}{477FBCCF.5010303\%40gmx.de}
\@namedef{freecol-developers.mbox_2497}{47893F97.2040709\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2504}{c2dd2ee70801151710u3ca42e84j8e0dbe338e678463\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2505}{478DA9C5.3040507\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2506}{c2dd2ee70801160531n478d16b3x8bec46dac51da466\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2514}{47902BB5.4090403\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2517}{47903E22.1080300\%40gmx.de}
\@namedef{freecol-developers.mbox_2552}{479ABE53.7080702\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2555}{479AF6BF.6000701\%40gmx.de}
\@namedef{freecol-developers.mbox_2558}{c2dd2ee70801260840i1e5a52d4uec7b02b6aad450c7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2563}{479C4EC1.4000308\%40gmx.de}
\@namedef{freecol-developers.mbox_2596}{47AD5C4F.1030702\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2597}{47AD6931.8010006\%40gmx.de}
\@namedef{freecol-developers.mbox_2598}{47AF73CF.4030901\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2599}{20080211114721.159650\%40gmx.net}
\@namedef{freecol-developers.mbox_2480}{op.t4l6c6lrrgcyhi\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2483}{9838.21812-8938-643652956-1200087984\%40seznam.cz}
\@namedef{freecol-developers.mbox_2485}{002201c854f4$df288ff0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2487}{47887CAF.3060901\%40gmx.de}
\@namedef{freecol-developers.mbox_2498}{c2dd2ee70801130138s23621e0bv1bd31e7d3fa23688\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2484}{9830.21814-12012-1869481297-1200093630\%40seznam.cz}
\@namedef{freecol-developers.mbox_2488}{47887D08.4000201\%40gmx.de}
\@namedef{freecol-developers.mbox_2486}{47887C43.6050608\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2489}{20080112105302.5174bd91.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2492}{4788909E.1010400\%40gmx.de}
\@namedef{freecol-developers.mbox_2490}{20080112110108.bd724107.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2491}{47888FBF.90409\%40gmx.de}
\@namedef{freecol-developers.mbox_2493}{4788AFDB.6050908\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2494}{4788B250.5070905\%40gmx.de}
\@namedef{freecol-developers.mbox_2496}{20080112142816.c3aaeea1.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2495}{20080112143630.db435cc2.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2499}{9238.21955-10002-518821217-1200245321\%40seznam.cz}
\@namedef{freecol-developers.mbox_2500}{478A77B2.7010708\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2501}{478AF4EA.90901\%40gmx.de}
\@namedef{freecol-developers.mbox_2502}{478B0418.7030202\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2503}{478C469C.5030101\%40gmx.de}
\@namedef{freecol-developers.mbox_2507}{478EF444.7080102\%40gmx.de}
\@namedef{freecol-developers.mbox_2513}{4790273A.9060208\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2518}{47903EDD.6010202\%40gmx.de}
\@namedef{freecol-developers.mbox_2508}{478F05C9.80101\%40gmx.de}
\@namedef{freecol-developers.mbox_2511}{c2dd2ee70801170847j1edf9f45h5f8b667578b9e334\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2515}{47903ADF.8020402\%40gmx.de}
\@namedef{freecol-developers.mbox_2512}{47902517.4060109\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2516}{47903D4A.6070905\%40gmx.de}
\@namedef{freecol-developers.mbox_2519}{47904953.6090308\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2520}{47905299.1030108\%40gmx.de}
\@namedef{freecol-developers.mbox_2522}{7b94298e0801180701h2ed2f821r3d8f44aa435d9684\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2509}{39504.45946.qm\%40web43141.mail.sp1.yahoo.com}
\@namedef{freecol-developers.mbox_2523}{54737.80.202.85.49.1200731469.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2510}{001401c858f2$8ff95070$8acc23b6\%40xwfe}
\@namedef{freecol-developers.mbox_2521}{4790B288.3030605\%40canadapost.postescanada.ca}
\@namedef{freecol-developers.mbox_2524}{56696.80.202.85.49.1200747077.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2525}{58460.80.202.85.49.1200753313.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2526}{47925826.4090407\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2527}{c2dd2ee70801191643h1380715cga0ced82310d3ae81\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2528}{47930526.40506\%40gmx.de}
\@namedef{freecol-developers.mbox_2551}{479AB9CD.8040504\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2529}{47932A42.1060206\%40gmx.de}
\@namedef{freecol-developers.mbox_2553}{479AC758.1050608\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2554}{479AF2FA.40001\%40gmx.de}
\@namedef{freecol-developers.mbox_2557}{7b94298e0801260554k4caeb1dha69cfa0671ddc5bd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2564}{49535.80.202.85.49.1201426160.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2565}{479C5FB1.4010002\%40gmx.de}
\@namedef{freecol-developers.mbox_2556}{61518.80.202.85.49.1201338184.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2561}{479BEE94.7060000\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2530}{7b94298e0801221147g428dd105ieb3eb25f09667ae\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2533}{7b94298e0801221751s5d1f66cdt4a187412559afa81\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2534}{7b94298e0801221832h265fd4ddue93e3c5d05ddf7fd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2531}{7755.23480-25689-906124900-1201039838\%40seznam.cz}
\@namedef{freecol-developers.mbox_2532}{47967BE8.5020206\%40actioninc.com}
\@namedef{freecol-developers.mbox_2535}{7b94298e0801221846h1958c4c3n346f9f9a49559f1b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2536}{20080123065819.180850\%40gmx.net}
\@namedef{freecol-developers.mbox_2537}{47978124.7090107\%40gmx.de}
\@namedef{freecol-developers.mbox_2538}{20080123211702.87dedfed.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2543}{4798AF08.8020900\%40gmx.de}
\@namedef{freecol-developers.mbox_2539}{47982DC7.8070300\%40momlaw.com}
\@namedef{freecol-developers.mbox_2540}{49356.80.202.85.49.1201159124.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2541}{c2dd2ee70801240511y1b0e4b9dve90539c8a04d3bc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2542}{4798AB14.4040409\%40gmx.de}
\@namedef{freecol-developers.mbox_2544}{7b94298e0801240732n2c67c237s55f356928184a7c0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2545}{4798B014.3060907\%40gmx.de}
\@namedef{freecol-developers.mbox_2547}{20080124184643.f29f7b96.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2549}{c2dd2ee70801241440m471b2ceeo1a46658026f3aaba\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2546}{4798C0ED.2040503\%40gmx.de}
\@namedef{freecol-developers.mbox_2548}{4798C8FA.6090304\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2550}{479A1085.9020809\%40gmx.de}
\@namedef{freecol-developers.mbox_2571}{47A016C1.7020702\%40gmx.de}
\@namedef{freecol-developers.mbox_2572}{47A16B75.7090207\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2559}{479BCEA7.1030701\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2560}{20080127030711.9e6c7742.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2562}{479C4D83.4060009\%40gmx.de}
\@namedef{freecol-developers.mbox_2567}{c2dd2ee70801270456m22e4178x762d03e44d588c3c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2568}{479C8FCA.2060909\%40gmx.de}
\@namedef{freecol-developers.mbox_2569}{d7db8e850801290440rfb67e4ctb2d60dc281f4a56\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2570}{20080129140645.70340\%40gmx.net}
\@namedef{freecol-developers.mbox_2566}{53051.80.202.85.49.1201437849.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2573}{01c8642a$c4611580$e8521651\%40tesquez}
\@namedef{freecol-developers.mbox_2574}{47A2DD99.4050705\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2577}{47A430E6.4040602\%40gmx.de}
\@namedef{freecol-developers.mbox_2585}{000001c8675a$218808e0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2575}{!~!UENERkVCMDkAAQACAAAAAAAAAAAAAAAAABgAAAAAAAAAYWiWpYplm0mJXUyowli63cKAAAAQAAAAWG69OQVdOEaB3+zjuaNK9gEAAAAA\%40dq.fct.unl.pt}
\@namedef{freecol-developers.mbox_2576}{7b94298e0802011218t4f117b90rf319a2e88e08750a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2578}{ccd806ea0802040023s159d1c51i95d389f02f71f082\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2579}{20080204083329.178990\%40gmx.net}
\@namedef{freecol-developers.mbox_2580}{ccd806ea0802040042y57c18a6ja1da70371f6a257e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2581}{20080204132604.152750\%40gmx.net}
\@namedef{freecol-developers.mbox_2582}{8c0d194e0802040533o114bfa9x9ba29a5bc347325e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2583}{ccd806ea0802040913s4b186418rd3295e8e06046bba\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2587}{20080205064149.174030\%40gmx.net}
\@namedef{freecol-developers.mbox_2588}{ccd806ea0802050141k78fec1baj7bf65364a3199d5c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2589}{ccd806ea0802050147y75ee091pd6ff479cca435ce1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2591}{47A8855D.20807\%40gmx.de}
\@namedef{freecol-developers.mbox_2594}{47A9E107.3080106\%40gmx.de}
\@namedef{freecol-developers.mbox_2600}{ccd806ea0802110441m7f15a0c6gf4d02f7a25326d6a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2601}{47B07653.5060608\%40gmx.de}
\@namedef{freecol-developers.mbox_2584}{ccd806ea0802040916o7912b96ex924f92ed07c57647\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2586}{01c86740$662f4180$a2d61d45\%40swr}
\@namedef{freecol-developers.mbox_2590}{01c867f9$7ac18680$8f00554d\%40ters}
\@namedef{freecol-developers.mbox_2592}{47A88FE9.8090102\%40gmx.de}
\@namedef{freecol-developers.mbox_2593}{47A89567.6010405\%40gmx.de}
\@namedef{freecol-developers.mbox_2595}{01c86a5c$b2d68d80$6536f257\%40mdon}
\@namedef{freecol-developers.mbox_2602}{47B36891.40701\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2603}{47B463E7.2040103\%40gmx.de}
\@namedef{freecol-developers.mbox_2604}{47B6A102.6060505\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2605}{47B6A394.501\%40gmx.de}
\@namedef{freecol-developers.mbox_2606}{47B8C20B.5080008\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2607}{47B92D41.1070301\%40gmx.de}
\@namedef{freecol-developers.mbox_2608}{02d701c87259$ce5f0a50$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2615}{47BD0C7C.1020100\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2616}{47BE680A.7090400\%40gmx.de}
\@namedef{freecol-developers.mbox_2618}{47BFF037.1000806\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2609}{47BA7AE9.7070006\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2610}{47BB21A0.9040903\%40scarlet.be}
\@namedef{freecol-developers.mbox_2611}{47BBD45D.1040207\%40gmx.de}
\@namedef{freecol-developers.mbox_2612}{op.t6tzamdx2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2614}{47BD0829.7040206\%40gmx.de}
\@namedef{freecol-developers.mbox_2613}{op.t6tzzadz2817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2706}{47E2073B.3040403\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2710}{op.t8df2rz62817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_2617}{47BFEF98.900\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2632}{47C17EE4.1010304\%40gmx.de}
\@namedef{freecol-developers.mbox_2619}{47C04B35.6080606\%40gmx.de}
\@namedef{freecol-developers.mbox_2620}{ccd806ea0802230936i7b420d7eq311a4f68e39a9553\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2630}{47C15C03.4030600\%40gmx.de}
\@namedef{freecol-developers.mbox_2635}{8c0d194e0802242322r3f40d0d1xeeb1f4b1a27bea57\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2641}{7b94298e0802250349w5ec4dd23wcab08596177cc683\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2642}{8c0d194e0802250438x75174260jb152df899ff936cc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2636}{ccd806ea0802242339g77c7efd9mf74b3648565da4cd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2621}{ccd806ea0802231346v5efdfbdweeb52a2ce89b1b88\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2622}{47C09D39.4000503\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2625}{47C144A5.6080601\%40gmx.de}
\@namedef{freecol-developers.mbox_2623}{ccd806ea0802231456r35f14cb6mec94288a76e24a35\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2624}{ccd806ea0802232321g6c28ea8cna0794589882ea0b8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2626}{47C145F1.70206\%40gmx.de}
\@namedef{freecol-developers.mbox_2628}{ccd806ea0802240351t4e784a9ep5c7344ac90b74776\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2631}{47C15D27.8090202\%40gmx.de}
\@namedef{freecol-developers.mbox_2644}{c2dd2ee70802252053q5979d437o64b1c1da2971a772\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2646}{47C3B4E3.9040708\%40gmx.de}
\@namedef{freecol-developers.mbox_2647}{49387.80.203.101.218.1204010587.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2664}{ccd806ea0802282052u4871649ar5895d134d3fb54f2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2627}{47C159CD.5070709\%40gmx.de}
\@namedef{freecol-developers.mbox_2633}{47C21059.8050309\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2634}{47C253B8.5070704\%40gmx.de}
\@namedef{freecol-developers.mbox_2637}{ccd806ea0802242344j3d17395di18e7ac4f2355b694\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2653}{52116.80.203.101.218.1204059540.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2658}{ccd806ea0802262329h20a0b01dw45025918bb9968c3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2629}{47C15B6C.2030003\%40gmx.de}
\@namedef{freecol-developers.mbox_2639}{47C278AB.9040809\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2645}{c2dd2ee70802252057y197a75c2g435b17af9ef83bfc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2648}{49423.80.203.101.218.1204011552.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2650}{8c0d194e0802260005u7b6a133ck8218f2ce13cf9825\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2667}{47CA9539.4020108\%40gmx.de}
\@namedef{freecol-developers.mbox_2668}{c2dd2ee70803021211p7c724d20nbe3f43cf01d1a450\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2638}{ccd806ea0802242358l583d0160vdf820c358c2e548c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2640}{47C27A10.7090104\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2643}{47C30BD7.2080502\%40gmx.de}
\@namedef{freecol-developers.mbox_2655}{005001c87902$17f29b10$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2649}{49504.80.203.101.218.1204012456.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2651}{ccd806ea0802260023j7a560864p9e9cd811d29bc498\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2652}{52017.80.203.101.218.1204058875.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2662}{ccd806ea0802280548y289682dat79a16297e4fed24e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2654}{52125.80.203.101.218.1204059981.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2656}{47C5096F.8070001\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2657}{47C50C17.9040805\%40gmx.de}
\@namedef{freecol-developers.mbox_2659}{ccd806ea0802262336o78efc5d4pfb1aa049703ef49d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2660}{47C63EE0.9070904\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2661}{47C64585.7050208\%40gmx.de}
\@namedef{freecol-developers.mbox_2663}{ccd806ea0802282046q5a163900kf6d02d6202233a3c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2665}{ccd806ea0803010938h2dee1146rf5bf7aa3c8d90add\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2666}{47CA8B0D.6010407\%40gmx.de}
\@namedef{freecol-developers.mbox_2669}{c2dd2ee70803021757x365ee83dy4b69df4265425e29\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2670}{47CC196D.8040008\%40gmx.de}
\@namedef{freecol-developers.mbox_2671}{47CD15BB.9020109\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2676}{56362.80.203.88.165.1204833806.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2684}{001e01c8817e$398af6d0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2699}{47DDFD28.7070102\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2700}{c2dd2ee70803170617k121224c0l44f01c4cbd1a8639\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2672}{005201c87eef$f752a050$e5f7e0f0$\%40de}
\@namedef{freecol-developers.mbox_2673}{fd6345820803051256r24e1ae0cwd18909c779291bce\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2675}{47D00FB5.7040407\%40gmx.de}
\@namedef{freecol-developers.mbox_2674}{01c87fa0$82ba4700$925c167b\%40hblnu}
\@namedef{freecol-developers.mbox_2677}{47D0FA7F.8090802\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2683}{64932.80.203.88.165.1205001010.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2678}{ccd806ea0803070129nac8afd1la8a27f13c12b14ed\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2681}{006401c880b8$e3c33ca0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2682}{47D24A9F.9040606\%40gmx.de}
\@namedef{freecol-developers.mbox_2690}{ccd806ea0803120914q3eba075eh7e922e7d55c8b7ee\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2679}{094181683.09441686667336\%40alsecco.cz}
\@namedef{freecol-developers.mbox_2680}{006301c880b8$8549e750$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2685}{47D3F623.70900\%40gmx.de}
\@namedef{freecol-developers.mbox_2686}{47D496A9.9040409\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2687}{c2dd2ee70803100524i2ab2f9b5n2af7265adf853b3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2692}{47D8B2F7.5020609\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2693}{47D8B72E.4060306\%40gmx.de}
\@namedef{freecol-developers.mbox_2696}{47DA2672.1070708\%40gmx.de}
\@namedef{freecol-developers.mbox_2688}{47D77056.1030607\%40gmx.de}
\@namedef{freecol-developers.mbox_2691}{47D80311.3000101\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2689}{ccd806ea0803120912k3cf89brba81e1b0402bdf53\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2694}{c2dd2ee70803131358q348ad160q31aab9a87d6f7376\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2695}{47DA12B6.4040402\%40gmx.de}
\@namedef{freecol-developers.mbox_2697}{47DD4FDE.8010304\%40gmx.de}
\@namedef{freecol-developers.mbox_2698}{47DDA147.80401\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2701}{47DE9AE0.4010401\%40gmx.de}
\@namedef{freecol-developers.mbox_2703}{47E08F8E.8050903\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2704}{47E13B0F.5090801\%40gmx.de}
\@namedef{freecol-developers.mbox_2702}{47DFF3FE.1020704\%40gmx.de}
\@namedef{freecol-developers.mbox_2705}{47E201B5.5020506\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2707}{47E39B06.3020009\%40gmx.de}
\@namedef{freecol-developers.mbox_2711}{47E54CC5.9060906\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2712}{47E61F66.4060105\%40gmx.de}
\@namedef{freecol-developers.mbox_2713}{BLU132-DAV12FE8C2AA0AE8EC5B74A9F93030\%40phx.gbl}
\@namedef{freecol-developers.mbox_2714}{47E63F59.2070907\%40gmx.de}
\@namedef{freecol-developers.mbox_2718}{47E6A1B6.8090401\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2719}{BLU132-DAV8530DD86FB1F7BF6C111193030\%40phx.gbl}
\@namedef{freecol-developers.mbox_2728}{47EB3E0B.9030408\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2731}{50637.80.203.88.165.1206868061.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2732}{47EF5FD3.4060308\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2708}{4d6107450803210537g7194bff2r8e795c1ad47aa6ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2709}{47E3BFE0.9090702\%40gmx.de}
\@namedef{freecol-developers.mbox_2715}{47E684DC.6090308\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2716}{47E68F97.4050402\%40gmx.de}
\@namedef{freecol-developers.mbox_2717}{47E69BE4.1050306\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2720}{47E913E2.9000001\%40gmx.de}
\@namedef{freecol-developers.mbox_2721}{c2dd2ee70803250908x4d5daa3ehead1388a7eebc711\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2722}{47E92632.2020503\%40gmx.de}
\@namedef{freecol-developers.mbox_2723}{397d46d00803260827i852c173o3288ee1cba8a429d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2724}{47EA6E77.3040807\%40gmx.de}
\@namedef{freecol-developers.mbox_2725}{397d46d00803260903m31e28cebpe1e2aa1780e688eb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2726}{47EA8273.3080308\%40gmx.de}
\@namedef{freecol-developers.mbox_2727}{7b94298e0803261355ub49588i9c54f6d89b4c174d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2755}{397d46d00804030856n7b7579efhed351a6bb3a3ff67\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2756}{47F505D6.1070107\%40gmx.de}
\@namedef{freecol-developers.mbox_2759}{47F93939.70304\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2760}{397d46d00804070936o7debc503x5d25b0a53ee957ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2761}{7b94298e0804080449g2398dea0ie694fb858cf45e68\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2729}{BAY119-W193A54B4E7EDC7BB0F171BF6FB0\%40phx.gbl}
\@namedef{freecol-developers.mbox_2730}{50537.80.203.88.165.1206867093.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2733}{47EF69EE.8080101\%40gmx.de}
\@namedef{freecol-developers.mbox_2734}{47EF8D58.9040007\%40gmx.de}
\@namedef{freecol-developers.mbox_2735}{ccd806ea0803300723s7e61d042h132b8d7870315508\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2736}{47EFAFE3.4060900\%40gmx.de}
\@namedef{freecol-developers.mbox_2737}{56403.80.203.88.165.1206909905.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2739}{47F0F628.9040506\%40gmx.de}
\@namedef{freecol-developers.mbox_2753}{62651.80.203.88.165.1207170338.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2738}{c2dd2ee70803301530x78c37e7fvcacd570d77918f61\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2740}{47F10662.8060103\%40gmx.de}
\@namedef{freecol-developers.mbox_2741}{32822fe60803311731j23dbf7bawb1369d55c19e3197\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2744}{47F251D9.70705\%40gmx.de}
\@namedef{freecol-developers.mbox_2745}{c2dd2ee70804010915q906fed8kf9ac05d881212d90\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2746}{47F260C7.8000602\%40gmx.de}
\@namedef{freecol-developers.mbox_2742}{61d2e9b20804010759q358e1c88g1261ad2947ee41d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2743}{47F24FB4.3090301\%40gmx.de}
\@namedef{freecol-developers.mbox_2747}{47F25417.9050203\%40gmx.de}
\@namedef{freecol-developers.mbox_2748}{c2dd2ee70804011750p54cc00b9p99cf74d2b5b12ef8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2749}{47F39527.3030802\%40gmx.de}
\@namedef{freecol-developers.mbox_2750}{c2dd2ee70804020909n39ae66e4u11478898d47dc6db\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2751}{47F3B3EE.7080406\%40gmx.de}
\@namedef{freecol-developers.mbox_2752}{c2dd2ee70804021210r3eb658e1gf4332f12d1a84be4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2754}{2104233_\%40TLZ7879628_\%40TLZ}
\@namedef{freecol-developers.mbox_2757}{397d46d00804031415h26e960aes9fdb98c3613462a5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2758}{397d46d00804041400h6ff14a2dt246da03b90828f60\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2762}{397d46d00804081341q1a9c7129r38d43e477093a1f9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2763}{47FCFB22.7000009\%40gmx.de}
\@namedef{freecol-developers.mbox_2775}{48006E3D.2050000\%40gmx.de}
\@namedef{freecol-developers.mbox_2783}{397d46d00804150959ie5711c3w46730007707567b1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2764}{47FCFC0D.6000005\%40gmx.de}
\@namedef{freecol-developers.mbox_2765}{c2dd2ee70804091522m37be0719w19d2c9ccceaf1a93\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2766}{016401c89ac0$c53ff300$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2769}{47FE32D8.3010309\%40gmx.de}
\@namedef{freecol-developers.mbox_2770}{47FE4729.60007\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2771}{20080411064420.230800\%40gmx.net}
\@namedef{freecol-developers.mbox_2773}{32822fe60804112205r1a489a7dkc1f87f163d760663\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2774}{4800693E.4000509\%40gmx.de}
\@namedef{freecol-developers.mbox_2776}{48006F63.4070509\%40gmx.de}
\@namedef{freecol-developers.mbox_2778}{480111E2.2030205\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2779}{4801D90C.9000309\%40gmx.de}
\@namedef{freecol-developers.mbox_2792}{48083555.5000609\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2767}{c2dd2ee70804100357h1415eac4yfee4d7dd614dcfcb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2768}{47FE3270.5040502\%40gmx.de}
\@namedef{freecol-developers.mbox_2772}{61d2e9b20804111307j7d836142jab7953d795054863\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2777}{48008215.2010808\%40gmx.de}
\@namedef{freecol-developers.mbox_2810}{4810274C.3080405\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2812}{63887.80.202.85.174.1209062033.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2814}{4812F607.2010202\%40gmx.de}
\@namedef{freecol-developers.mbox_2816}{4816CCF1.7000404\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2780}{4801FEA5.7040606\%40gmx.de}
\@namedef{freecol-developers.mbox_2784}{4805890A.1010005\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2785}{397d46d00804160416g6dba711cs116d55fbce7e42a8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2786}{48061538.5090205\%40gmx.de}
\@namedef{freecol-developers.mbox_2787}{4806161E.7090503\%40gmx.de}
\@namedef{freecol-developers.mbox_2788}{4806F7C4.7040306\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2789}{48075C12.1000807\%40gmx.de}
\@namedef{freecol-developers.mbox_2781}{E503D14C.8\%Dariusz-ietshcad\%40BizBoxCo.com}
\@namedef{freecol-developers.mbox_2782}{61d2e9b20804141143g6b3427a0h9297791dddd98878\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2790}{7b94298e0804171343s666c4b5ci37f575befcf041cf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2794}{C9F50B6E.4\%dnuur1991\%4095dc.com}
\@namedef{freecol-developers.mbox_2795}{4808B92D.9090903\%40gmx.de}
\@namedef{freecol-developers.mbox_2796}{397d46d00804180946l601c2176p7776c10eea370074\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2797}{397d46d00804180947r70248a4fg934c28ea93216769\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2798}{4809B6EB.3040901\%40gmx.de}
\@namedef{freecol-developers.mbox_2800}{480B44AB.7080105\%40gmx.de}
\@namedef{freecol-developers.mbox_2801}{20080420105711.3b59a57f.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2802}{480C2344.3090003\%40gmx.de}
\@namedef{freecol-developers.mbox_2808}{397d46d00804231119k1566c7fej8dcd93f61a3c3771\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2809}{397d46d00804231140s72aecef1g13934d4fa6282b98\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2799}{9B7229EF.5\%maskinsj_1998\%40MARSHALLFURNITURE.COM}
\@namedef{freecol-developers.mbox_2803}{480BFF28.8020506\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2805}{c2dd2ee70804220726w1f17ffcbo25ccb3d77dd6826\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2806}{480EC4BF.3090306\%40gmx.de}
\@namedef{freecol-developers.mbox_2811}{481027B1.1060806\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2804}{5CA61894.8\%bestmind\%40NaturalMarketing.com}
\@namedef{freecol-developers.mbox_2807}{6440C21E.3\%edazbara_1967\%40CAT.CA}
\@namedef{freecol-developers.mbox_2815}{48132072.1050609\%40gmx.de}
\@namedef{freecol-developers.mbox_2823}{481D6B00.8060003\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2825}{481D8AD8.5010106\%40gmx.de}
\@namedef{freecol-developers.mbox_2817}{4819F70F.6090404\%40gmx.de}
\@namedef{freecol-developers.mbox_2818}{c2dd2ee70805011614h646d4660y95035102c351768c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2820}{481C0E1D.7030105\%40gmx.de}
\@namedef{freecol-developers.mbox_2821}{55688.80.202.85.174.1209838395.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2824}{481D8A03.5020203\%40gmx.de}
\@namedef{freecol-developers.mbox_2819}{19F1798C.5\%tineille1981\%40Oanow.Com}
\@namedef{freecol-developers.mbox_2822}{481D6743.6080906\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2826}{481D8C35.7040006\%40gmx.de}
\@namedef{freecol-developers.mbox_2827}{481DF988.4090304\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_2828}{c2dd2ee70805041535t278320d2q8bd82dc21e43deb6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2832}{397d46d00805060626k50c0cca2x1c1faa18fc2465df\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2829}{0470DF08.3\%hcneb-ss\%40194.82.111.219.dy.bbexcite.jp}
\@namedef{freecol-developers.mbox_2830}{15753F04.F\%metagged1953\%40KUIJPERS.COM}
\@namedef{freecol-developers.mbox_2831}{48200394.6070702\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2833}{4820680B.9050303\%40gmx.de}
\@namedef{freecol-developers.mbox_2834}{48228E7C.508\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2835}{20080508104233.269870\%40gmx.net}
\@namedef{freecol-developers.mbox_2846}{4826A71F.50004\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2847}{4826C723.80807\%40gmx.de}
\@namedef{freecol-developers.mbox_2836}{AB5662806B7C4393A4A2034036DBF0B5\%40kasutaja3bf56e}
\@namedef{freecol-developers.mbox_2837}{397d46d00805081452r4ed149bar72fcf9cb70432c86\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2839}{48246BAE.8020509\%40gmx.de}
\@namedef{freecol-developers.mbox_2838}{000a01c8b191$d0963ba0$1e57c7d0\%40miti.local}
\@namedef{freecol-developers.mbox_2840}{482558A9.3070707\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2841}{48255BBF.6050302\%40gmx.de}
\@namedef{freecol-developers.mbox_2842}{4825618D.6040608\%40gmx.de}
\@namedef{freecol-developers.mbox_2843}{48256CB9.3010703\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2844}{482579E8.2070602\%40gmx.de}
\@namedef{freecol-developers.mbox_2845}{4825A118.8070504\%40gmx.de}
\@namedef{freecol-developers.mbox_2848}{7b94298e0805111028od4075e7x691ddba58ab78f1a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2849}{4828265A.6020807\%40gmx.de}
\@namedef{freecol-developers.mbox_2850}{4829ACA4.7010600\%40gmx.de}
\@namedef{freecol-developers.mbox_2851}{482E938C.5000502\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2852}{4833C709.4010404\%40gmx.de}
\@namedef{freecol-developers.mbox_2853}{48349BFA.9090808\%40free.fr}
\@namedef{freecol-developers.mbox_2854}{48357F27.3060208\%40gmx.de}
\@namedef{freecol-developers.mbox_2855}{483AE75A.8070503\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2856}{483BADA2.9000702\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2857}{483BBF8F.5030201\%40gmx.de}
\@namedef{freecol-developers.mbox_2885}{57695.80.202.85.174.1212827179.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2858}{7b94298e0805280650x7a61c404r500d6c2ca5b880c4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2859}{483E5A8B.70301\%40gmx.de}
\@namedef{freecol-developers.mbox_2860}{501f5b5d0805290151k2d30b2e7pcec8118044c317bb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2861}{501f5b5d0805290151k2d30b2e7pcec8118044c317bb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2862}{7b94298e0805290152k4ca62367u6b6f4aa036ac2c8f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2878}{55627.80.202.85.174.1212789671.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2887}{484A7925.70104\%40gmx.de}
\@namedef{freecol-developers.mbox_2864}{483F0D05.1090103\%40free.fr}
\@namedef{freecol-developers.mbox_2863}{483FAFA4.6040300\%40gmx.de}
\@namedef{freecol-developers.mbox_2882}{484A1801.9030404\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2888}{484A7E64.5080001\%40free.fr}
\@namedef{freecol-developers.mbox_2865}{000001c8c32a$e792a7d0$2f02a8c0\%40willy}
\@namedef{freecol-developers.mbox_2866}{484172DF.7030609\%40gmx.de}
\@namedef{freecol-developers.mbox_2867}{48446C46.2060501\%40free.fr}
\@namedef{freecol-developers.mbox_2870}{484620CE.4050004\%40gmx.de}
\@namedef{freecol-developers.mbox_2873}{7b94298e0806050857s50b2b718s5f88bc2c786b1d34\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2874}{7b94298e0806050909h3a130e87vc624a8e3a58ced76\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2876}{7b94298e0806060624wd95ca6dv4175ea6337e4e1a7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2879}{4849CE87.8040103\%40free.fr}
\@namedef{freecol-developers.mbox_2868}{4844C7E9.5020704\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2869}{20080603095554.115520\%40gmx.net}
\@namedef{freecol-developers.mbox_2871}{4846230D.6060305\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2872}{484775A0.2030709\%40gmx.de}
\@namedef{freecol-developers.mbox_2880}{484A0CAB.6030306\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2886}{484A78CC.5060405\%40gmx.de}
\@namedef{freecol-developers.mbox_2875}{20080606123415.18740\%40gmx.net}
\@namedef{freecol-developers.mbox_2877}{7b94298e0806060631wd4f6b8y6f1d14c308392907\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2881}{484A1002.5050703\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2884}{57592.80.202.85.174.1212826462.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2883}{57507.80.202.85.174.1212824744.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2890}{7b94298e0806091030k3a834d13h56929eaf49d6c5ed\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2898}{27264.84.49.2.1.1213193531.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2889}{b84591f00806081655v69203bb1l8a0baae849ebd640\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2894}{484E9647.4060008\%40gmx.de}
\@namedef{freecol-developers.mbox_2891}{484D8ED2.8080602\%40free.fr}
\@namedef{freecol-developers.mbox_2892}{484E2832.9080206\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2893}{484E95AB.1080609\%40gmx.de}
\@namedef{freecol-developers.mbox_2895}{484EAEF0.8000004\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2896}{397d46d00806101013g24d9482bg4d5cc4e3f75adcbb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2897}{b84591f00806110222q449d5e9gd656d8cae9e4ff8a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2899}{48500497.1000809\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2900}{50836.80.202.85.174.1213214118.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2916}{7b94298e0807011529o1a34b3c0pe0b1eca8b7da8772\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2934}{7b94298e0807161218p611611b4o6c56bbc89a8d3889\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2901}{4853E782.2000908\%40gmx.de}
\@namedef{freecol-developers.mbox_2902}{4854DC69.2080307\%40gmx.de}
\@namedef{freecol-developers.mbox_2903}{4854DC5D.5080903\%40free.fr}
\@namedef{freecol-developers.mbox_2904}{4854E07B.7030203\%40gmx.de}
\@namedef{freecol-developers.mbox_2905}{4854E2AE.70101\%40gmx.de}
\@namedef{freecol-developers.mbox_2907}{54803.80.202.85.174.1213647998.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2908}{48573E73.2030906\%40gmx.de}
\@namedef{freecol-developers.mbox_2906}{54678.80.202.85.174.1213643911.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2909}{52367.80.202.85.174.1213997989.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2911}{485CB426.6040300\%40gmx.de}
\@namedef{freecol-developers.mbox_2919}{48758039.3080906\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2920}{20080710084238.67590\%40gmx.net}
\@namedef{freecol-developers.mbox_2923}{59771.80.203.101.186.1215723333.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2912}{397d46d00806231514g4ff1f479m749b90d9a049b868\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2913}{b84591f00806240059q5649439djf2677eb410280d75\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2910}{485CB2AC.4010807\%40gmx.de}
\@namedef{freecol-developers.mbox_2914}{48663DF8.90103\%40gmx.de}
\@namedef{freecol-developers.mbox_2915}{7b94298e0806280703ta042a0ehfd2f5a04ac0b5d51\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2917}{4870BFA6.7080708\%40gmx.de}
\@namedef{freecol-developers.mbox_2918}{48723FE7.80609\%40gmx.de}
\@namedef{freecol-developers.mbox_2921}{48763C79.2020004\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2922}{48763F48.5070803\%40gmx.de}
\@namedef{freecol-developers.mbox_2924}{50136.84.49.2.1.1215786649.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2925}{7b94298e0807111036u245cd367x5b1e825fdef5fa62\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2927}{20080711235402.5bfbd1f5.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2926}{397d46d00807111121k92f00dbwd8939a4f9a143e67\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2928}{397d46d00807111416obf300c6pd28b6e3a6f7c0926\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2930}{487878EE.8020507\%40gmx.de}
\@namedef{freecol-developers.mbox_2932}{397d46d00807140636t6847023x9a798e007f2aab48\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2933}{487D77C9.6050501\%40gmx.de}
\@namedef{freecol-developers.mbox_2929}{49268.80.203.101.186.1215819579.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2931}{487A1A5A.3030307\%40gmx.de}
\@namedef{freecol-developers.mbox_2935}{7b94298e0807171430m18099a0erfe6b59b266c31a32\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3035}{7b94298e0809170500o23fa5debqd099bfea1323c285\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3140}{7b94298e0810080449m2c059400ua2f0c8d1c4f4894a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2936}{48824BAE.6080101\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2937}{48830A6E.8020002\%40gmx.de}
\@namedef{freecol-developers.mbox_2938}{48832C92.7020500\%40gmx.de}
\@namedef{freecol-developers.mbox_2947}{FA8ACC664B974E649DA6626EBB533D72\%40miti.local}
\@namedef{freecol-developers.mbox_2948}{4889E5E3.2020301\%40gmx.de}
\@namedef{freecol-developers.mbox_2939}{20080721180647.a05fa7ba.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_2940}{4885F06D.6090506\%40gmx.de}
\@namedef{freecol-developers.mbox_2941}{48860685.1020300\%40gmx.de}
\@namedef{freecol-developers.mbox_2942}{1216589056.5976.13.camel\%40r025072}
\@namedef{freecol-developers.mbox_2943}{48875B3F.8080507\%40gmx.de}
\@namedef{freecol-developers.mbox_2944}{56a2c980807231955j3e599413q12d495638012ef68\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2945}{111A284831CF4150B1087180EA75B313\%40miti.local}
\@namedef{freecol-developers.mbox_2946}{397d46d00807241038x2f1d7345h4fa687cf31cb3101\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2949}{4889F5BA.4080702\%40gmx.de}
\@namedef{freecol-developers.mbox_2950}{397d46d00807250924g4e5e8b4as8898f10797b87204\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2951}{488A03F4.8040206\%40gmx.de}
\@namedef{freecol-developers.mbox_2954}{541902A5-222A-4F06-870B-36D3DBFD1AF8\%40tarnkappenbaum.org}
\@namedef{freecol-developers.mbox_2955}{24316.84.49.2.1.1217606174.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_2956}{7b94298e0808011242u592ad88dpcc09bc18b60040f4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2957}{7b94298e0808011246i7406e2a3t60a73c8285e3a63c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2958}{7b94298e0808011305v74cc2d77mbe7a43d79f71a6e5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2952}{3a7129160807291008xe0e1842lb7742f71b7400290\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2953}{7b94298e0807291316q65c2b392x60a42ae1d04662b3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2959}{4893FFEB.6060008\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2960}{489C6584.1070200\%40gmx.de}
\@namedef{freecol-developers.mbox_2961}{b84591f00808081442y4512448cmfd46db0c05a3aa17\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2962}{489D4B76.1000803\%40gmx.de}
\@namedef{freecol-developers.mbox_2963}{48A68B92.8050400\%40gmx.de}
\@namedef{freecol-developers.mbox_2964}{48A80EAA.5090401\%40gmx.de}
\@namedef{freecol-developers.mbox_2965}{7b94298e0808170504o58ec0226i52c9f1ce11552a59\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2966}{48A82DAD.7050806\%40gmx.de}
\@namedef{freecol-developers.mbox_2967}{6e5148e60808190502m699d7701h9f9e42f38b37c82e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2968}{BAY139-W105654EBA60E0253950EDAE9690\%40phx.gbl}
\@namedef{freecol-developers.mbox_2969}{397d46d00808190633q609101f2o3e48f85509bd0b29\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2970}{48AC26E3.1030908\%40gmx.de}
\@namedef{freecol-developers.mbox_2971}{48ADA2D2.1010401\%40gmx.de}
\@namedef{freecol-developers.mbox_2972}{48B1C79C.6020705\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2973}{48B25628.7020005\%40gmx.de}
\@namedef{freecol-developers.mbox_2974}{200808252148.37818.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2977}{48B3A958.7010402\%40gmx.de}
\@namedef{freecol-developers.mbox_2975}{48B388A6.4060704\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2976}{48B3A692.4040200\%40gmx.de}
\@namedef{freecol-developers.mbox_2985}{200808302255.53628.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2986}{200809012148.49732.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2987}{48BC2F09.7090007\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2988}{200809021929.27986.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2990}{48BD6AED.4060607\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2978}{48B3DB2C.9050703\%40gmx.de}
\@namedef{freecol-developers.mbox_2982}{48B52345.60505\%40gmx.de}
\@namedef{freecol-developers.mbox_2983}{48B523CC.7000700\%40gmx.de}
\@namedef{freecol-developers.mbox_2979}{200808261149.m7QBnVKf005457\%40malbec.vatican.com.au}
\@namedef{freecol-developers.mbox_2984}{200808272048.24260.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2980}{200808261221.m7QCLQ6w005952\%40malbec.vatican.com.au}
\@namedef{freecol-developers.mbox_2981}{48B46561.9090009\%40gmx.de}
\@namedef{freecol-developers.mbox_2989}{200809022143.32154.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2991}{48BD6E94.5060103\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2992}{48BE26D5.8050608\%40metaintegration.net}
\@namedef{freecol-developers.mbox_2993}{64923D1919E548F596F68DA4A82A70C1\%40miti.local}
\@namedef{freecol-developers.mbox_2994}{2ce9650b0809031155x5d86945g5fb99287328886b3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2999}{48162D9FE6E1470C830DB6ADC4C652F1\%40miti.local}
\@namedef{freecol-developers.mbox_3000}{200809042311.01855.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_2995}{20080903202822.GC8723\%40lh.kyla.fi}
\@namedef{freecol-developers.mbox_2998}{501f5b5d0809032308i4dcdeaebg57065d9c66228072\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_2996}{20080903202728.GB8723\%40lh.kyla.fi}
\@namedef{freecol-developers.mbox_2997}{1BEAFA6676D443AAB8ADE9C178219640\%40miti.local}
\@namedef{freecol-developers.mbox_3001}{200809051121.06537.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3003}{1D975D0EA8E54F7893995C40C21E69E8\%40miti.local}
\@namedef{freecol-developers.mbox_3044}{200809182131.40856.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3049}{48D26905.5010707\%40gmx.de}
\@namedef{freecol-developers.mbox_3002}{397d46d00809050636j5b0f6509x15a73aebdc5ace5b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3004}{200809071235.22288.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3005}{48C4D392.4060503\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3007}{200809082311.27621.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3008}{200809082214.17996.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3006}{54408.84.49.2.1.1220861818.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3009}{52266.80.213.136.138.1221082783.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3010}{b164d84d0809101657q29226eb6t27d54fe93d8ddfc6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3011}{64247.80.213.136.138.1221169237.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3012}{b164d84d0809111658j35e117deq8ee390345bc886ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3014}{48CA2530.1000708\%40gmx.de}
\@namedef{freecol-developers.mbox_3013}{b164d84d0809111721s31df924ated2ef94a225576e1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3015}{48CA5346.5020802\%40gmx.de}
\@namedef{freecol-developers.mbox_3019}{b164d84d0809122220x3b48e688m4b2b115f48d2b5ad\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3020}{48CB9627.7060704\%40gmx.de}
\@namedef{freecol-developers.mbox_3016}{b164d84d0809120936h2198f481v94fbd288fd72506e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3022}{48CB9A72.8090708\%40gmx.de}
\@namedef{freecol-developers.mbox_3023}{b164d84d0809131208o117ae538uaab4ef8b2783ac2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3024}{48CC165D.4060501\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3026}{48CCB94C.2080509\%40gmx.de}
\@namedef{freecol-developers.mbox_3017}{200809122038.27766.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3021}{48CB9706.2000704\%40gmx.de}
\@namedef{freecol-developers.mbox_3025}{200809140923.31193.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3029}{b164d84d0809140756n50bab685s947891105b3d6170\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3031}{200809150736.56739.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3032}{b164d84d0809151218m4b85f196rcefc900262e5a28d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3033}{48CFC963.7070606\%40gmx.de}
\@namedef{freecol-developers.mbox_3034}{200809160756.50623.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3018}{b164d84d0809121049t4fa6f675yf97d2913012b7e75\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3027}{20080914121340.628b1719.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3028}{48CCF807.7070206\%40gmx.de}
\@namedef{freecol-developers.mbox_3030}{b164d84d0809140826m433694a6qb688360e1fef7d25\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3036}{48D1086D.6070205\%40gmx.de}
\@namedef{freecol-developers.mbox_3037}{7b94298e0809171131s2f38c7dbsfaf0e71b4571ec41\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3038}{8B821DF6203247CDBC451A39CFEF1C68\%40miti.local}
\@namedef{freecol-developers.mbox_3039}{3978E8D462B14FBDAF67401ECC1F7E0A\%40miti.local}
\@namedef{freecol-developers.mbox_3040}{b164d84d0809171418y7bdcbef4mc59e3cbc89c656ef\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3041}{E699D408A15F4A5A9B66E325E7BE26A3\%40miti.local}
\@namedef{freecol-developers.mbox_3046}{48D26514.5090100\%40gmx.de}
\@namedef{freecol-developers.mbox_3051}{b164d84d0809181000y6ab6d44en25637d88356b1ebf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3053}{CFD771AC32CB4DC99F36163197603CD8\%40miti.local}
\@namedef{freecol-developers.mbox_3054}{48D48BF3.9080009\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3055}{48D4A8A7.4050709\%40gmx.de}
\@namedef{freecol-developers.mbox_3060}{b164d84d0809221202j34d0afbdjf29bd6eee742d190\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3063}{20080923101839.113230\%40gmx.net}
\@namedef{freecol-developers.mbox_3045}{48D2647A.2040708\%40gmx.de}
\@namedef{freecol-developers.mbox_3042}{b164d84d0809171645v4fe96474w5bcf747b226a4e60\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3047}{48D2671D.1000102\%40gmx.de}
\@namedef{freecol-developers.mbox_3052}{b164d84d0809181114m7108edd8j71ac4dfb739be6b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3043}{200809182118.02557.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3048}{48D2689A.6010501\%40gmx.de}
\@namedef{freecol-developers.mbox_3050}{48D26A0D.3070903\%40gmx.de}
\@namedef{freecol-developers.mbox_3064}{200809232330.45174.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3066}{48D9C5E9.7060807\%40gmx.de}
\@namedef{freecol-developers.mbox_3067}{20080924120707.127330\%40gmx.net}
\@namedef{freecol-developers.mbox_3068}{b164d84d0809241517l1d416712s3011b889dd69ece6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3069}{48DB2721.2000709\%40gmx.de}
\@namedef{freecol-developers.mbox_3070}{20080925104455.307850\%40gmx.net}
\@namedef{freecol-developers.mbox_3073}{b164d84d0809250948nf94ab86qee926ce1e5a097bd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3074}{1222364631.6624.15.camel\%40amiloxi}
\@namedef{freecol-developers.mbox_3075}{b164d84d0809251235w1b353019x87fbe05eff98752f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3078}{48DC681A.1080400\%40gmx.de}
\@namedef{freecol-developers.mbox_3079}{20080926112900.45800\%40gmx.net}
\@namedef{freecol-developers.mbox_3081}{b164d84d0809260647y7371bda0h6ae9c321b1b3177d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3085}{48DDE003.4080401\%40gmx.de}
\@namedef{freecol-developers.mbox_3104}{1222452803.7214.11.camel\%40amiloxi}
\@namedef{freecol-developers.mbox_3083}{b164d84d0809261219n4436c47fpef575f13fe2ee4a3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3084}{1222495902.6783.18.camel\%40amiloxi}
\@namedef{freecol-developers.mbox_3086}{48DDE523.4070102\%40gmx.de}
\@namedef{freecol-developers.mbox_3088}{1222507804.9951.23.camel\%40amiloxi}
\@namedef{freecol-developers.mbox_3089}{48DE01B9.5050605\%40gmx.de}
\@namedef{freecol-developers.mbox_3090}{48DE09B1.3080309\%40gmx.de}
\@namedef{freecol-developers.mbox_3115}{48E86B2A.9020605\%40gmx.de}
\@namedef{freecol-developers.mbox_3077}{48DC6638.7040306\%40gmx.de}
\@namedef{freecol-developers.mbox_3082}{b164d84d0809260649q94c78f5r6e9c4028e39c729f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3072}{200809252239.01623.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3076}{48DC65E3.9080101\%40gmx.de}
\@namedef{freecol-developers.mbox_3080}{200809262137.44928.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3087}{48DDEC51.1050106\%40gmx.de}
\@namedef{freecol-developers.mbox_3105}{48DDE225.2060208\%40gmx.de}
\@namedef{freecol-developers.mbox_3106}{48DE1CDB.6090505\%40gmx.de}
\@namedef{freecol-developers.mbox_3124}{200810062211.02796.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3131}{48EAF051.9020907\%40gmx.de}
\@namedef{freecol-developers.mbox_3132}{48EB102D.7010002\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3133}{200810072025.42810.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3136}{48EC3ACA.7040004\%40gmx.de}
\@namedef{freecol-developers.mbox_3139}{48EC582D.6060907\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3145}{200810092120.21005.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3151}{48EEEB67.4000205\%40gmx.de}
\@namedef{freecol-developers.mbox_3169}{200810132159.30262.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3171}{48F362B3.5090701\%40gmx.de}
\@namedef{freecol-developers.mbox_3173}{op.uiy0rsco55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3174}{200810142242.50170.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3177}{op.ui2hiehb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3178}{200810160829.35530.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3179}{adcf5e800810151533v264ee358sdcae3d4189ce5fa0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3181}{200810162056.54946.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3185}{48F76D9D.4080103\%40gmx.de}
\@namedef{freecol-developers.mbox_3183}{48F76C2D.8050108\%40gmx.de}
\@namedef{freecol-developers.mbox_3191}{op.ui41s0o955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3184}{48F76D31.2050901\%40gmx.de}
\@namedef{freecol-developers.mbox_3190}{op.ui40mpxa55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3175}{200810142257.54969.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3056}{48D4AA16.8030703\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3057}{48D4C5D9.40008\%40gmx.de}
\@namedef{freecol-developers.mbox_3058}{48D572D1.9000409\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3059}{48D5FF12.3060006\%40gmx.de}
\@namedef{freecol-developers.mbox_3061}{b164d84d0809221206p13c1f75dq4e3eea1f5c935dc8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3062}{b164d84d0809221208r279f596as759efb28d0ff11d3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3065}{b164d84d0809231321g1839d68bgbdf971056f0ff376\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3071}{20080925104536.307900\%40gmx.net}
\@namedef{freecol-developers.mbox_3091}{adcf5e800809271809n65756e9ex73e4569d1cbdbf31\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3092}{48DF6013.1070904\%40gmx.de}
\@namedef{freecol-developers.mbox_3093}{adcf5e800809280402w1c42456cxb091d238a7335e95\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3094}{49A5BB2DFBA84B79B827BE79BC4944E3\%40miti.local}
\@namedef{freecol-developers.mbox_3098}{48E3995D.40605\%40gmx.de}
\@namedef{freecol-developers.mbox_3108}{op.uiafgitf55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3114}{48E86B9F.7010304\%40gmx.de}
\@namedef{freecol-developers.mbox_3120}{adcf5e800810050817x51db1440w43cc2e42e75c1ad0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3109}{adcf5e800809301048s21b15c5ake771028201ed9bab\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3095}{48E322D7.6040408\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3096}{adcf5e800810010415p51ffa8eai902a16a333be28fd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3099}{48E39A4A.8080901\%40gmx.de}
\@namedef{freecol-developers.mbox_3101}{adcf5e800810010918p483e0ca5rd7d47bd7ace1d91\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3102}{48E3AE28.9010504\%40gmx.de}
\@namedef{freecol-developers.mbox_3111}{48E44DE6.5040207\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3112}{adcf5e800810020528x5fac428t52459d37ecb1ef0f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3113}{48E80BF0.6010305\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3097}{20081001143151.b084a8e8.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3110}{adcf5e800810010607n1e8c83dbv4eb908f8b510614c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3100}{adcf5e800810010904p54a2c6c2me53f58d49b7ad2f3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3103}{b164d84d0810011330v7490d77anfe26edcea639d3c7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3107}{op.uh82yxa655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3116}{48E894CF.80506\%40gmx.de}
\@namedef{freecol-developers.mbox_3123}{48E9EBDC.5070202\%40free.fr}
\@namedef{freecol-developers.mbox_3130}{48EAEF2B.7080701\%40gmx.de}
\@namedef{freecol-developers.mbox_3117}{op.uijzqjcl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3118}{48E8D18F.5080004\%40gmx.de}
\@namedef{freecol-developers.mbox_3119}{BAY137-W53B3820540B53303FCECE5C5410\%40phx.gbl}
\@namedef{freecol-developers.mbox_3127}{48EAECD7.2060109\%40gmx.de}
\@namedef{freecol-developers.mbox_3121}{op.uij9kyde55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3128}{48EAEE0A.50103\%40gmx.de}
\@namedef{freecol-developers.mbox_3122}{op.uikjyzi455t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3129}{48EAEEEE.9030109\%40gmx.de}
\@namedef{freecol-developers.mbox_3125}{op.uil4etp255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3126}{48EAEC09.3060506\%40gmx.de}
\@namedef{freecol-developers.mbox_3134}{b164d84d0810071451k4605d60fje40a789167ff14b6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3135}{6DF18694590443318377169D8ED2A487\%40miti.local}
\@namedef{freecol-developers.mbox_3137}{48EC3F69.7050205\%40gmx.de}
\@namedef{freecol-developers.mbox_3141}{b164d84d0810081033m3186b761vb83b74085d2fbe80\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3138}{48EC4081.40305\%40gmx.de}
\@namedef{freecol-developers.mbox_3142}{b164d84d0810081110h2fade7cnf2365cf0ae691846\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3147}{48EEE1E3.4020004\%40gmx.de}
\@namedef{freecol-developers.mbox_3153}{op.uis8ag1355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3156}{48F05B3E.4050605\%40gmx.de}
\@namedef{freecol-developers.mbox_3161}{op.uiuxh7ej55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3143}{48EDBDB3.5020006\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3144}{op.uiq3mt1g55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3146}{200810092041.02025.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_3148}{48EEE38D.8080007\%40gmx.de}
\@namedef{freecol-developers.mbox_3164}{48F0F755.40506\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3166}{48F21E5D.2080900\%40gmx.de}
\@namedef{freecol-developers.mbox_3168}{48F25122.4050505\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3172}{48F36DD8.5090707\%40gmx.de}
\@namedef{freecol-developers.mbox_3180}{48F6CBAC.1040003\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3186}{48F76F41.8060801\%40gmx.de}
\@namedef{freecol-developers.mbox_3188}{op.ui4okixe55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3194}{48F8A9A1.9060303\%40gmx.de}
\@namedef{freecol-developers.mbox_3189}{2ce9650b0810161313i32956c2eq6ebfd68a7be32d81\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3195}{48F8A9C8.50702\%40gmx.de}
\@namedef{freecol-developers.mbox_3149}{48EEE2B9.4000401\%40catprint.ca}
\@namedef{freecol-developers.mbox_3150}{48EEEAA8.1080701\%40gmx.de}
\@namedef{freecol-developers.mbox_3152}{8C572C44-5E89-4C28-9C2D-33C704E1478A\%40optusnet.com.au}
\@namedef{freecol-developers.mbox_3155}{48F05A9A.9090502\%40gmx.de}
\@namedef{freecol-developers.mbox_3154}{200810102353.18995.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3157}{48F0601B.7010701\%40gmx.de}
\@namedef{freecol-developers.mbox_3160}{48F08750.70606\%40gmx.de}
\@namedef{freecol-developers.mbox_3162}{200810112155.41015.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3163}{48F0945F.6020707\%40gmx.de}
\@namedef{freecol-developers.mbox_3158}{6B3AAFF8-D90F-4DDC-BB66-38FD160CFE7A\%40optusnet.com.au}
\@namedef{freecol-developers.mbox_3159}{48F07433.4000808\%40gmx.de}
\@namedef{freecol-developers.mbox_3165}{960955110810111146w1d0bb84di9cf6a48b97985ea0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3167}{48F24F5C.5030003\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3170}{48F360AF.6080806\%40gmx.de}
\@namedef{freecol-developers.mbox_3182}{200810162107.12053.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3187}{48F7706C.2030309\%40gmx.de}
\@namedef{freecol-developers.mbox_3192}{48F82D7B.7040301\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3193}{48F8A8A2.9020202\%40gmx.de}
\@namedef{freecol-developers.mbox_3196}{200810181201.58698.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3200}{48F99036.3020501\%40gmx.de}
\@namedef{freecol-developers.mbox_3205}{op.ui94j9ed55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3206}{adcf5e800810191533g21b025a5w8245b2c1d7617ba9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3267}{op.uj7pynwv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3268}{588c53d774a809877fd70c20b2359f64.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3231}{op.ujq4ppe155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3232}{49088CB8.3080201\%40gmx.de}
\@namedef{freecol-developers.mbox_3242}{200810312216.00332.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3198}{48F967E5.9080405\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3199}{48F98E26.2090706\%40gmx.de}
\@namedef{freecol-developers.mbox_3176}{op.ui13zkq92817da\%40thimphu.pcpool.mi.fu-berlin.de}
\@namedef{freecol-developers.mbox_3197}{48F95AFB.7020800\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3201}{48F995B5.1040407\%40gmx.de}
\@namedef{freecol-developers.mbox_3202}{200810182107.22062.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3203}{48FAB7FD.1060901\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3204}{48FAF006.6050201\%40gmx.de}
\@namedef{freecol-developers.mbox_3207}{op.ujbhvtep55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3208}{200810222047.51897.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3209}{op.ujfcemyk55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3211}{200810241636.29656.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3212}{200810242306.24643.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3213}{op.uji8byf055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3220}{4902E401.9030003\%40gmx.de}
\@namedef{freecol-developers.mbox_3214}{49028D41.7050208\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3215}{200810251457.42499.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3219}{4902E2BD.4070402\%40gmx.de}
\@namedef{freecol-developers.mbox_3217}{4902E18B.20904\%40gmx.de}
\@namedef{freecol-developers.mbox_3218}{4902E079.7030300\%40gmx.de}
\@namedef{freecol-developers.mbox_3223}{200810261643.50097.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3225}{490431D1.1040502\%40gmx.de}
\@namedef{freecol-developers.mbox_3226}{200810262028.38568.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3210}{op.ujhx17v655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3216}{4902E1E0.8080205\%40gmx.de}
\@namedef{freecol-developers.mbox_3233}{op.ujs3ojs055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3234}{49094692.60800\%40gmx.de}
\@namedef{freecol-developers.mbox_3236}{4909DFEC.9000500\%40gmx.de}
\@namedef{freecol-developers.mbox_3240}{op.ujuo9g2k55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3265}{op.uj5001ps55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3266}{op.uj51xfmr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3221}{490327A3.9030005\%40gmx.de}
\@namedef{freecol-developers.mbox_3222}{490379CC.8070305\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3224}{49043099.7030906\%40gmx.de}
\@namedef{freecol-developers.mbox_3227}{49057399.3080101\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3228}{op.ujpbu5bw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3229}{200810282041.30374.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3230}{49074BBE.5060200\%40gmx.de}
\@namedef{freecol-developers.mbox_3235}{200810302035.15114.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3237}{4909E379.4050106\%40gmx.de}
\@namedef{freecol-developers.mbox_3238}{4909E6B8.1000806\%40gmx.de}
\@namedef{freecol-developers.mbox_3249}{200811032053.18999.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3251}{op.uj1of0dt55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3257}{490F29B0.5040004\%40gmx.de}
\@namedef{freecol-developers.mbox_3260}{200811040810.17734.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3263}{200811042112.00437.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3239}{4909E940.2060703\%40gmx.de}
\@namedef{freecol-developers.mbox_3241}{op.ujurcwih55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3243}{490C1D26.6040305\%40gmx.de}
\@namedef{freecol-developers.mbox_3244}{490D54FC.4040607\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3245}{490D872D.3030406\%40gmx.de}
\@namedef{freecol-developers.mbox_3246}{490DE76E.5000803\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3248}{adcf5e800811021546q7582a6bbh95ada1935c65224c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3250}{op.uj1mqi1355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3255}{490F3AEA.4090009\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3295}{491EA404.109\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3258}{490F2A3E.8090805\%40gmx.de}
\@namedef{freecol-developers.mbox_3247}{000501c93d12$3fcd13c0$bf673b40$\%40de}
\@namedef{freecol-developers.mbox_3252}{20081103142712.M13757\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3254}{490F2801.9030409\%40gmx.de}
\@namedef{freecol-developers.mbox_3253}{20081103190749.M79903\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3269}{20081109221158.M30021\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3256}{490F3CC5.8020700\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3259}{op.uj1v9xw055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3270}{4917A51D.6040401\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3271}{op.ukeeydky55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3272}{20081110104919.M72926\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3273}{op.ukepsnkb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3274}{20081110174456.M13098\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3297}{491EA899.30604\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3275}{491910D8.1060909\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3277}{20081111085129.M5569\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3278}{200811112042.25555.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3280}{20081111102933.M49254\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3281}{op.ukgs6kzl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3283}{20081111173509.M39028\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3285}{op.ukir2fsl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3287}{20081113103816.M79504\%40tfh-berlin.de}
\@namedef{freecol-developers.mbox_3289}{491C700D.8060107\%40gmx.de}
\@namedef{freecol-developers.mbox_3292}{2ce9650b0811140135k54740681ub6f7e611ccf7f5ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3284}{491A5B8B.6030708\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3279}{op.ukf9wcnj55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3261}{42191DB76A4144BCBD90A3FF4B342819\%40miti.local}
\@namedef{freecol-developers.mbox_3262}{200811042006.57876.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3264}{BLU107-W23A763683E82FF48551454D11C0\%40phx.gbl}
\@namedef{freecol-developers.mbox_3276}{49192618.8040507\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3282}{op.ukgukyuv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3286}{491BDCF2.7040205\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3290}{491C7098.7080507\%40gmx.de}
\@namedef{freecol-developers.mbox_3291}{op.ukklnywh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3288}{0015174c0c72b6d8be045b902cf4\%40google.com}
\@namedef{freecol-developers.mbox_3293}{7b94298e0811141227s27f01a72o14c74c8bb972b861\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3294}{491E8D1C.7050801\%40gmx.de}
\@namedef{freecol-developers.mbox_3296}{491EA748.7050105\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3309}{200811162118.54066.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_3298}{7b94298e0811150331sfa66bfcj1acf0884a233408a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3299}{491EB728.2080408\%40gmx.de}
\@namedef{freecol-developers.mbox_3300}{7b94298e0811150356w6b8cf753ne68a1c07199a72bd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3302}{491EBE50.6030702\%40gmx.de}
\@namedef{freecol-developers.mbox_3303}{7b94298e0811150441n2b903cf7x98768c55a2bd077a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3308}{200811162120.57414.sergiocambra\%40users.sourceforge.net}
\@namedef{freecol-developers.mbox_3310}{200811172100.40997.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3301}{491EBE1F.5090501\%40gmx.de}
\@namedef{freecol-developers.mbox_3304}{200811160938.39084.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3305}{491FDFB8.3090601\%40gmx.de}
\@namedef{freecol-developers.mbox_3306}{49202A07.6050600\%40gmx.de}
\@namedef{freecol-developers.mbox_3315}{49250DC4.3010709\%40gmx.de}
\@namedef{freecol-developers.mbox_3316}{200811202208.17554.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3317}{49264AE5.4040002\%40gmx.de}
\@namedef{freecol-developers.mbox_3318}{200811212133.40828.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3319}{7b94298e0811210325o31ae283bi467ae6548985ad46\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3320}{20081121140631.169350\%40gmx.net}
\@namedef{freecol-developers.mbox_3323}{4927CB7D.8030204\%40gmx.de}
\@namedef{freecol-developers.mbox_3324}{200811222120.14878.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3325}{4927E520.8010208\%40gmx.de}
\@namedef{freecol-developers.mbox_3327}{200811230856.15308.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3336}{853eca16f66a1437d805ec43ff7fd1af.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3339}{200811242125.30106.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3346}{df777a08fe653f4785473202a0236c31.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3348}{200811252107.09916.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3307}{49202B29.60907\%40gmx.de}
\@namedef{freecol-developers.mbox_3311}{492271EE.5090606\%40gmx.de}
\@namedef{freecol-developers.mbox_3312}{7b94298e0811180435s65f039d9td7a79c9015867880\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3313}{4923A755.1070509\%40gmx.de}
\@namedef{freecol-developers.mbox_3314}{4923BA83.9070500\%40gmx.de}
\@namedef{freecol-developers.mbox_3321}{7b94298e0811211133s2f551772o6e035fc46070218e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3322}{4927BD2F.9080801\%40gmx.de}
\@namedef{freecol-developers.mbox_3326}{7b94298e0811220711x508a08e1r4a9082a69115f278\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3333}{op.uk2nlnji55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3335}{7b94298e0811230859v303a90cdpb985322eced38433\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3343}{op.uk4h4x2n55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3345}{7b94298e0811240554i3b4a02a8s689ac617c0ca9074\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3347}{op.uk49jiej55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3349}{7b94298e0811250426s246a1d69y944ab4b55630ada8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3350}{op.uk8dq6mw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3328}{7b94298e0811221759h3f6f1f85h542c0a5e67148c6c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3329}{7b94298e0811221811s51f04b53ne4e16c809766bdf6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3330}{49293AA6.4040205\%40gmx.de}
\@namedef{freecol-developers.mbox_3337}{200811240807.17892.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3338}{7b94298e0811240202r619bc8b7h7b572618797b2163\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3340}{7b94298e0811240319h42d8ee98y5f5d60e1f7f6337\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3331}{49293D3B.2030106\%40gmx.de}
\@namedef{freecol-developers.mbox_3332}{7b94298e0811230424u5486294fs4b97d06d2c1b88c4\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3334}{49295034.6010804\%40gmx.de}
\@namedef{freecol-developers.mbox_3351}{7b94298e0811261158y48e0705aj7204153ef737180c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3352}{7b94298e0811270318u6c9e969bj3dc1b78cb8d97b7e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3341}{200811242151.00230.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3342}{op.uk4gho1q55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3344}{7b94298e0811240539i4c25b7b2hb24dd2667b6921da\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3353}{200811272149.17310.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3354}{7b94298e0811270644s188d726dn1ad3e6242deeb0c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3355}{7b94298e0811290653k42c65f14t8020ba5ec3a315f0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3356}{493159A1.2090800\%40gmx.de}
\@namedef{freecol-developers.mbox_3357}{7b94298e0811291554t3c604337x84b26852484de0f8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3358}{7b94298e0811301619j49c770d1ubc299c62adcce105\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3359}{7b94298e0811301739q2adf35ecs4e279a0c56d5eaa8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3362}{49376D01.6090000\%40gmx.de}
\@namedef{freecol-developers.mbox_3363}{op.ulmm2mkm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3369}{4938C1CC.2040703\%40gmx.de}
\@namedef{freecol-developers.mbox_3371}{op.uloyvzap55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3360}{49337F40.3080201\%40gmx.de}
\@namedef{freecol-developers.mbox_3361}{200812011955.12662.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3364}{200812042051.21711.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3365}{7b94298e0812040727q1549612egcad7def793690559\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3366}{op.ulm9ubmi55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3367}{7b94298e0812040754y21c54cf5ybd939efb5fd49369\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3368}{op.ulnbdc1u55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3370}{200812052155.19641.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3374}{493A3876.7030101\%40gmx.de}
\@namedef{freecol-developers.mbox_3376}{7b94298e0812060317s6380c95bgb960833d3b96dbf2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3377}{7b94298e0812060319w5c856658ne46877b1204b3cbe\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3378}{493A622E.5090803\%40gmx.de}
\@namedef{freecol-developers.mbox_3379}{7b94298e0812060337w751d01fx2df9eed0aa77c422\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3382}{493A784D.5030301\%40gmx.de}
\@namedef{freecol-developers.mbox_3385}{op.ulywciew55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3386}{7b94298e0812101458sbd46878wa502e3f84e1aed49\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3389}{4941350E.9070203\%40gmx.de}
\@namedef{freecol-developers.mbox_3372}{7b94298e0812051839v17ed4de3r92f1d87ce108b51d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3373}{493A3664.6050306\%40gmx.de}
\@namedef{freecol-developers.mbox_3375}{493A5967.3010608\%40gmx.de}
\@namedef{freecol-developers.mbox_3380}{7b94298e0812060341k37b5e9ebwa0cc3f40de9b223d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3381}{493A777A.40206\%40gmx.de}
\@namedef{freecol-developers.mbox_3383}{493A8517.4030707\%40gmx.de}
\@namedef{freecol-developers.mbox_3384}{493D04AA.20305\%40gmx.de}
\@namedef{freecol-developers.mbox_3387}{200812112329.15009.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3390}{494139C8.3050205\%40gmx.de}
\@namedef{freecol-developers.mbox_3391}{200812120830.52006.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3388}{200812112347.39729.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3392}{49420DDD.4010702\%40gmx.de}
\@namedef{freecol-developers.mbox_3393}{20081215030824.bprer6aely0ccwos\%40webmail.ntnu.no}
\@namedef{freecol-developers.mbox_3396}{494754A0.3070009\%40gmx.de}
\@namedef{freecol-developers.mbox_3398}{49479F82.7090108\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3403}{4948933D.5090709\%40gmx.de}
\@namedef{freecol-developers.mbox_3394}{op.ul7i02bb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3395}{49474AF3.10704\%40gmx.de}
\@namedef{freecol-developers.mbox_3397}{200812162043.39368.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3399}{7b94298e0812160355h12521cadj8782b071f0b69b07\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3400}{7b94298e0812160350u588498a0q3a6526948aa69cd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3450}{op.umqo2ixm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3452}{4954A260.2050206\%40gmx.de}
\@namedef{freecol-developers.mbox_3453}{op.umrqmtmm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3454}{4954CA19.7060608\%40gmx.de}
\@namedef{freecol-developers.mbox_3511}{7b94298e0812301421x746c694dw771dddf9ffbdace3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3514}{495B34DF.3020809\%40gmx.de}
\@namedef{freecol-developers.mbox_3401}{7b94298e0812160356j5d5f0896w513c549e7afaddb3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3402}{op.ul9n6zim55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3404}{494969DB.8080900\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3409}{4949EDAC.5060105\%40gmx.de}
\@namedef{freecol-developers.mbox_3411}{200812182055.33667.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3412}{494A2862.5090403\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3413}{7b94298e0812180931i72e52c0cq5a18864d69c86628\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3414}{7b94298e0812180933g3cee246bv9b95071ecfa8a00c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3405}{49498563.1010203\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3407}{4949E8FB.8010407\%40gmx.de}
\@namedef{freecol-developers.mbox_3415}{494AC00B.6030503\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3417}{494B3056.3090509\%40gmx.de}
\@namedef{freecol-developers.mbox_3406}{49498A03.1020702\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3408}{4949EA12.4040305\%40gmx.de}
\@namedef{freecol-developers.mbox_3410}{494A2406.2030007\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3416}{494AD34C.4050902\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3418}{494B30A5.5000208\%40gmx.de}
\@namedef{freecol-developers.mbox_3419}{494CB81B.2010109\%40gmx.de}
\@namedef{freecol-developers.mbox_3420}{op.umgm2ll855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3421}{494D1398.7090706\%40gmx.de}
\@namedef{freecol-developers.mbox_3422}{op.umgxe6b955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3424}{200812221853.13712.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3425}{op.umkf0vjj55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3426}{494FD09F.8040106\%40gmx.de}
\@namedef{freecol-developers.mbox_3427}{20081222195239.0a028f45\%40schabi.de}
\@namedef{freecol-developers.mbox_3428}{op.umkzycuc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3429}{200812230755.31404.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3430}{op.umk8rhaz55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3436}{4952008A.2070507\%40gmx.de}
\@namedef{freecol-developers.mbox_3439}{op.umn37kjq55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3441}{495237DA.1010905\%40gmx.de}
\@namedef{freecol-developers.mbox_3445}{op.umpxdbsa55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3446}{49538374.6010900\%40gmx.de}
\@namedef{freecol-developers.mbox_3449}{op.umqokvk455t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3431}{7b94298e0812200447j2b3a470aw42b4a04451f59d61\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3423}{200812211135.27434.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3432}{200812232210.16249.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3433}{op.ummnbrnr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3434}{op.ummnoynl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3435}{200812240715.12881.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3437}{4952276A.9080207\%40gmx.de}
\@namedef{freecol-developers.mbox_3438}{op.umn2uxlv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3440}{495236B2.1010903\%40gmx.de}
\@namedef{freecol-developers.mbox_3442}{7b94298e0812241822u16afe71dvc9e3a8203cd92a63\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3443}{49536F3B.4010201\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3444}{op.umpvugeo55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3447}{7b94298e0812251211k375b9e58g88b12c30361aa0f2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3448}{op.umqodxoi55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3451}{4954A0DC.8080902\%40gmx.de}
\@namedef{freecol-developers.mbox_3455}{200812271019.20459.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3456}{7b94298e0812261832t70edd7f6o37af1d60528cad01\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3457}{200812271538.40312.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3459}{7b94298e0812270718n264b8db7v4645f219ae18ba33\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3461}{op.umtujzhl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3463}{7b94298e0812270756s20a8afbw860cd47c03bf65d1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3469}{200812281608.46600.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3476}{7b94298e0812280633k5136a138p718c2a244162d05e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3482}{200812291342.07390.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3460}{op.umtt6pl155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3464}{49566292.5050800\%40gmail.com}
\@namedef{freecol-developers.mbox_3466}{7b94298e0812270950g1ee360e5lf7cfa8deafa24501\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3465}{7b94298e0812270949v2ba3f762o86d2c17d8967a69d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3458}{op.umtqr8ky55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3484}{495882C1.1040901\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3486}{op.umxac81s55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3488}{4958C8B9.4000504\%40gmx.de}
\@namedef{freecol-developers.mbox_3517}{495B39AF.3040309\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3522}{495B6BA1.3060104\%40gmx.de}
\@namedef{freecol-developers.mbox_3512}{7b94298e0812301447l518dadcbrdceb18ca57293154\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3513}{7b94298e0812301504m57c95710q8d9ee07675a038c8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3515}{495B366D.9000008\%40gmx.de}
\@namedef{freecol-developers.mbox_3462}{49564F60.6090804\%40gmx.de}
\@namedef{freecol-developers.mbox_3468}{7b94298e0812271733pf92c99fs835621e6c0ac8e82\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3477}{495791A2.6040001\%40gmx.de}
\@namedef{freecol-developers.mbox_3478}{4957A2D4.6070103\%40gmx.de}
\@namedef{freecol-developers.mbox_3495}{7b94298e0812291258r22433f7pd77c9a5185d5970c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3496}{4959DEA9.8060104\%40gmx.de}
\@namedef{freecol-developers.mbox_3467}{op.umt9pwoa55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3480}{op.umv4zwsm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3485}{49588FFB.4050509\%40gmx.de}
\@namedef{freecol-developers.mbox_3487}{op.umxargbl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3489}{4958C8EA.9050304\%40gmx.de}
\@namedef{freecol-developers.mbox_3490}{op.umxh4et255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3491}{4958F50A.5000004\%40gmx.de}
\@namedef{freecol-developers.mbox_3492}{7b94298e0812291044nd4c1d8ct5e0857c6b441220b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3493}{7b94298e0812291045x10dca373t41e8e979e9f55dd2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3494}{op.umxvnshe55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3470}{49574917.4050306\%40gmx.de}
\@namedef{freecol-developers.mbox_3471}{op.umvgs7zb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3472}{op.umviojra55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3473}{4957841D.7090508\%40gmx.de}
\@namedef{freecol-developers.mbox_3475}{4957886B.8080208\%40gmx.de}
\@namedef{freecol-developers.mbox_3479}{op.umvxovcr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3483}{49588A65.10502\%40gmx.de}
\@namedef{freecol-developers.mbox_3481}{200812290906.18935.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3474}{495785AA.8040104\%40gmx.de}
\@namedef{freecol-developers.mbox_3497}{4959E682.9060401\%40gmx.de}
\@namedef{freecol-developers.mbox_3499}{200812302220.17560.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3498}{20081230122851.30c4d579\%40schabi.de}
\@namedef{freecol-developers.mbox_3500}{495A086C.8060504\%40gmx.de}
\@namedef{freecol-developers.mbox_3501}{495A197D.9060204\%40gmx.de}
\@namedef{freecol-developers.mbox_3502}{20081230141132.21117f49\%40schabi.de}
\@namedef{freecol-developers.mbox_3503}{495A33CA.9\%40gmx.de}
\@namedef{freecol-developers.mbox_3504}{20081230160540.47848bb1\%40schabi.de}
\@namedef{freecol-developers.mbox_3505}{495A466F.9070805\%40gmx.de}
\@namedef{freecol-developers.mbox_3506}{20081230172246.45d88ad0\%40schabi.de}
\@namedef{freecol-developers.mbox_3508}{495A5375.6050102\%40gmx.de}
\@namedef{freecol-developers.mbox_3510}{495A5BA9.7030503\%40gmx.de}
\@namedef{freecol-developers.mbox_3507}{20081230174156.354efccc\%40schabi.de}
\@namedef{freecol-developers.mbox_3516}{495B37FB.5030606\%40gmx.de}
\@namedef{freecol-developers.mbox_3509}{20081230180016.075110be\%40schabi.de}
\@namedef{freecol-developers.mbox_3518}{495B3A54.7000807\%40gmx.de}
\@namedef{freecol-developers.mbox_3519}{20081231112835.2fd8d6a0\%40schabi.de}
\@namedef{freecol-developers.mbox_3521}{495B6803.3080501\%40gmx.de}
\@namedef{freecol-developers.mbox_3520}{20081231120545.11ee9011\%40schabi.de}
\@namedef{freecol-developers.mbox_3523}{495B6E8F.1030808\%40gmx.de}
\@namedef{freecol-developers.mbox_3552}{20090102104232.7b761601\%40schabi.de}
\@namedef{freecol-developers.mbox_3553}{200901022109.45373.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3554}{20090102120117.4e869df1\%40schabi.de}
\@namedef{freecol-developers.mbox_3556}{495E03FE.7040502\%40gmx.de}
\@namedef{freecol-developers.mbox_3524}{op.um02u6rn55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3525}{7b94298e0812310701qc4f29c4j82b0873aa83397ea\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3526}{7b94298e0812310706q472832c6y422698b0ce9f2b00\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3527}{op.um1gz7hg55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3528}{200901011330.50477.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3529}{495C96C5.7020707\%40gmx.de}
\@namedef{freecol-developers.mbox_3530}{495C9DC8.20608\%40gmx.de}
\@namedef{freecol-developers.mbox_3531}{200901012156.44017.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3532}{495CB529.6080208\%40gmx.de}
\@namedef{freecol-developers.mbox_3533}{495CB6A4.6050507\%40gmx.de}
\@namedef{freecol-developers.mbox_3571}{200901032201.56663.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3572}{495F52C1.7080606\%40gmx.de}
\@namedef{freecol-developers.mbox_3600}{200901051952.41741.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3601}{BLU132-DS7D6DD3C3794508C10722C93E10\%40phx.gbl}
\@namedef{freecol-developers.mbox_3605}{7b94298e0901050508o2742aeetfe9822c7354236a8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3607}{4962F2F3.4000704\%40gmx.de}
\@namedef{freecol-developers.mbox_3610}{BLU132-DS2909E77DB2C9F14A119ED93DE0\%40phx.gbl}
\@namedef{freecol-developers.mbox_3618}{496448B9.5020909\%40gmx.de}
\@namedef{freecol-developers.mbox_3634}{7b94298e0901070733g5f731884o2272f415717bd6c8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3639}{7b94298e0901071026i19303f26t509829425317b7fb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3642}{BLU132-DS3E81739B9B9E3B0D0505093DF0\%40phx.gbl}
\@namedef{freecol-developers.mbox_3619}{49644AE2.9060200\%40gmx.de}
\@namedef{freecol-developers.mbox_3612}{20090106225736.1a32d7ff\%40schabi.de}
\@namedef{freecol-developers.mbox_3538}{7b94298e0901010930r128642eakcae5402d0667d353\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3540}{7b94298e0901011014y11cdd9d9nb20fb9f423d98bb2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3541}{7b94298e0901011020n38fa772bt8532605c2e33d920\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3542}{op.um3g2goh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3544}{7b94298e0901011230g47e410c7n6423a194ef333a07\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3548}{op.um3k6psf55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3555}{200901022152.46990.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3557}{495E051C.1010306\%40gmx.de}
\@namedef{freecol-developers.mbox_3558}{495E203C.3030606\%40gmx.de}
\@namedef{freecol-developers.mbox_3559}{7b94298e0901020721j2e63d2aevc7dccbb1410eb6a5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3561}{495E3983.1040808\%40gmx.de}
\@namedef{freecol-developers.mbox_3562}{op.um41ipp355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3563}{op.um5h64ag55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3568}{495F2B3B.3030005\%40gmx.de}
\@namedef{freecol-developers.mbox_3573}{op.um6jjdni55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3574}{495F555B.4040000\%40gmx.de}
\@namedef{freecol-developers.mbox_3577}{op.um6le8po55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3575}{495F55CD.6060108\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3576}{op.um6lemt355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3578}{495F6DDF.6050406\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3579}{495F717C.30800\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3580}{495F7390.2040404\%40gmx.de}
\@namedef{freecol-developers.mbox_3581}{op.um6tkjeo55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3560}{op.um4yb6gn55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3543}{op.um3hcc2n55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3545}{7b94298e0901011234u29e787b6nea0fb2aa4cb576df\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3546}{op.um3jf1en55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3549}{7b94298e0901011420i7d925575s33dee106021a93e6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3550}{495DDF8F.1040600\%40gmx.de}
\@namedef{freecol-developers.mbox_3534}{495CD571.5050000\%40gmx.de}
\@namedef{freecol-developers.mbox_3535}{7b94298e0901010730w640d14c7ya8ed7eb4eae5e990\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3536}{7b94298e0901010837kdc32ba1uc1fbcc538701a062\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3537}{op.um29adzr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3539}{7b94298e0901010956k58094b57vfafee809a61acc9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3547}{7b94298e0901011314v54ca5e00x4a69243ec0ea097a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3551}{495DDFBC.5070109\%40gmx.de}
\@namedef{freecol-developers.mbox_3564}{7b94298e0901022032m315d32b9n9282638908ae5621\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3565}{495F25EC.2000904\%40gmx.de}
\@namedef{freecol-developers.mbox_3566}{BLU132-DS729354F8B7A56E93E42EB93E30\%40phx.gbl}
\@namedef{freecol-developers.mbox_3567}{495F29E7.5080004\%40gmx.de}
\@namedef{freecol-developers.mbox_3569}{200901032043.47081.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3570}{495F3D57.9010305\%40gmx.de}
\@namedef{freecol-developers.mbox_3583}{7b94298e0901030829r7e47c64dyf8a9fe373426c931\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3585}{7b94298e0901031238p67fab453v713ae67b12e8d3e5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3582}{7b94298e0901030827u361553b5o2ae8979d072d9005\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3584}{7b94298e0901031001j52857394j8012f6f1a4fd14c7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3586}{49607F7A.80906\%40gmx.de}
\@namedef{freecol-developers.mbox_3587}{200901042148.16863.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3588}{4960A7A0.4060204\%40gmx.de}
\@namedef{freecol-developers.mbox_3589}{4960B95D.5040509\%40gmx.de}
\@namedef{freecol-developers.mbox_3590}{op.um8j1wcq55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3591}{7b94298e0901040626r11697c21i7177f03fc18589b9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3592}{4960C8EB.7050609\%40gmx.de}
\@namedef{freecol-developers.mbox_3595}{op.um80ojuh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3597}{4961A059.9090107\%40gmx.de}
\@namedef{freecol-developers.mbox_3604}{7b94298e0901050506t7d37acf9q6b122220afc6ef2b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3606}{op.unahe4r855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3667}{7b94298e0901081220r7b6bb209v6edaa5b9b0a34c7c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3674}{4966ECDD.9060800\%40gmx.de}
\@namedef{freecol-developers.mbox_3677}{20090109114411.1a23be99\%40schabi.de}
\@namedef{freecol-developers.mbox_3679}{op.unhla1x955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3681}{op.unhlngt555t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3682}{496747B4.6070004\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3684}{7b94298e0901090533l4c6da8a6m1ec36dd8b0694ed5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3689}{49676AF5.20001\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3691}{7b94298e0901091126l3cb164b6u87ff9cf9e4302524\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3692}{4967AC7D.8090808\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3693}{7b94298e0901091214h6b96897dycd74bbffe887650a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3694}{4967B49B.8050903\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3695}{7b94298e0901091354s309e8721h71e083c79a7b9aa0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3696}{7b94298e0901091412k68e84feetb5ab7081b2f88eaf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3697}{7b94298e0901091415s29473c25h1a8cf2d91a999ae7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3701}{49687E5F.8020706\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3707}{7b94298e0901100458x543048dbod54cc00d7fc8336f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3685}{7b94298e0901090605s63806748r5fd5641d75b498cf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3688}{op.unhvemff55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3710}{op.unjhkyij55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3721}{7b94298e0901101135x41c6f4d9hd8cbd79180b4fd65\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3686}{20090109150858.133de188\%40schabi.de}
\@namedef{freecol-developers.mbox_3687}{op.unhtznta55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3593}{7b94298e0901040802t73fbe8c6y9ffb3a663288db72\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3594}{7b94298e0901040808v13a443fav9d9d4677c08370b2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3666}{7b94298e0901081158j390faf27yb537cd55d2adaf3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3673}{4966EC1F.4060104\%40gmx.de}
\@namedef{freecol-developers.mbox_3596}{7b94298e0901041448i3f5f1cc8h22b39db745c8357e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3598}{4961A0E4.6040201\%40gmx.de}
\@namedef{freecol-developers.mbox_3599}{20090105100513.a898bc95.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3611}{eead3e9aa5928a13ced06f2aef79a78d.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3613}{7b94298e0901061451n1944fe25j94e3ae6c256d389d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3616}{496446BF.7070103\%40gmx.de}
\@namedef{freecol-developers.mbox_3620}{200901071908.05180.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3622}{20090107115414.4e8f3fc8.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3664}{7b94298e0901080936x310da176le6f6026c887ed64f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3665}{7b94298e0901081022y745507adh206e7e5e856a572c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3712}{ad7de84cb18a491f91b72ce48be83572.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3718}{7b94298e0901100859n44a30716kceecf80283ac2089\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3719}{66c890189121e011892ca8ba223fdeff.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3722}{7b94298e0901101228s78098ba8xd914bcd27941dc5b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3723}{cf7af800db69588241c3de6470fb7af9.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3724}{7b94298e0901101608h4aa30ff5y28aee5d99658095e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3725}{7b94298e0901101620l6dcf631aq41196412750ec966\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3742}{op.unnlwlyr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3745}{7b94298e0901121012v7e82a1dbu871b7c60c29b70dd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3752}{op.unn15pbr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3754}{7b94298e0901121618t42cf7e41v6cadfeddf5bd95b6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3758}{op.unoxk5u155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3756}{7b94298e0901121741h35625fadr85e217b251d7f6bc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3668}{7b94298e0901081241q1254ab70h8207ec5aceaa6361\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3675}{3408d4a94deb68fefc72bbf6ea86ffb0.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3602}{4961DD39.7020202\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3603}{4961DDC5.8040802\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3608}{4962F6E2.3020008\%40gmx.de}
\@namedef{freecol-developers.mbox_3609}{op.unb96cqm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3617}{496447BE.4\%40gmx.de}
\@namedef{freecol-developers.mbox_3614}{7b94298e0901061933n2c9423f9vc6a38699da5b7ab6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3615}{496445B1.2060208\%40gmx.de}
\@namedef{freecol-developers.mbox_3627}{adcf5e800901070505w5dd702c2gada28f1270a3679e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3629}{7b94298e0901070547j53f9a813kc179221b583de3b8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3632}{20090107145738.1592f144\%40schabi.de}
\@namedef{freecol-developers.mbox_3621}{20090107105308.0a02ba1f\%40schabi.de}
\@namedef{freecol-developers.mbox_3630}{7b94298e0901070550k128b58efhe0ab195ea9807835\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3623}{op.undu0kd655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3625}{op.undxw7nv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3635}{7b94298e0901070850ked32d3fv777b17e11e3d6062\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3636}{op.unedg1u355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3637}{op.unedq1er55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3647}{op.unetslgb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3649}{7b94298e0901071702x4c2fd623jf582aec064d21790\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3626}{op.undxf6vc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3633}{7b94298e0901070727m1f194427gd27c82010251da8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3638}{op.uneeuilb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3643}{20090107201743.3ad0bd26\%40schabi.de}
\@namedef{freecol-developers.mbox_3644}{7b94298e0901071122y448ff5a3w10ea4abf47167272\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3645}{op.unep3c1t55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3648}{7b94298e0901071701n377d3b97g9e86c273d43ab714\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3651}{op.unfgp6b855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3655}{op.unflvojp55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3663}{7b94298e0901080928x66bfdacwfc89ebc42ceb3a1b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3678}{20090109114831.4059e731\%40schabi.de}
\@namedef{freecol-developers.mbox_3680}{BLU132-DS5C8B7B869F2A6F321564093DD0\%40phx.gbl}
\@namedef{freecol-developers.mbox_3683}{7b94298e0901090521s7535391dhc0f24787b5f4bc44\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3624}{op.undybp0g55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3640}{7b94298e0901071100w780718b5r524ff50e5d1ebefc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3641}{4964FCD1.803\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3646}{op.uneqdgfz55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3650}{7b94298e0901071718m59d3579fq1d676b007d6cafd8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3652}{4965B03D.501\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3653}{4965B3BD.8050809\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3654}{4965B3E7.9010203\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3669}{4966E8A6.4090007\%40gmx.de}
\@namedef{freecol-developers.mbox_3702}{op.unjiqffl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3706}{4968990B.1\%40gmx.de}
\@namedef{freecol-developers.mbox_3628}{adcf5e800901070523h2809f4ddn3be6aa1ea7e0e312\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3631}{20090107150053.300ea990\%40schabi.de}
\@namedef{freecol-developers.mbox_3656}{4965E0E5.4020203\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3670}{4966E90D.5060005\%40gmx.de}
\@namedef{freecol-developers.mbox_3657}{20090108154345.476b100a\%40korb.intern.schabi.de}
\@namedef{freecol-developers.mbox_3671}{4966E989.90708\%40gmx.de}
\@namedef{freecol-developers.mbox_3658}{20090108162455.2a1d1cf0\%40korb.intern.schabi.de}
\@namedef{freecol-developers.mbox_3659}{20090108162612.048cf6a3\%40korb.intern.schabi.de}
\@namedef{freecol-developers.mbox_3660}{49661D4A.7020200\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3662}{20090108165504.3ea39cdb\%40korb.intern.schabi.de}
\@namedef{freecol-developers.mbox_3698}{49685C45.4000400\%40gmx.de}
\@namedef{freecol-developers.mbox_3704}{20090110123952.0bdc53bf\%40schabi.de}
\@namedef{freecol-developers.mbox_3661}{20090108165201.166e81c3\%40korb.intern.schabi.de}
\@namedef{freecol-developers.mbox_3672}{4966EAFF.6010706\%40gmx.de}
\@namedef{freecol-developers.mbox_3690}{20090109175847.146cee20\%40schabi.de}
\@namedef{freecol-developers.mbox_3676}{2ce9650b0901090108m5f3175b7r4e2087fe9bb1245e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3699}{49685E12.6030809\%40gmx.de}
\@namedef{freecol-developers.mbox_3700}{2ce9650b0901100246j39604033s3ca63580a04db4ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3703}{20090110130436.34adca01\%40schabi.de}
\@namedef{freecol-developers.mbox_3709}{op.unjmffkc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3728}{4969C5AE.6050305\%40gmx.de}
\@namedef{freecol-developers.mbox_3729}{op.unlcevra55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3730}{4969E0FF.4010807\%40gmx.de}
\@namedef{freecol-developers.mbox_3733}{496A2176.50800\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3705}{20090110134737.2563668b\%40schabi.de}
\@namedef{freecol-developers.mbox_3708}{20090110140013.5cc5850a\%40schabi.de}
\@namedef{freecol-developers.mbox_3711}{4968C16B.5080603\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3713}{4968C1AD.4020308\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3714}{71a3bad7d9e4ab3c75b85438f0ef77a1.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3715}{op.unjt0utw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3716}{f48b37a31326f54dc6f69933b71c57e2.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3717}{f11256ad494fdbb93a7dd7c4562025e6.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3727}{4969C55F.1080007\%40gmx.de}
\@namedef{freecol-developers.mbox_3720}{7b94298e0901101130n83393fav24be1ee03f81a218\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3726}{4969C4D8.1030401\%40gmx.de}
\@namedef{freecol-developers.mbox_3734}{op.unlstfs755t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3731}{4969D981.9010700\%40gmx.de}
\@namedef{freecol-developers.mbox_3743}{7b94298e0901121007l6eebea27i1cafe283379d2794\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3732}{9795763bd027ffdfd82eb438a1039833.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3739}{7b94298e0901120832vc40bc8ftf12d5e6900f69103\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3740}{7b94298e0901120833w2b2cca04m2dbbd8591532a56b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3760}{496CBED8.7090701\%40gmx.de}
\@namedef{freecol-developers.mbox_3769}{7b94298e0901131152k66d74128n8a376bf3cd8b14bf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3770}{651ea77419a5f6fd085041acb55f7daf.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3772}{7b94298e0901131258s6c221b87y352f0a732a260a7d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3775}{c2323fff2265edb26ab41b3e5d00b608.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3773}{77a9f0bd3163703ddb504ab294cc97d4.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3774}{7b94298e0901131613ofa164c7udc5c99da71fc6637\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3778}{20090114131652.4f06f2d4\%40schabi.de}
\@namedef{freecol-developers.mbox_3779}{7b94298e0901140525m327423d1yf94dc560650aab90\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3735}{op.unm790ld55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3736}{20090112132709.05307145\%40schabi.de}
\@namedef{freecol-developers.mbox_3737}{496B385D.9000606\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3738}{op.unnakfal55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3741}{20090112190634.972fd61e.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3759}{496CBE2B.9070401\%40gmx.de}
\@namedef{freecol-developers.mbox_3761}{496CC616.9090500\%40gmx.de}
\@namedef{freecol-developers.mbox_3762}{20090113190434.f428df57.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3763}{496CCD08.3020507\%40gmx.de}
\@namedef{freecol-developers.mbox_3764}{496CD6A7.30103\%40gmx.de}
\@namedef{freecol-developers.mbox_3765}{20090113200926.4152bb14.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3766}{op.unpjvr0455t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3768}{496CEADF.2080101\%40gmx.de}
\@namedef{freecol-developers.mbox_3777}{op.unqu1ad855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3781}{496E0431.8090208\%40gmx.de}
\@namedef{freecol-developers.mbox_3784}{op.unrbrljb55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3783}{496E09D2.6030001\%40gmx.de}
\@namedef{freecol-developers.mbox_3744}{op.unnosyef55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3746}{7b94298e0901121103u16f2fccbx2bcc1032db14e165\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3767}{7b94298e0901131123j3b98df1ctb6845f0dd61edf3c\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3747}{op.unntptoo55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3749}{7b94298e0901121227m4476b59bwfcf4d1c91ab2aaa0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3748}{op.unntwpzx55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3750}{7b94298e0901121246k1a350156r46347c05d9938d22\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3751}{7b94298e0901121248k2866b4f0p82e2660be9e573a3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3753}{op.unn2lwqu55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3755}{7b94298e0901121749u69d3d7a7o88a6c77f673a3adf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3757}{722531.6182.qm\%40web111104.mail.gq1.yahoo.com}
\@namedef{freecol-developers.mbox_3771}{20090113221115.f7348276.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3776}{op.unqs7r1y55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3780}{0dc2e5059dfff72174f895c7f764e591.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3782}{496E0696.201\%40gmx.de}
\@namedef{freecol-developers.mbox_3785}{8ba8edced21e5cfdb108cbd968b610fc.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3786}{b82194a00901141953g4b3a23bjbf3b47fe2bb273b6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3787}{496F6CBC.70502\%40gmx.de}
\@namedef{freecol-developers.mbox_3788}{7b94298e0901151200r38f6d1dev219ed6ed4eef7405\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3790}{op.unte9thp55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3791}{49703884.8000608\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3793}{op.unun0qn655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3797}{4970A655.5040305\%40gmx.de}
\@namedef{freecol-developers.mbox_3789}{op.untd8l0t55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3792}{49703A9A.3000304\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3799}{4970A800.2020503\%40gmx.de}
\@namedef{freecol-developers.mbox_3798}{4970A6AE.8070400\%40gmx.de}
\@namedef{freecol-developers.mbox_3794}{op.unul63b255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3795}{op.unurnpjc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3796}{op.unus6ulp55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3800}{4970AD0C.6000901\%40gmx.de}
\@namedef{freecol-developers.mbox_3816}{op.unwkiv0355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3801}{4970B092.9050703\%40gmx.de}
\@namedef{freecol-developers.mbox_3802}{501f5b5d0901160834n479e931djdadbf234ab5d950a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3803}{4970B953.2000301\%40gmx.de}
\@namedef{freecol-developers.mbox_3805}{501f5b5d0901160926qe56a8c5oc5ab21c53c19301e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3808}{4970C7FD.6060105\%40gmx.de}
\@namedef{freecol-developers.mbox_3854}{200901271136.13324.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3858}{497F25F5.4020007\%40gmx.de}
\@namedef{freecol-developers.mbox_3809}{7b94298e0901161038v6b4d2ce8v38f7f6455ac04a0e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3804}{4a4665cf905716f34ea8fe59fc37241f.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3806}{BLU132-DS32645902D9B8D6D2FC64793D40\%40phx.gbl}
\@namedef{freecol-developers.mbox_3807}{4970C754.5080601\%40gmx.de}
\@namedef{freecol-developers.mbox_3810}{1114e5af64525958ff68904757fadc6e.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3813}{49719D7B.2030103\%40gmx.de}
\@namedef{freecol-developers.mbox_3814}{20090117133546.62a982df.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3818}{4971DF63.6000909\%40gmx.de}
\@namedef{freecol-developers.mbox_3821}{20090117193009.f70acfb2.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3815}{op.unwjtbvr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3817}{4971DC35.6050100\%40gmx.de}
\@namedef{freecol-developers.mbox_3819}{op.unwuc2ph55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3822}{fc03774cf86a1f44a3752766e46afc1c.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3823}{op.unw2yug755t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3827}{8b91d5d906a1088d7fe0393ff405be8e.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3834}{op.unyjqqyi55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3842}{op.un3q1th355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3843}{4978090C.8070101\%40gmx.de}
\@namedef{freecol-developers.mbox_3847}{op.un9tbyix55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3848}{497C1332.1050104\%40gmx.de}
\@namedef{freecol-developers.mbox_3852}{op.uodgyob555t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3824}{4972F2FB.1000201\%40gmx.de}
\@namedef{freecol-developers.mbox_3828}{b5c833d703359c09ecc12a357f4b4d91.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3849}{200901262108.39707.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3851}{497DDBEE.6060306\%40gmx.de}
\@namedef{freecol-developers.mbox_3855}{200901272128.00908.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3856}{497F1FBB.2070107\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3857}{497F259D.4030104\%40gmx.de}
\@namedef{freecol-developers.mbox_3966}{031801c9a600$898056b0$9c810410$\%40net}
\@namedef{freecol-developers.mbox_3967}{200903162137.25873.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3970}{49BF3EE9.5070805\%40gmx.de}
\@namedef{freecol-developers.mbox_3972}{200903172042.41668.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3969}{49BF3DB8.2030605\%40gmx.de}
\@namedef{freecol-developers.mbox_3853}{op.uodhlej755t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3833}{op.unyeflsr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3841}{7b94298e0901190436w46920757q5e5bb351c93a859d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3811}{7b94298e0901161335y76b3b3d6sbb56ffbf5859f9a8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3812}{4971971F.1030508\%40gmx.de}
\@namedef{freecol-developers.mbox_3820}{7b94298e0901170915o51d110c1u43bd173367edf4f9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3850}{200901262150.09908.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3825}{4972F408.1080701\%40gmx.de}
\@namedef{freecol-developers.mbox_3829}{90badddbeea0aa734f4d6f45943dea48.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3830}{497305F4.1050809\%40gmx.de}
\@namedef{freecol-developers.mbox_3831}{49730CED.9070906\%40gmx.de}
\@namedef{freecol-developers.mbox_3832}{49731E7B.9090205\%40gmx.de}
\@namedef{freecol-developers.mbox_3826}{4972F965.6030306\%40gmx.de}
\@namedef{freecol-developers.mbox_3836}{op.unyojmi355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3840}{497426A1.3080904\%40gmx.de}
\@namedef{freecol-developers.mbox_3835}{20090118170818.658ca6eb\%40schabi.de}
\@namedef{freecol-developers.mbox_3838}{49741496.8000500\%40gmx.de}
\@namedef{freecol-developers.mbox_3837}{op.unyw7cnw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3839}{49742340.1020003\%40gmx.de}
\@namedef{freecol-developers.mbox_3844}{7b94298e0901220950r94d1687hd3d945330e6ab52\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3845}{4979581E.3060000\%40gmx.de}
\@namedef{freecol-developers.mbox_3846}{49797012.100\%40gmx.de}
\@namedef{freecol-developers.mbox_3859}{op.uogwahyw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3860}{20090128125215.154460\%40gmx.net}
\@namedef{freecol-developers.mbox_3861}{49847F8D.7080302\%40gmx.de}
\@namedef{freecol-developers.mbox_3862}{49856571.6050307\%40gmx.de}
\@namedef{freecol-developers.mbox_3866}{c50d13f97f5cee8cc0b52f8166ae4460.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3863}{49856738.6050107\%40gmx.de}
\@namedef{freecol-developers.mbox_3864}{49856C77.2090900\%40gmx.de}
\@namedef{freecol-developers.mbox_3865}{5adea11ae7ad50679f280b783c055e92.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3953}{7b94298e0903101224r6fa301dbrffb48d8983594ab5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3954}{d13676f5b52a828789e49bee4ec34c7f.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3955}{200903110747.54374.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3956}{200903112046.49883.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3959}{4881436bcaef2e7eaf28e32d76368359.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3960}{d599572851e56609432ec26dba35d1aa.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3962}{7b94298e0903140957mddc22d5q53a00f8e779e9510\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3957}{7b94298e0903111443r1c06ea63jb750f7c410a72513\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3867}{op.uoxnsjj555t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3868}{498D4BC2.4000909\%40gmx.de}
\@namedef{freecol-developers.mbox_3870}{op.uo1arelu55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3871}{498EDE54.5010508\%40gmx.de}
\@namedef{freecol-developers.mbox_3869}{498D55F9.5080802\%40gmx.de}
\@namedef{freecol-developers.mbox_3872}{498F063F.10903\%40gmx.de}
\@namedef{freecol-developers.mbox_3873}{49905D95.1080402\%40gmx.de}
\@namedef{freecol-developers.mbox_3874}{op.uo4xwpjv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3875}{4991A362.1000207\%40gmx.de}
\@namedef{freecol-developers.mbox_3876}{op.uo5gtsc555t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3877}{580990fe0902101353g5916db0di466565ff64b59fd0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3880}{op.uo6oi9hx55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3882}{4992F584.7090702\%40gmx.de}
\@namedef{freecol-developers.mbox_3883}{op.uo8o0wxh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3891}{op.upcnk7ul55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3892}{4996F1DD.9030606\%40gmx.de}
\@namedef{freecol-developers.mbox_3878}{op.uo6ka9ex55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3879}{200902112017.00248.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3881}{op.uo6o79to55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3884}{49945C85.4010207\%40gmx.de}
\@namedef{freecol-developers.mbox_3885}{200902132058.26908.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3886}{49958D82.8090006\%40gmx.de}
\@namedef{freecol-developers.mbox_3887}{8833b90cc3b73a4b41f3c26943bddf97.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3888}{49969308.6080701\%40gmx.de}
\@namedef{freecol-developers.mbox_3889}{200902142055.32920.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3895}{580990fe0902150352g24d9fcc6pc8493c0999e09fc3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3890}{4996C5ED.1080504\%40gmx.de}
\@namedef{freecol-developers.mbox_3893}{46bcf0a68b2deb766d6536d8a356fb0a.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3894}{op.upd4p0zg55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3896}{op.upd7hpas55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3897}{580990fe0902150451ra3d50bdw24b6b2cc38b9eda\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3898}{49981A89.10202\%40gmx.de}
\@namedef{freecol-developers.mbox_3899}{op.upeg6kwn55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3900}{24631B5C-67F0-4F00-B075-EF44E68F0CA0\%40nickshanks.com}
\@namedef{freecol-developers.mbox_3901}{49991703.2050200\%40gmx.de}
\@namedef{freecol-developers.mbox_3902}{580990fe0902160214r11c248e0t295d44c38a37e71a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3903}{op.upf3xclw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3904}{580990fe0902160852h25a0d7a6y40b8ae9a04698f0b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3907}{op.upghsle655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3908}{580990fe0902161043i6ab966eer8d7f4f83897ef207\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3909}{op.upgl5nrz55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3911}{200902171950.36813.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3910}{ce8f6bf898ae9251b0f27c7d5eece815.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3912}{op.uphyyodk55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3919}{499C2D25.3030808\%40gmx.de}
\@namedef{freecol-developers.mbox_3930}{9CCAC3E1-AA5F-4023-BBD4-2B2479451CEC\%40nickshanks.com}
\@namedef{freecol-developers.mbox_3905}{2ce9650b0902160902n3c7afc67g8c689c0e8ad5525f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3906}{580990fe0902161000l7898e210t87ec844eb6f45b33\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3913}{200902182053.23429.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3914}{499BE40D.70909\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_3915}{op.upjocanq55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3916}{200902182256.09214.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3918}{op.upjulrth55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3924}{200902192043.40177.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3926}{op.upliiczt55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3927}{200902192345.21051.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3917}{20090218135110.c4d05b3d.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3920}{op.upkb7sm855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3921}{20090218221419.c17b87ca.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3922}{499CF37E.5040502\%40gmx.de}
\@namedef{freecol-developers.mbox_3923}{op.uplfxhdn55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3928}{20090219133038.a89decab.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_3929}{op.uplqopbc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3925}{op.uplgulim55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_3931}{1e9600396b17c5e492f613d20c59e24c.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3934}{499FED57.8070805\%40gmx.de}
\@namedef{freecol-developers.mbox_3933}{34c733bdd5ee5d211036d1a59f7de522.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3932}{499FF1E7.3080304\%40gmx.de}
\@namedef{freecol-developers.mbox_3935}{200902231824.13714.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3937}{49A2CD6E.1040704\%40gmx.de}
\@namedef{freecol-developers.mbox_3936}{11739057.1235395819583.JavaMail.root\%40webmail01.superonline.com}
\@namedef{freecol-developers.mbox_3940}{49A42CCD.2000003\%40gmx.de}
\@namedef{freecol-developers.mbox_3971}{014701c9a6da$448fb5c0$cdaf2140$\%40net}
\@namedef{freecol-developers.mbox_3938}{d0c098564212.49a2a239\%40shaw.ca}
\@namedef{freecol-developers.mbox_3939}{49A42383.1040905\%40gmx.de}
\@namedef{freecol-developers.mbox_3941}{49AB7916.8040706\%40gmx.de}
\@namedef{freecol-developers.mbox_3942}{ccd806ea0903020419k2dbd33e6r5122c0dc7fb78076\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3943}{580990fe0903020854q141049d0ifb574b33491b503\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3945}{49AD587B.3050305\%40gmx.de}
\@namedef{freecol-developers.mbox_3944}{fb55f61d0903021333h2f3a4ca0g83726491e105f809\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3946}{49AD5B1C.3060005\%40gmx.de}
\@namedef{freecol-developers.mbox_3947}{580990fe0903030937ua8853f5k303af7be9c6046dd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3948}{59442d52458f8f625b55b4adace9dedf.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3949}{49AE1601.3030502\%40gmx.de}
\@namedef{freecol-developers.mbox_3950}{200903052024.39807.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3951}{49B0B636.9010002\%40gmx.de}
\@namedef{freecol-developers.mbox_3952}{49B0BD59.8030800\%40gmx.de}
\@namedef{freecol-developers.mbox_3958}{49BA938D.8020000\%40gmx.de}
\@namedef{freecol-developers.mbox_3961}{7b94298e0903140955x32c695byab2e269afac22ef\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3963}{7b94298e0903141200g450a9f91r32dbb64f45d9158b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3964}{49BCE855.5060704\%40gmx.de}
\@namedef{freecol-developers.mbox_3965}{49BCFC41.8030202\%40gmx.de}
\@namedef{freecol-developers.mbox_3973}{200903172115.42290.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3974}{49C2766E.1060607\%40gmx.de}
\@namedef{freecol-developers.mbox_3975}{4408b5f5c93201a9d889331a91f47a96.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3976}{49C4A4ED.7030407\%40gmx.de}
\@namedef{freecol-developers.mbox_3978}{b81359575fe9572a378daf426af93302.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3979}{49C619F0.9000108\%40gmx.de}
\@namedef{freecol-developers.mbox_3968}{247962.79215.qm\%40web52412.mail.re2.yahoo.com}
\@namedef{freecol-developers.mbox_3977}{49C60EBC.5080407\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3981}{49C61CBD.90408\%40gmx.de}
\@namedef{freecol-developers.mbox_3982}{200903222152.34534.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3984}{3ab65d239f96672d5b5a1f4aa7347e0e.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_3985}{49C67A85.3000906\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3986}{49C7390B.5030903\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3989}{7b94298e0903230454v361c9e31y2ee351626da31ee9\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3988}{200903232125.00788.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3980}{49C61A5E.9080209\%40gmx.de}
\@namedef{freecol-developers.mbox_3983}{7b94298e0903220612y34f7e2e9rf175c8d77b692830\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3987}{200903231924.35409.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3990}{200903241134.18802.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3996}{49CDE233.1070402\%40gmx.de}
\@namedef{freecol-developers.mbox_3997}{200903282032.05350.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_3991}{88F2CD8F-1B0C-4801-B2E1-4870BF25A9B8\%40gmail.com}
\@namedef{freecol-developers.mbox_3992}{501f5b5d0903240136s66d7417j9c484c04830286ec\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3993}{49C9DFDE.9010103\%40metaintegration.net}
\@namedef{freecol-developers.mbox_3995}{49CDE023.8050400\%40gmx.de}
\@namedef{freecol-developers.mbox_3994}{7327d4e0903261315m3b294473v778a741f9fca589a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_3998}{49CDDF49.4090002\%40gmx.de}
\@namedef{freecol-developers.mbox_3999}{49D44FB1.7070605\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4000}{200904021956.21194.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4002}{49D59358.7020009\%40gmx.de}
\@namedef{freecol-developers.mbox_4003}{200904032104.13314.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4004}{op.urs8t7zh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4005}{003801c9b4a2$a2e63fb0$e8b2bf10$\%40net}
\@namedef{freecol-developers.mbox_4006}{7598ef817770dc3304be27f18f3c4e62.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4008}{49D709BE.3040507\%40gmx.de}
\@namedef{freecol-developers.mbox_4007}{49D70725.3040908\%40gmx.de}
\@namedef{freecol-developers.mbox_4001}{49D58D01.7010201\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4012}{49D75099.6040502\%40gmx.de}
\@namedef{freecol-developers.mbox_4014}{49D7F401.2050002\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4015}{49D7FF13.4010503\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4016}{op.urwo0pka55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4019}{49D89574.1030501\%40gmx.de}
\@namedef{freecol-developers.mbox_4020}{49D91BD2.9000408\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4021}{op.urxmln0h55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4024}{200904062000.25021.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4026}{49DC2A26.9020307\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4017}{op.urwpprzs55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4018}{49D894C7.4040700\%40gmx.de}
\@namedef{freecol-developers.mbox_4022}{200904060758.26669.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4023}{49D996BD.2060908\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4312}{7b94298e0907021022l3c73b1fal513dc1e7b711be00\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4009}{34800cdb7062f07252a7b314aff76375.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4013}{49D7ACAD.6000607\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4010}{980d2f3b4ad80c9b32414d5072a86416.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4011}{49D75008.3080201\%40gmx.de}
\@namedef{freecol-developers.mbox_4025}{200904062120.55692.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4027}{49DC36C5.6030809\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4028}{49DC45B6.60008\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4036}{200904112103.24967.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4037}{49E088B5.8090506\%40gmx.de}
\@namedef{freecol-developers.mbox_4029}{49DD6D0C.3090002\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4030}{49DD6F31.4070806\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4035}{49E0384A.6000105\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4038}{49E1EA51.4080209\%40gmx.de}
\@namedef{freecol-developers.mbox_4039}{49E2CB6C.9060600\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4040}{49E2E831.1030700\%40gmx.de}
\@namedef{freecol-developers.mbox_4031}{49DD725E.8000901\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4032}{49DEB231.7070000\%40metaintegration.net}
\@namedef{freecol-developers.mbox_4033}{200904101308.46468.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4034}{49DEFF4A.9020102\%40gmx.de}
\@namedef{freecol-developers.mbox_4041}{7b94298e0904181149s71f25515x8bbaf3f78d620d68\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4042}{7b94298e0904181203s257812qfe43db39f2ffa711\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4043}{200904190717.12620.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4044}{6305C0BF-E397-40F7-AC9D-80E3338F60A7\%40rumms.uni-mannheim.de}
\@namedef{freecol-developers.mbox_4045}{200904251856.17504.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4046}{49F30695.8040407\%40gmx.de}
\@namedef{freecol-developers.mbox_4047}{200904252247.38569.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4048}{49F30F43.10500\%40gmx.de}
\@namedef{freecol-developers.mbox_4049}{200904272139.52669.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4050}{49F68C52.8060509\%40gmx.de}
\@namedef{freecol-developers.mbox_4051}{6e5148e60904290116p6ea9de5exab0c1035ab48cbae\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4052}{op.us54a2ks55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4057}{49FC659D.5080108\%40gmx.de}
\@namedef{freecol-developers.mbox_4058}{7b94298e0905021004nf380d0bo7e012546bb874ac\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4061}{49FD3831.3030808\%40gmx.de}
\@namedef{freecol-developers.mbox_4070}{6e5148e60905040503y59000827x115dafce92080065\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4072}{49FF0722.80402\%40gmx.de}
\@namedef{freecol-developers.mbox_4073}{575E9EE1-AE91-41A2-B4C3-EE4F1E7E51DA\%40nickshanks.com}
\@namedef{freecol-developers.mbox_4074}{7b94298e0905050629t200fe5dfxe0b4d6f82adc1de2\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4064}{cf2744b7999412e17022419416a3564f.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4067}{49FD7913.9010103\%40gmx.de}
\@namedef{freecol-developers.mbox_4068}{op.utde19fw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4071}{49FF05FE.601\%40gmx.de}
\@namedef{freecol-developers.mbox_4053}{49FBF34A.7030209\%40gmx.de}
\@namedef{freecol-developers.mbox_4054}{200905021852.28649.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4055}{501f5b5d0905020327k22e2656fy4bd88b0377b3e15b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4056}{49FC4C52.4070301\%40gmx.de}
\@namedef{freecol-developers.mbox_4059}{200905031126.21306.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4060}{49FD3557.2080000\%40gmx.de}
\@namedef{freecol-developers.mbox_4062}{f2005221dd65676b5f878cf9ce768662.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4063}{b3d70940241fd197c1486aca3414b8f6.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4065}{200905031956.10819.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4066}{820c1c0e00047ea223dcee8d6deb5a97.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4069}{920b971d45ceaba1ce9a723d9c0bd8cb.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4075}{7b94298e0905050757i21aad38bp713e87b2ba53d6a1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4076}{200905062208.54082.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4077}{op.utihifsr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4078}{4A01A4CB.5000102\%40gmx.de}
\@namedef{freecol-developers.mbox_4082}{op.utjt58oq55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4083}{200905072023.09833.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4087}{4A030178.1050207\%40gmx.de}
\@namedef{freecol-developers.mbox_4090}{200905081844.55270.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4095}{4A05A401.3090205\%40gmx.de}
\@namedef{freecol-developers.mbox_4079}{4A01A582.4020409\%40gmx.de}
\@namedef{freecol-developers.mbox_4080}{7b94298e0905061021t237b1a39gdb349df19e263950\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4081}{7b94298e0905061049t1c3ca989hc3abfcb497025fd1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4088}{4A030352.1030100\%40gmx.de}
\@namedef{freecol-developers.mbox_4084}{200905072113.24348.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4085}{op.utj9y5ca55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4086}{4A030044.70303\%40gmx.de}
\@namedef{freecol-developers.mbox_4091}{200905081849.36435.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4092}{op.utlujkf155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4093}{200905081959.13611.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4094}{op.utl0nu1055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4089}{4A0310B1.3030204\%40gmx.de}
\@namedef{freecol-developers.mbox_4097}{7b94298e0905100811pcaaafc6u9bc301af704688d6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4096}{4A06AA9E.6\%40gmx.de}
\@namedef{freecol-developers.mbox_4098}{op.utqb7zwq55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4099}{4A07BF98.6040003\%40gmx.de}
\@namedef{freecol-developers.mbox_4100}{21587bd960088019ba6acd1cc92b116f.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4101}{501f5b5d0905112353s3b1fa5e2tba1eb36ab39afd1e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4102}{200905130852.34387.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4103}{4A0A74B1.8090600\%40gmx.de}
\@namedef{freecol-developers.mbox_4104}{20090513101453.84a33d9f.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4106}{4A0BCAB3.6030000\%40gmx.de}
\@namedef{freecol-developers.mbox_4105}{200905141122.22966.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4107}{4A0BEB2E.8000204\%40gmx.de}
\@namedef{freecol-developers.mbox_4149}{op.uuafp1i455t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4151}{4A163201.2060004\%40gmx.de}
\@namedef{freecol-developers.mbox_4152}{op.uubve1gm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4153}{op.uubv41aa55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4154}{4A1693E7.5050709\%40gmx.de}
\@namedef{freecol-developers.mbox_4156}{op.uub0evm655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4157}{4A16A7B2.5060401\%40gmx.de}
\@namedef{freecol-developers.mbox_4158}{op.uudor6di55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4159}{4A18EE46.1000404\%40gmx.de}
\@namedef{freecol-developers.mbox_4160}{op.uufl34uw55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4161}{op.uuf83n0h55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4162}{4A1A4DCC.2010503\%40gmx.de}
\@namedef{freecol-developers.mbox_4163}{op.uuhfotg955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4164}{580990fe0905251320u3e861a4an939afa98184302d8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4165}{4A1B92D3.40202\%40gmx.de}
\@namedef{freecol-developers.mbox_4166}{21FB9E22-0A9E-4AB0-BBE4-81934252BDF3\%40nickshanks.com}
\@namedef{freecol-developers.mbox_4167}{4A1CE261.8030009\%40gmx.de}
\@namedef{freecol-developers.mbox_4173}{op.uuk8hraz55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4175}{4A1D3EB9.3060208\%40gmx.de}
\@namedef{freecol-developers.mbox_4178}{op.uunmhybe55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4179}{4A1FAD7C.9030800\%40gmx.de}
\@namedef{freecol-developers.mbox_4182}{op.uuoxtsio55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4194}{4A2233DB.7030803\%40gmx.de}
\@namedef{freecol-developers.mbox_4195}{op.uusmgsof55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4196}{4A227F90.3060003\%40gmx.de}
\@namedef{freecol-developers.mbox_4197}{op.uusux31255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4198}{4A237D27.3000206\%40gmx.de}
\@namedef{freecol-developers.mbox_4199}{op.uuuhedcf55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4108}{4A0E5F02.8020704\%40gmx.de}
\@namedef{freecol-developers.mbox_4110}{200905161914.47260.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4109}{4A0E6DA8.6000206\%40gmx.de}
\@namedef{freecol-developers.mbox_4111}{200905161923.46786.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4114}{op.ut2ovgus55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4115}{4A10F1A5.7040701\%40gmx.de}
\@namedef{freecol-developers.mbox_4117}{4A10F8F9.2030004\%40gmx.de}
\@namedef{freecol-developers.mbox_4125}{op.ut4g7mcy55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4126}{4A114925.3040107\%40gmx.de}
\@namedef{freecol-developers.mbox_4129}{7b94298e0905181306g51230c08l252d662d54a4619\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4130}{op.ut48h8ve55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4131}{7b94298e0905181522h468d942u59d9ebb118ab2a4a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4132}{4A124343.30004\%40gmx.de}
\@namedef{freecol-developers.mbox_4141}{op.ut6eqtf855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4112}{4A0E992D.8030509\%40gmx.de}
\@namedef{freecol-developers.mbox_4113}{200905172118.17654.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4116}{4A10F35B.7050705\%40gmx.de}
\@namedef{freecol-developers.mbox_4118}{20090518094411.bf4ce11a.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4119}{4A11135D.5090504\%40gmx.de}
\@namedef{freecol-developers.mbox_4121}{20090518115420.020990d7.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4123}{200905181939.33596.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4124}{20090518131909.ae3f99eb.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4127}{7b94298e0905180509n42c43982w255500c1be82b3fd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4138}{200905192009.27166.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4140}{7b94298e0905190421t61736e68s2681a5baf09209eb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4143}{200905200732.49582.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4120}{BLU137-W350FF10BA1EF0A826161E0C45D0\%40phx.gbl}
\@namedef{freecol-developers.mbox_4122}{4A111F20.9030708\%40gmx.de}
\@namedef{freecol-developers.mbox_4128}{7b94298e0905180447i288d4cb6u854336c83c50a117\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4133}{4A126B8E.50509\%40gmx.de}
\@namedef{freecol-developers.mbox_4134}{200905191919.21903.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4135}{20090519125523.ccc0e072.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4136}{7b94298e0905190319w1bec16bekcd19fef5d5ff099b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4137}{4A128A98.9030804\%40gmx.de}
\@namedef{freecol-developers.mbox_4139}{7b94298e0905190354v5adbed0apc97232c2ce92f84a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4142}{4A12B636.2050409\%40gmx.de}
\@namedef{freecol-developers.mbox_4144}{4A138CC4.1040604\%40gmx.de}
\@namedef{freecol-developers.mbox_4145}{op.ut8sfvyr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4146}{4A15224C.9050304\%40gmx.de}
\@namedef{freecol-developers.mbox_4150}{20090521212543.17a34f22.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4147}{200905212057.08017.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4148}{4A153E02.50108\%40gmx.de}
\@namedef{freecol-developers.mbox_4200}{7b94298e0906010738p65b3fbl1fc6f5d87d663ff3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4201}{7b94298e0906010744v51e5aee6wadd7a51addabbd2b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4203}{200906022109.08130.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4155}{4A169589.4030200\%40gmx.de}
\@namedef{freecol-developers.mbox_4168}{4A1CE5E4.8060709\%40gmx.de}
\@namedef{freecol-developers.mbox_4170}{op.uuk2grs155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4171}{200905272021.10279.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4169}{4A1D083C.1000905\%40gmx.de}
\@namedef{freecol-developers.mbox_4172}{200905272032.22519.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4174}{4A1D3C2D.6040506\%40gmx.de}
\@namedef{freecol-developers.mbox_4176}{502583.80714.qm\%40web44803.mail.sp1.yahoo.com}
\@namedef{freecol-developers.mbox_4177}{4A1E3CF3.9010401\%40gmx.de}
\@namedef{freecol-developers.mbox_4180}{200905291940.10009.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4181}{7b94298e0905290536h18b17809rc90b4b5cffcd50d3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4183}{op.uuow8hpm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4185}{4A1FEB91.2080103\%40gmx.de}
\@namedef{freecol-developers.mbox_4190}{4A20EDFD.50108\%40gmx.de}
\@namedef{freecol-developers.mbox_4191}{200905302013.10934.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4193}{200905302205.38266.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4184}{4A1FE0E6.7070506\%40gmx.de}
\@namedef{freecol-developers.mbox_4187}{7b94298e0905291041j278e1914ncae489804b0e9fd3\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4188}{4A20E35A.7060309\%40gmx.de}
\@namedef{freecol-developers.mbox_4192}{200905302202.13702.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4186}{37fed22b0905290748p5ed47aedo66ea51b5efc8135\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4189}{4A20E450.2070505\%40gmx.de}
\@namedef{freecol-developers.mbox_4283}{3a7129160906271308w156045aaq906fd3cfe77ed875\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4310}{4A4CCCF2.4030502\%40gmx.de}
\@namedef{freecol-developers.mbox_4365}{3a7129160907150603u508efb55udf06e41ad2a36806\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4373}{4A5F3705.60108\%40gmx.de}
\@namedef{freecol-developers.mbox_4375}{3a7129160907161249i1c8c83fcvabe1d9f951736497\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4387}{4A617EAC.3030206\%40gmx.de}
\@namedef{freecol-developers.mbox_4393}{3a7129160907181130w2955c4d1o5a667d8946a1666e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4402}{4A62F3DE.1050109\%40gmx.de}
\@namedef{freecol-developers.mbox_4202}{op.uuv1ufia55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4204}{4A253EEE.8090803\%40gmx.de}
\@namedef{freecol-developers.mbox_4205}{op.uuwqcvy455t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4206}{4A256053.5060402\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_4207}{op.uuwuifmc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4208}{4A257673.5030704\%40stud.ntnu.no}
\@namedef{freecol-developers.mbox_4214}{4A269233.2060906\%40gmx.de}
\@namedef{freecol-developers.mbox_4209}{200906030724.06841.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4212}{op.uux2ozda55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4213}{200906032044.04771.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4228}{127295.40771.qm\%40web58305.mail.re3.yahoo.com}
\@namedef{freecol-developers.mbox_4231}{op.uu9dcvli55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4237}{914004.5296.qm\%40web58306.mail.re3.yahoo.com}
\@namedef{freecol-developers.mbox_4240}{op.uvbg0o0055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4241}{4A2E7E6D.4060203\%40gmx.de}
\@namedef{freecol-developers.mbox_4236}{17801.59339.qm\%40web58301.mail.re3.yahoo.com}
\@namedef{freecol-developers.mbox_4238}{op.uvazqnlr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4210}{4A264296.40306\%40gmail.com}
\@namedef{freecol-developers.mbox_4215}{4A26938A.5010402\%40gmx.de}
\@namedef{freecol-developers.mbox_4216}{580990fe0906040648k289f57b2s68fd65d5e21c5498\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4217}{4A27DB2B.3040402\%40gmx.de}
\@namedef{freecol-developers.mbox_4221}{37fed22b0906050327w1ee74dddnc8f5a81a64dd9f97\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4222}{200906052024.22744.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4223}{4A2A216E.8040702\%40gmx.de}
\@namedef{freecol-developers.mbox_4225}{4A2A25BC.90802\%40gmail.com}
\@namedef{freecol-developers.mbox_4226}{4A2A299A.8060204\%40gmx.de}
\@namedef{freecol-developers.mbox_4227}{4A2A2CE7.9030405\%40gmail.com}
\@namedef{freecol-developers.mbox_4244}{4A3246EB.5070604\%40gmail.com}
\@namedef{freecol-developers.mbox_4246}{4A335AA2.6000108\%40gmx.de}
\@namedef{freecol-developers.mbox_4211}{op.uux15dq255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4218}{4A27E2FD.1050504\%40gmail.com}
\@namedef{freecol-developers.mbox_4219}{4A27E809.8080608\%40gmx.de}
\@namedef{freecol-developers.mbox_4220}{op.uu0owal855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4224}{4A2A2246.7040608\%40gmx.de}
\@namedef{freecol-developers.mbox_4245}{4A32590F.2010006\%40gmail.com}
\@namedef{freecol-developers.mbox_4247}{4A335EA5.2060506\%40gmx.de}
\@namedef{freecol-developers.mbox_4248}{4A33975E.5080104\%40gmail.com}
\@namedef{freecol-developers.mbox_4249}{4A33A737.5090004\%40gmx.de}
\@namedef{freecol-developers.mbox_4267}{4A421BAC.70706\%40gmail.com}
\@namedef{freecol-developers.mbox_4287}{4A478F7F.10605\%40gmx.de}
\@namedef{freecol-developers.mbox_4290}{4A48D5FB.5010706\%40gmx.de}
\@namedef{freecol-developers.mbox_4229}{200906092123.15342.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4230}{op.uu9bjjum55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4233}{4A2E80FA.7080104\%40gmx.de}
\@namedef{freecol-developers.mbox_4234}{20090609194144.284b55cf.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4239}{200906102229.28608.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4232}{7b94298e0906090517v41c41e10t7e3ba16771e12248\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4235}{20090609195253.2b7b28af.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4242}{4A312053.9090403\%40gmx.de}
\@namedef{freecol-developers.mbox_4243}{20090611200449.43289af3.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4250}{4A34D958.807\%40gmx.de}
\@namedef{freecol-developers.mbox_4251}{20090614150943.e9f7c1a5.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4252}{7b94298e0906140745v27e3d733x3621c2bf566325cc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4253}{op.uviseos555t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4254}{7b94298e0906141028r2f250e55tc685a787eeeba368\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4255}{op.uvi06tnm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4256}{4A366682.2050407\%40gmx.de}
\@namedef{freecol-developers.mbox_4257}{op.uvkst6lx55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4258}{op.uvsmfifo55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4259}{4A3C95E0.3020403\%40gmx.de}
\@namedef{freecol-developers.mbox_4260}{op.uvtoansx55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4261}{4A3CE8EA.8080904\%40gmx.de}
\@namedef{freecol-developers.mbox_4262}{4A41B467.6010003\%40gmx.de}
\@namedef{freecol-developers.mbox_4263}{97544.85192.qm\%40web58308.mail.re3.yahoo.com}
\@namedef{freecol-developers.mbox_4271}{4A43052D.10006\%40gmx.de}
\@namedef{freecol-developers.mbox_4264}{200906242024.54773.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4265}{op.uv00w7u055t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4273}{4A43078B.3050505\%40gmx.de}
\@namedef{freecol-developers.mbox_4269}{7b94298e0906241628k3e9bdccl7ee96bbd41ba9cdf\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4274}{4A430EEB.9060409\%40gmx.de}
\@namedef{freecol-developers.mbox_4275}{20090625121004.0b6b01bc.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4294}{7b94298e0906300712o2953e250o156eff783e41834\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4297}{200907012008.08253.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4298}{4A4B72D0.4080606\%40gmx.de}
\@namedef{freecol-developers.mbox_4301}{7b94298e0907011048u37be5114o69176610abe95c22\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4304}{op.uweiifpt55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4309}{4A4CCB1B.60200\%40gmx.de}
\@namedef{freecol-developers.mbox_4302}{7b94298e0907011054x7ae5ae23xb69d606245b70ac1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4308}{4A4CCC73.40600\%40gmx.de}
\@namedef{freecol-developers.mbox_4313}{7b94298e0907021310r1d3d4c95s82624f8292de10d0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4322}{4A4E188A.30105\%40gmx.de}
\@namedef{freecol-developers.mbox_4295}{7b94298e0906300718vdd60aa4la96bcaea2b64758a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4296}{200906302144.33803.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4299}{7b94298e0907011028t7565b53ajab5c1a5b97d8fcd6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4305}{4A4CCA01.4030701\%40gmx.de}
\@namedef{freecol-developers.mbox_4311}{op.uwf7l6an55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4315}{7b94298e0907021641p7a4ff67di5a2a13e5967f3679\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4324}{4A4E1A02.3010204\%40gmx.de}
\@namedef{freecol-developers.mbox_4325}{7b94298e0907030751r29be0292tf20a6486d65b81f7\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4341}{200907092143.09856.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4348}{4A586964.8020708\%40gmx.de}
\@namedef{freecol-developers.mbox_4350}{580990fe0907111156w4f73913byb976d05458a2b58\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4354}{4A59D859.5090204\%40gmx.de}
\@namedef{freecol-developers.mbox_4351}{7b94298e0907111200q2ccf97f3sf3f911ef221eed07\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4353}{7b94298e0907111236m4da20256y2362c2225d1e641\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4316}{7b94298e0907021736p61a00a75t28b5de0b990cc58b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4318}{7b94298e0907021719y4889b951k27cebec49bd53c63\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4320}{200907032046.06379.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4321}{7b94298e0907030652t50a70290hb934be7f2242c469\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4327}{4A4E1BB8.6060509\%40gmx.de}
\@namedef{freecol-developers.mbox_4328}{7b94298e0907030801i16275c8ajfda240c57f3ae40d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4346}{200907102106.54215.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4300}{7b94298e0907011045o255682a5naaf7a339f1df10cc\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4306}{4A4CCA83.7030603\%40gmx.de}
\@namedef{freecol-developers.mbox_4333}{4A4F0C5A.4000709\%40gmx.de}
\@namedef{freecol-developers.mbox_4334}{7b94298e0907041318j5203c143mf03c38a1e3533590\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4317}{7b94298e0907021726i5083ea02p809bffd071d5cd03\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4335}{7b94298e0907042110k652d669ana851fe8a3e356569\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4338}{4A54250B.4080001\%40gmx.de}
\@namedef{freecol-developers.mbox_4336}{7b94298e0907051237v746c44f8u2643c1bd76532a93\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4337}{200907062113.55434.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4339}{4A5424D8.3020607\%40gmx.de}
\@namedef{freecol-developers.mbox_4374}{7b94298e0907160952q2d2850c0y44c7451aef88b650\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4388}{4A617F9C.8000007\%40gmx.de}
\@namedef{freecol-developers.mbox_4401}{200907191528.58972.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4342}{op.uwuhpjwg55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4343}{580990fe0907100322w2e68a03x1ca39307ec9f6a1e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4347}{4A58686F.9050009\%40gmx.de}
\@namedef{freecol-developers.mbox_4344}{200907102003.34598.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4345}{200907102023.00355.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4363}{7b94298e0907141734m21a96c72o44c7e0cba750db\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4364}{7b94298e0907150405x2919bf0eh98d9c934dc6b5e1b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4394}{30fee1458094c8159a9386550fca897a.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4404}{4A631F67.3090606\%40gmx.de}
\@namedef{freecol-developers.mbox_4405}{7b94298e0907190724g776db08fybbaa8cd36ac7af50\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4408}{c5eb7541c1a6e9d1b440d49ebcd90fae.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4411}{7b94298e0907191158g306a704lbecd91abb22aabc1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4417}{200907212102.16048.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4419}{5ce2015f90f48399d36895a87c6561b9.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4421}{4A669CB9.6030407\%40gmx.de}
\@namedef{freecol-developers.mbox_4424}{47be75349d9b658db6dea4e777b25af0.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4427}{200907222136.25021.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4429}{b19ade0727293301977274e4475b91bb.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4430}{a3283285f932daeb0129632f5f4dabf2.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4436}{4A67ECCF.70808\%40gmx.de}
\@namedef{freecol-developers.mbox_4458}{e4db9f0379e0d1a86c414e435a5f584e.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4463}{4A73F036.6050203\%40gmx.de}
\@namedef{freecol-developers.mbox_4435}{4A67EBCA.1090308\%40gmx.de}
\@namedef{freecol-developers.mbox_4366}{7b94298e0907150747m14b8dc7ak2dc59c339972392d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4368}{op.uw369zx355t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4369}{200907160746.37699.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4370}{op.uw5c7ntu55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4371}{200907161930.24931.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4372}{op.uw5ygnbv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4380}{200907170747.33753.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4381}{op.uw7c10mi55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4460}{op.uxwgr2wt55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4378}{7b94298e0907161343h40c0be84w4e795a7e15a705e1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4382}{op.uw7d3bkd55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4385}{4A617D67.3010603\%40gmx.de}
\@namedef{freecol-developers.mbox_4416}{200907212050.43593.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4266}{200906242125.10945.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4268}{7b94298e0906240515m1768ad30oe3a9497b0922395b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4270}{op.uv04xjek55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4272}{4A4306E1.2020605\%40gmx.de}
\@namedef{freecol-developers.mbox_4276}{200906251907.31769.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4278}{op.uv216hks55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4277}{200906251908.45935.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4279}{4A445181.7010201\%40gmx.de}
\@namedef{freecol-developers.mbox_4280}{7b94298e0906260926s380c121fxd6c24c43968e22f8\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4281}{200906272143.57391.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4284}{200906281223.40425.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4285}{4A474088.7010807\%40gmx.de}
\@namedef{freecol-developers.mbox_4288}{7b94298e0906281700l48ee4093r158985540c049930\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4289}{4A48D21C.3090803\%40gmx.de}
\@namedef{freecol-developers.mbox_4291}{7b94298e0906291330y38045110y73d732eba5139ea5\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4292}{200906300722.38062.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4293}{7b94298e0906291829h34fe0200u4ec8bf702fb61eeb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4282}{fc1f98245e5e.4a45fc6d\%40uwo.ca}
\@namedef{freecol-developers.mbox_4286}{4A478F2F.7050504\%40gmx.de}
\@namedef{freecol-developers.mbox_4314}{op.uwgjujjv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4323}{4A4E1929.6090100\%40gmx.de}
\@namedef{freecol-developers.mbox_4329}{op.uwhyx3fl55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4331}{4A4E2297.7040804\%40gmx.de}
\@namedef{freecol-developers.mbox_4303}{7b94298e0907011103o5cb16baeq18afab36b41ef6ab\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4307}{4A4CCBF1.80904\%40gmx.de}
\@namedef{freecol-developers.mbox_4319}{op.uwhkvmdf55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4326}{4A4E1B4A.50006\%40gmx.de}
\@namedef{freecol-developers.mbox_4330}{op.uwhzlgof55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4332}{4A4E22F9.4020609\%40gmx.de}
\@namedef{freecol-developers.mbox_4418}{op.uxfe16w255t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4340}{4A542C4B.3060103\%40gmx.de}
\@namedef{freecol-developers.mbox_4349}{4A587885.6050404\%40gmx.de}
\@namedef{freecol-developers.mbox_4352}{7b94298e0907111228h64fb0d56me8408d7ddec7269\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4355}{4A59DA5B.1050307\%40gmx.de}
\@namedef{freecol-developers.mbox_4356}{7b94298e0907120632x316ca2a2ne23ec9fa030e5f02\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4357}{op.uwyjyyut55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4358}{4A59F426.1000602\%40gmx.de}
\@namedef{freecol-developers.mbox_4359}{7b94298e0907120744o445cffe5s80066360ea6888cd\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4360}{4A5A038E.3030406\%40gmx.de}
\@namedef{freecol-developers.mbox_4361}{200907130807.24183.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4362}{7b94298e0907141348u2bdbf5b7uca4730a45afc6a3f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4367}{7b94298e0907150800m11df4b3x9e670bbe8912a85f\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4383}{op.uw7ghgjm55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4384}{7b94298e0907170758p7312bb73kd6a22f1a1f108802\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4389}{op.uw9kjkgr55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4390}{4A61CF2A.9080507\%40gmx.de}
\@namedef{freecol-developers.mbox_4397}{op.uxadrfnv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4398}{d6f9ca5c77d684b431a8e1b574865dca.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4400}{7b94298e0907181642m5897fecdn53a48e2166c720b1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4376}{7b94298e0907161308g1a0e43e3rbf97bc2f7e38c780\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4377}{7b94298e0907161324w8763bd9pf4f6ac1daf34a636\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4379}{7b94298e0907161423j47618996sbbd987bf80000330\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4386}{4A617E5E.40702\%40gmx.de}
\@namedef{freecol-developers.mbox_4391}{ad69eb3953fca3e11a9997c00bb6eb68.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4395}{7b94298e0907181157t9b861dr892b202f472ab15d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4396}{002eb324845280c5596ac7113369c6d3.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4399}{7b94298e0907181627r7df8b81fnc26536404e98ab75\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4415}{580990fe0907201130g5c0533ach2c8923c3b87d51d0\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4459}{op.uxwfbccs55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4392}{ba36b850da6891149cba59ac96dccd4e.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4403}{4A62F79E.900\%40gmx.de}
\@namedef{freecol-developers.mbox_4406}{7b94298e0907190817k12b01a16u4beec2f70174285d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4407}{7b94298e0907190820i85303b2j76896655de5250fb\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4409}{0a6a8a6e48c62c28699f4157ae27d7b3.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4410}{7b94298e0907191156o736b6f61k6836d3ed001e31e1\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4412}{1584fa23ee0f41b4ded7f6691a1990ed.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4414}{44956.19036.qm\%40web112219.mail.gq1.yahoo.com}
\@namedef{freecol-developers.mbox_4413}{4A63FD02.3010905\%40gmx.de}
\@namedef{freecol-developers.mbox_4426}{200907222120.30637.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4420}{4A669A62.5010708\%40gmx.de}
\@namedef{freecol-developers.mbox_4423}{63ac13c1d5e8c65bcb9adbc98fc30ec0.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4428}{7b94298e0907220557ha1065b1kbff08f1336716b1e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4434}{4A67E8FE.7010602\%40gmx.de}
\@namedef{freecol-developers.mbox_4422}{4A669D39.5030009\%40gmx.de}
\@namedef{freecol-developers.mbox_4425}{3853ef202716e87b40dd18a74ce45fbd.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4431}{7b94298e0907221159t1f9b9d26yde550524a27a199a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4432}{7b94298e0907221411v2606db33o4b893c309b73287e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4437}{4A67ED9E.1000102\%40gmx.de}
\@namedef{freecol-developers.mbox_4433}{7b94298e0907221725o204bce89re591b0166b654c41\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4438}{7b94298e0907231438m30e8e16ch5e465bcda6bb2a7a\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4439}{4A693E0F.4060003\%40gmx.de}
\@namedef{freecol-developers.mbox_4440}{612e21350907231924o2cd3ebchf3ba7ddc4207d569\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4441}{4A6ACDEC.9020601\%40gmx.de}
\@namedef{freecol-developers.mbox_4442}{200907282148.19418.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4443}{4A6F150A.4060207\%40gmx.de}
\@namedef{freecol-developers.mbox_4445}{200907292021.16372.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4444}{580990fe0907281204h17e201dfu34f954942994762e\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4447}{200907292152.00296.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4448}{op.uxtyp5h655t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4451}{200907302108.12518.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4454}{op.uxvr9j0x55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4461}{200907312223.21977.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4456}{4A71BA7D.1040906\%40gmx.de}
\@namedef{freecol-developers.mbox_4462}{200907312230.53636.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4464}{4A73F1CA.7030004\%40gmx.de}
\@namedef{freecol-developers.mbox_4449}{4A705FF5.5030800\%40gmx.de}
\@namedef{freecol-developers.mbox_4455}{4A71B68E.9070609\%40gmx.de}
\@namedef{freecol-developers.mbox_4496}{4A7D79F2.9090107\%40gmx.de}
\@namedef{freecol-developers.mbox_4446}{200907292106.51433.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4450}{7b94298e0907291707l34ceb294v7bb0b719a891032b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4468}{200908012102.50439.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4470}{4A743153.7090307\%40gmx.de}
\@namedef{freecol-developers.mbox_4488}{200908040714.57457.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4490}{7b94298e0908040522g634f003cpbd973dbd71dd2e7b\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4493}{200908050722.43861.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4494}{200908052059.37625.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4452}{200907302113.50797.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4453}{op.uxvraygp55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4467}{200908011944.15467.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4469}{4A742E9D.20805\%40gmx.de}
\@namedef{freecol-developers.mbox_4475}{200908021117.19813.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4477}{4A753F88.9010109\%40gmx.de}
\@namedef{freecol-developers.mbox_4486}{200908022109.08869.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4457}{580990fe0907300942x79699c7br27526fe48abb5a39\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4465}{4A73F2BA.1070304\%40gmx.de}
\@namedef{freecol-developers.mbox_4466}{4A73FF5F.4040003\%40gmx.de}
\@namedef{freecol-developers.mbox_4471}{4A743F4F.6060801\%40gmx.de}
\@namedef{freecol-developers.mbox_4472}{e6544a6541f2cea52df5d808879aff1c.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4473}{fac5a88b36b389beb9ca91b998084243.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4476}{4A753EC1.6070307\%40gmx.de}
\@namedef{freecol-developers.mbox_4478}{713c7e3d37604da6cd1bc3eb0c2a7682.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4474}{6af380b530ab929ca3987746e213217b.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4479}{4A754C69.2050009\%40gmx.de}
\@namedef{freecol-developers.mbox_4480}{4A755110.2090104\%40gmx.de}
\@namedef{freecol-developers.mbox_4481}{56f28b7c71f6fb8184333d9c945f0f6a.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4482}{4A7561B2.1070400\%40gmx.de}
\@namedef{freecol-developers.mbox_4483}{4ea3e133b26a04e82c1f1e21098ed6dc.squirrel\%40webmail.uio.no}
\@namedef{freecol-developers.mbox_4484}{3a7129160908020310x403096dr380fcb4be74e2d22\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4485}{4A7570DF.7090305\%40gmx.de}
\@namedef{freecol-developers.mbox_4487}{3a7129160908020530t5ae9d497l697df24247251b50\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4489}{op.ux3x3rii55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4491}{580990fe0908041001w434423feq156eae64de2c9c88\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4492}{4A786C66.2030206\%40gmx.de}
\@namedef{freecol-developers.mbox_4495}{4A7BC891.2020602\%40gmx.de}
\@namedef{freecol-developers.mbox_4497}{CB5B62CE-7D33-4E2F-B8EF-44C596AE56C8\%40nickshanks.com}
\@namedef{freecol-developers.mbox_4499}{4A8037D7.50300\%40gmx.de}
\@namedef{freecol-developers.mbox_4504}{580990fe0908101131h612ea4b2rd1dd435fad97eff6\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4498}{4A803601.8050408\%40gmx.de}
\@namedef{freecol-developers.mbox_4500}{op.uyge0jcn55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4503}{580990fe0908101122l2633c2adl32d97b37cc5fe67d\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4505}{200908112036.49202.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4506}{4A81852D.3000108\%40gmx.de}
\@namedef{freecol-developers.mbox_4501}{op.uyge7hyz55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4502}{580990fe0908101120n2c28e19bs5a42e6354893667\%40mail.gmail.com}
\@namedef{freecol-developers.mbox_4507}{4A8191F1.8010405\%40gmx.de}
\@namedef{freecol-developers.mbox_4515}{200908142117.46056.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4508}{4A86A44C.2010100\%40gmx.de}
\@namedef{freecol-developers.mbox_4528}{op.uyu9t7p855t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4531}{4A8B825B.8040507\%40gmx.de}
\@namedef{freecol-developers.mbox_4532}{200908192044.51720.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4533}{op.uywxcsj955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4537}{4A8CEAC8.7000609\%40gmx.de}
\@namedef{freecol-developers.mbox_4536}{4A8CEA8C.20902\%40gmx.de}
\@namedef{freecol-developers.mbox_4540}{200908201953.20632.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4541}{op.uyyxnx0755t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4542}{200908210727.49849.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4543}{op.uyzex7o755t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4545}{200908212010.17776.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4546}{op.uy0e9qiy55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4547}{4A8E9818.4060907\%40gmx.de}
\@namedef{freecol-developers.mbox_4548}{op.uy0mozrd55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4550}{200908241913.40906.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4551}{op.uy5xmwc155t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4552}{200908242156.25041.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4553}{op.uy548vx955t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4544}{4A8E495B.8000506\%40gmx.de}
\@namedef{freecol-developers.mbox_4538}{4A8CEB2F.3030505\%40gmx.de}
\@namedef{freecol-developers.mbox_4539}{op.uyx9uxdv55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4509}{4A86A50C.3050400\%40gmx.de}
\@namedef{freecol-developers.mbox_4510}{20090815155301.390b8413.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4511}{op.uypk1qlh55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4512}{4A86DCB7.60002\%40gmx.de}
\@namedef{freecol-developers.mbox_4513}{20090815211207.6f775e9c.dfisek\%40fisek.com.tr}
\@namedef{freecol-developers.mbox_4514}{op.uypuk9hc55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4516}{200908161834.58554.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4517}{200908162024.38654.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4518}{4A87EB2F.7070502\%40gmx.de}
\@namedef{freecol-developers.mbox_4519}{4A87EBE3.2040004\%40gmx.de}
\@namedef{freecol-developers.mbox_4520}{200908162122.27410.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4521}{4A881CC8.8090200\%40gmx.de}
\@namedef{freecol-developers.mbox_4522}{200908170814.24525.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4523}{4A88E21C.5010206\%40gmx.de}
\@namedef{freecol-developers.mbox_4524}{4A88E514.3080501\%40gmx.de}
\@namedef{freecol-developers.mbox_4525}{200908171918.29262.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4526}{4A8A33C6.1050702\%40gmx.de}
\@namedef{freecol-developers.mbox_4527}{200908182013.01357.mpope\%40computer.org}
\@namedef{freecol-developers.mbox_4529}{op.uyvj091f55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4530}{4A8B8114.5050404\%40gmx.de}
\@namedef{freecol-developers.mbox_4534}{op.uywxhn1v55t2cl\%40smtp.1und1.com}
\@namedef{freecol-developers.mbox_4535}{4A8CE5FF.3040009\%40gmx.de}
\@namedef{freecol-developers.mbox_4549}{COL110-W35EF1B0777E681FEBCFBF28CFA0\%40phx.gbl}
\@namedef{freecol-developers.mbox_4554}{4A92A6CD.6070201\%40gmx.de}
\@namedef{freecol-developers.mbox_4555}{4A92A9D9.20505\%40gmx.de}

\makeatother

